Understanding Queries by Conditional Instances

A powerful way to understand a complex query is by observing how it operates on data instances. However, specific database instances are not ideal for such observations: they often include large amounts of superfluous details that are not only irrelevant to understanding the query but also cause cognitive overload; and one specific database may not be enough. Given a relational query, is it possible to provide a simple and generic "representative" instance that (1) illustrates how the query can be satisfied, (2) summarizes all specific instances that would satisfy the query in the same way by abstracting away unnecessary details? Furthermore, is it possible to find a collection of such representative instances that together completely characterize all possible ways in which the query can be satisfied? This paper takes initial steps towards answering these questions. We design what these representative instances look like, define what they stand for, and formalize what it means for them to satisfy a query in "all possible ways." We argue that this problem is undecidable for general domain relational calculus queries, and develop practical algorithms for computing a minimum collection of such instances subject to other constraints. We evaluate the efficiency of our approach experimentally, and show its effectiveness in helping users debug relational queries through a user study.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/chase.tex <==
% \section{Chase}

\subsection{Tree Chase to Link Chase}
The previous tree-based algorithm is intuitive, however, it makes it hard to discuss the properties of the algorithm. Using the following equivalences, we can convert a DRC syntax tree into a right deep binary tree in which quantifier nodes can only appear at the root or be the right child of a node: 
\begin{align*}
\exists x \phi \land \psi \dashv \vdash \exists x (\phi \land \psi)\\
\exists x \phi \lor \psi \dashv \vdash \exists x (\phi \lor \psi)\\
\forall x \phi \land \psi \dashv \vdash \forall x (\phi \land \psi)\\
\forall x \phi \lor \psi \dashv \vdash \forall x (\phi \lor \psi)
\end{align*}

where $x$ is not free in $\psi$. 
\begin{Definition}[Right Deep Tree of DRC Formula]
A right deep tree of a DRC formula is a binary tree satisfying following rules:
\begin{enumerate}
    \item All leaf nodes are atoms or negation of atoms; atoms only appear in leaf nodes
    \item All internal nodes are quantifiers ($\forall$ and $\exists$) with variables or connectives ($\land$ and $\lor$)
    \item Each quantifier node has only one child; each connective node has two children.
    \item The root is a quantifier node. Except the root, each quantifier node must be either  the child of a quantifier node, or the right child of a connective node whose parent is a quantifier node.
    \item For each connective node with two children, the sub-tree rooted at its left child contains no quantifiers. 
    %If the connective node $t$ is the child of a quantifier node, then either there is no quantifier node in the subtree rooted at $t$, or the right child of $t$ is a quantifier node. 
\end{enumerate}
\end{Definition}

With the right-deep tree, we can perform the chase procedure without branching.

\begin{algorithm}[t]\caption{RD-Conjunctive-Tree-Chase}\label{alg:rd-conj-tree-chase}
{\small
\begin{codebox}
\algorithmicrequire $R$: the schema of the relational database; \\
$Q$: a right deep conjunctive tree of a DRC query; \\
$I$: current c-instance; \\
$f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
$\phi$: current conjunction of literals.\\
\algorithmicensure a list of list of c-instances\\
  \Procname{$\proc{RD-Conj-Tree-Chase-Static}(Q, I, f, \phi)$}
  \li \If there is no quantifier in $Q$
  \Then
    \li $\phi \gets \phi \land f(\proc{tree-to-conj}(Q))$
    \li $J \gets $ add $f(\phi)$ to $I$
    \li \If $J$ is consistent
        \Then \li \Return $J$
    \li \Else
        \li \Return $\bot$
        \End
  \End
  \li \If Q.root.operator $\in \{\land\}$
  \Then
    \li $\phi' \gets f(\proc{tree-to-conj}(Q.root.lchild))$
    \li \Return $\proc{RD-Conj-Tree-Chase-Static}(Q.root.rchild, I, f, \phi \land \phi')$
  \li \ElseIf Q.root.operator $\in \{\exists\}$
  \Then
    \li $res \gets []$
    \li \For $x \in I.domain(Q.root.variable)$
    \Do
        \li $g \gets f \cup \{Q.root.variable \to x\}$
        \li $res.append(\proc{RD-Conj-Tree-Chase-Static}(Q.root.child, I, g, \phi))$
    \End
    \li $I, \phi \gets \proc{Add-Fresh-Var}(Q.root.variable, I.domain(Q.root.variable), \phi)$
    \li $g \gets f \cup \{Q.root.variable \to Q.root.variable\}$
    \li $res.append(\proc{RD-Conj-Tree-Chase-Static}(Q.root.child, I, g, \phi))$
    \li \Return res
  \li \ElseIf Q.root.operator $\in \{\forall\}$
  \Then 
    \li \If $I.domain(Q.root.variable) = \emptyset$
        \Then
            \li $res.append(I)$
            \li $I, \phi \gets \proc{Add-Fresh-Var}(Q.root.variable, I.domain(Q.root.variable), \phi)$
        \End
    \li $Ilist \gets [I]$
    \li \For $x \in I.domain(Q.root.variable)$
    \Do
        \li $Ilist' \gets []$
        \li \For $J \in IList$
        \Do
            \li $g \gets f \cup \{Q.root.variable \to x\}$
            \li $J' \gets \proc{RD-Conj-Tree-Chase-Static}( Q.root.child, J, g)$ 
            \li \If $J' \neq \bot$
                \Then \li $Ilist'.append(J')$
            \End
        \End
        \li $Ilist \gets Ilist'$
    \End
    \li \Return $Ilist$
    
  \End
\end{codebox}
}
\end{algorithm}

\begin{Definition}[Conj-Chase Step]
Let $K$ be a c-instance, we construct a c-instance $K'$ by adding relational atoms and conditions to $K$. This is done by traversing the right deep conjuetive tree of query $Q$. As illustrated in Algorithm~\ref{alg:rd-conj-tree-chase}, we traverse the tree through right edges. Let $T$ be the current tree, $h$ be current homomorphism, and $\phi$ be current conjuct, thus $h$ maps $Var(T.ancestors) \cup FreeVar(Q) \cup Cons(\phi)$ to $Var(K) \cup Cons(K)$. We have four possible cases:
\begin{enumerate}
    \item $T.root$ is $\land$ (Line 8-10), we obtain $\phi'$ from the left branch of $T.root$ (it is quantifier free), and then go to the right branch.
    \item $T.root$ is $\exists$ (Line 12-18), we try every possible extenstion of $h$ to a homomorphism from $Var(T.ancestors)\cup FreeVar(Q) \cup Cons(\phi) \cup \{T.root.variable\}$ to $Var(K) \cup Cons(K)$ and the extension of $h$ such that $T.root.variable$ is assigned a fresh variable.
    (To ensure safety, whenever a fresh variable is created, a new tuple is also added to $K$ based on the domain.)
    \item $T.root$ is $\forall$ (Line 20-32), first we check if the domain of $Q.root.variable$ is empty. If it is empty, we have the current instance as a valid solution, and add a fresh variable to this domain.
    Then similarly, we try every possible extenstion of $h$ to a homomorphism from $Var(T.ancestors)\cup FreeVar(Q) \cup Cons(\phi) \cup \{T.root.variable\}$ to $Var(K) \cup Cons(K)$, but this time for every extension $h'$ of $h$, we have to keep performing conj-chase on the returned c-instances of the previous extension. (Let the formula of $T$ be the form $\forall x (\alpha(x) \land \beta(x))$ where $\alpha$ is a quantifier-free conjunction and $\beta$ has quantifiers, the instance $K$ satisfies $T$ only if $$\bigwedge\limits_{g: \{x \rightarrow dom(I)\} \cup h} \big (\alpha(g(x)) \land \beta'(g(x)) \big)$$ is true, where $\beta'$ is the quantifier-free formula by further extending $h$ inside $\beta$.
    \item If $T$ is quantifier free, then it comes to the end of one mini conj-chase step. We add to $K$ the images of the atoms/conditions of $\phi$ under $h$ and obtain $K'$.
 )
\end{enumerate}


\begin{algorithm}[t]\caption{Right-Deep-Conjunctive-Tree-Chase}\label{alg:rd-deep-conj-tree-chase}
{\small

\begin{codebox}
\algorithmicrequire $R$: the schema of the relational database; \\
$Q_1, Q_2$: two DRC queries; \\
$limit$: the maximum number of tuples in the c-instances\\
\algorithmicensure A list of c-instances that represent counterexamples for $Q_1$ and $Q_2$. \\
\Procname{$\proc{RD-Conj-Tree-Chase}(R, Q_1, Q_2, limit)$}
\li $Q'_1 \gets \exists \mathbf{x} (Q_1)$ where $x$ are the free variables in $Q_1$
\li $Q'_2 \gets \exists \mathbf{x} (Q_2)$ where $x$ are the free variables in $Q_2$
\li $Q \gets Q'_1 \land \neg Q'_2$
\li $Tlist \gets \proc{Conj-Tree-Cons}(Q)$
\li $res \gets []$
\li \For $T \in Tlist$
    \Do
    \li $u \gets $ a conj-chase tree of one single node labeled by an empty c-instance of $R$
    \li \While $True$
        \Do
            \li $updateFlag \gets False$
            \li \For $v \in u.leaves$
            \Do
                \li \If $\proc{Conj-Tree-SAT-Static}(T, v.label, \emptyset)$
                    \Then  
                        \li $res.append(v.label)$
                        \li continue
                    \End
                \li $Ilist \gets \proc{Conj-Tree-Chase-Step}(T, I, \{\}, True)$
                \li \For $J \in Ilist$
                \Do
                   \li \If $J \neq \bot$ and $|J| < limit$
                    \Then
                        \li Add to $v$ a child node labeled by $J$
                        \li $updateFlag = True$
                    \End
                \End
            \End
            \li \If $updateFlag$
                \Then
                 \li Break
                \End 
            \li \If all $u.leaves$ are $\bot$ or reach the size limit
                \Then 
                    \li Break
                \End
            \li \If  $\proc{Conj-Tree-SAT-Static}(T, I, \{\})$ 
                \Then
                    \li $res.append(I)$
                    \li Break
                \End
        \End
    \End
\li \Return $res$
\end{codebox}
}
\end{algorithm}

After every mini conj-chase step, we check $K'$ for satisfiability / consistency. There are two cases: (1) If $K'$ is not satisfiable we say the result of chasing $Q$ with $h$ on $K$ is failure and denote $K \xrightarrow[]{\phi, h} \bot$, and (2) otherwise $K'$ is satisfiable and thus $Rep(K') \neq \emptyset$, we say the result of chasing $Q$ with $h$ on $K$ is $K'$, and denote $K \xrightarrow[]{\phi, h} K'$.

Running the procedure $\proc{RD-Conj-Tree-Chase-Static}$ would execute multiple mini conj-chase steps and we say it as a conj-chase step. A conj-chase step would return a list of c-instances in which every c-instance is obtained by chasing $q$ with multiple homomorphsims. Therefore, a conj-chase step on $K$ will contribute paths of a conj-chase tree. 
\end{Definition}

A conj-chase tree is a tree where each node is labeled by a c-instance and the root is $\emptyset$. Each mini conj-chase step presents an edge in this conj-chase tree, and thus a conj-chase step on $K$ expands the conj-chase tree by seeding the subtree rooted at $K$. The target is to have each leaf node to be labeled by a counterexample c-instance $K'$ satisfying $Q$ or the failure case $\bot$. So the conj-tree chase step is performed on every leaf node until there is no leaf node labeled with c-instances not satisfying $Q$.
The result of a conj-chase tree is the set of all non-failure leaf nodes.
\begin{Definition}[Ground Solution]
Let $T$ be a RD-conjunctive tree of the query $Q$, a ground solution $K$ of $T$ is a ground instance such that $T$ satisfies $K$ and thus $Q(K) \neq \emptyset$.
\end{Definition}


\begin{Example}
Consider one single query:$Q_1:$ Find the drinkers for whom every beer liked by the drinker is also liked by another drinker.

\begin{align*}
Drinker & \join_{name = drinker1} ( \\
    &\rename_{drinker1, beer1} Likes \join_{beer1 = beer2 \land  drinker1 \neq drinker2} \\
    &\rename_{drinker2, beer2} Likes));
\end{align*}

The DRC of $Q_1$:
\begin{align*}
\{(d_1) \ \mid  \exists a_0 &Drinker(d_1, a_0) \land \\
\forall b_1 &\Big(\neg Likes(d_1, b_1) \lor \\
&\exists d_2 \big(Likes(d_2, b_1) \land d_1 \neq d_2\big)\Big)\}
\end{align*}

Possible counterexamples:
\begin{itemize}
\item Case a: With only one drinker $(d_1, *)$.
\item Case b: With one drinker $(d_1, *)$ and beer $(b_1, *)$, $\neg Likes(d_1, b_1)$.
\item Case c: With two drinkers $(d_1, *)$, $(d_2, *)$ where $d_1 \neq d_2$ and beer $(b_1, *)$, $\neg Likes(d_1, b_1)$ and $Likes(d_2, b_1)$.
\item Case d: With two drinkers $(d_1, *)$, $(d_2, *)$ where $d_1 \neq d_2$ and beer $(b_1, *)$, $Likes(d_1, b_1)$ and $Likes(d_2, b_1)$.
\end{itemize}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/conj-trees.png}
    \caption{RD-Conjunctive trees of $Q_1$ marked by resulting c-instances. Note that case $a$ can come from either of this.}
    \label{fig:eg-conj-tree}
\end{figure*}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/rd-conj-chase-steps-ab.png}
    \caption{Chase steps of RD-Conjunctive trees of $Q_1$, case $a$ and $b$.}
    \label{fig:eg-conj-tree-chase-steps-ab}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/rd-conj-chase-steps-cd.png}
    \caption{Chase steps of RD-Conjunctive trees of $Q_1$, case $c$ and $d$.}
    \label{fig:eg-conj-tree-chase-steps-cd}
\end{figure}

\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{4em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & $T$ \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
      \end{tabular}
      }
    \end{minipage}
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case1}\small
  The c-instance of case a.}
\end{figure}
\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{4em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & $T$ \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $b_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
        \multicolumn{3}{|c|}{$\neg Likes(d_1, b_1)$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case1}\small
  The c-instance of case b.}
\end{figure}
\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{4em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & $d_1 \neq d_2$ \\
        $d_2$ & $*$ & $d_1 \neq d_2$ \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $b_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $d_2$ & $b_1$ & $T$ \\\hline
        \multicolumn{3}{|c|}{$\neg Likes(d_1, b_1)$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case1}\small
  The c-instance of case c.}
\end{figure}

\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
     \begin{minipage}[b]{0.30\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{4em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & $d_1 \neq d_2$ \\
        $d_2$ & $*$ & $d_1 \neq d_2$ \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $b_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $d_1$ & $b_1$ & $T$ \\
       $d_2$ & $b_1$ & $T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case1}\small
  The c-instance of case d.}
\end{figure}



\amir{Is this a universal solution? Will all these be outputted by Algorithms 5,7,8,9?}

\end{Example}


\begin{Definition}[Universal Solution]
Let $T$ be a RD-conjunctive tree of the query $Q$, a universal solution of $T$ is a set of c-instances $\mathcal{J} = \{J_1, ..., J_n\}$ such that for every ground solution $K$ of $T$, it has a subinstance $K' \subseteq K$ where $K' \in Rep(J_i)$ for some $J_i \in \mathcal{J}$.
\end{Definition}


\begin{proposition}
Let $T$ be a RD-conjunctive tree of the query $Q$, let $I$ be a c-instance initialized using free variables in $Q$. Assume $t$ is a finite conj-chase tree rooted at $I$ for $Q$, the the result of $t$ is a universal solution for $Q$.
\end{proposition}
\begin{proof}
Let $\mathcal J$ be the result of $t$. $\mathcal J$
consists of c-instances that satisfies $Q$. For every ground solution $K$, we need to show that it has a subinstance $K' \subseteq K$ where $K' \in Rep(J_i)$ for some $J_i \in \mathcal{J}$.
We can obtain such a $K'$ by construction: in the conj-chase step, instead of adding fresh variables to the domain of current instance, we use constants from $K.domain$ such that the atoms and conditions in $\phi = \psi_{free} \land \gamma_{free} \land \psi_{cons} \land \gamma_{cons}$, where $\psi_{free}$ ($\gamma_{free}$, respectively) is the conjunction of atoms (conditions, respectively) that contain free variables in $Q$ and $\psi_{cons}$ ($\gamma_{free}$, respectively) is the conjunction of atoms (conditions, respectively) without free variables in $Q$, satisfy that $h(\psi_{cons})$ only has atoms in $K$ and $h(\gamma_{cons})$ is satisfied. Then, for each c-instances in the result of the new conj-chase tree, we can validate if there is a mapping $g$ from $FreeVar(Q)$ to $Cons(K)$, and $(g \cup h)(\psi_{free})$ is also in $K$ and $(g \cup h)(\gamma_{free})$ is satisfied. This construction indicates we can find a homomorphsim from some c-instance $J$ in the result of conj-chase tree to a subinstance $K'$ of any ground solution $K$ of $T$, therefore $K' \in Rep(J)$.
\end{proof}

==> sections/completeness_proof.tex <==
\subsection{Completeness Proof}\label{sec:completeness}

We next prove Theorem~\ref{theorem:completeness}. 
% First, we need Lemma~\ref{lemma:ground_to_c}.

% \begin{Lemma}\label{lemma:ground_to_c}
% Given a DRC query syntax tree $Q$ and a ground instance $\ains$ satisfying $Q$ with coverage $\cov_\ains$, there exists a c-instance $\cinstance$ containing only atoms from $Q$ as tuples with labeled nulls replacing variables and constants from $Q$ such that $\cov_\ains = \cov_\cinstance$. 
% \end{Lemma}

% \begin{proof}
% Let $\assignment_1, \ldots, \assignment_l$ be the assignments that satisfy $Q$ w.r.t. $\ains$. 
% We generate a c-instance $\cinstance$ with the same schema as $Q$ in the following manner. For each atom satisfied by an assignment $\assignment_i$, the atoms satisfied by $\assignment_i$ are added as tuples of $\cinstance$ in their respective tables (according to their relation names) and the set of selection conditions satisfied by $\ains$ under every $\assignment_i$ are added as the global conditions of $\cinstance$, in addition to negated atoms that do not appear in $\ains$. 

% We need to show that $\cinstance$ is satisfiable and that its coverage is equal to that of $\ains$. 
% We first show that $\cinstance$ is satisfiable.
% Since $\ains$ is a ground instance, it cannot contain a contradiction and cannot satisfy contradicting conditions even from different assignments (i.e., it cannot be that $\assignment_i$ satisfies a conditions that contradicts a conditions satisfied by $\assignment_j$). 
% We only included the conditions satisfied by $\assignment_1\cup \ldots \cup \assignment_l$ and thus the conjunction of these conditions is satisfiable. 
% To show $\cov_\ains = \cov_\cinstance$, consider the way $\cinstance$ was built. For every satisfying assignment $\assignment_i$, we included all atoms and conditions satisfied by $\assignment_i$ as tuples in $\cinstance$, therefore, $\cov_\cinstance = \bigcup_{i=1}^l \assignment_i[K]^-1 = \cov_\cinstance$
% \end{proof}


\begin{proof}[Proof of the conjunction case in Theorem \ref{theorem:completeness}]
We prove the theorem by induction on the number of nodes in the syntax tree $Q$. 

First, note that the process that starts with Algorithm \ref{alg:rd-tree-chase-main} and illustrated in Figure \ref{fig:chase_illustration} generates a chase tree that contains all c-instances that covers any subset of atoms and conditions from $Q$ up to size $limit$, since, for every node, every possible mapping from a variable to a labeled null or constant is considered. 

If $|Q| = 1$, there is only one leaf node $u$ it can only be an atom or the negation of an atom, and the coverage can only be $\{u\}$ (otherwise $Q$ is not satisfied).
In this case, the algorithm simply calls $\proc{Tree-Chase}$ one time to add this atom to the empty c-instance and returns a list with only this instance, which covers $u$. 

Assume that for any query syntax tree $Q$ of size $< n$, for any ground instance $\ains$ with coverage $\cov$, Algorithm \ref{alg:rd-tree-chase-main} finds a c-instance $\cinstance$ with coverage equal to $\cov$.
We show that the claim is true for $Q$ with $|V(Q)| = n$, considering the four cases according to the four types of inner nodes.

Assume $Q = Q_1 \land Q_2$ is of size $n$ and there is a ground instance $\ains$ covering $Q$ with coverage $\cov_\ains$. 
Thus, $\ains$ covers $Q_1$ with coverage $\cov^1_\ains$ and covers $Q_2$ with coverage $\cov^2_\ains$. 
Based on the induction hypothesis, there exist $\cinstance_1, \cinstance_2$ found by Algorithm 
\ref{alg:rd-tree-chase-main} with coverages $\cov^1_\ains$ and $\cov^2_\ains$ respectively (as $Q_1$ and $Q_2$ both have size smaller than $n$). 
To compute the c-instances for $Q$, Algorithm 
\ref{alg:rd-tree-chase-main} calls Algorithm 
\ref{alg:rd-tree-chase} that calls Algorithm 
\ref{alg:and-op} to handle the conjunction. 
So, the c-instance $\cinstance_1$ is part of the list generated in line 1 of the algorithm, and  $\cinstance_2$ is merged into it in line 5. 
Our goal is then to show that one of the merged c-instances, $\cinstance^\star$, is satisfiable and has coverage $\cov_\ains$. 
The merge is defined as adding the tuples in $\cinstance_1$ to $\cinstance_2$ along with its mappings, and joining their global conditions using a conjunction \amir{check with Zhengjie}. 

Since $\ains$ is a ground instance, it cannot contain a contradiction and cannot satisfy contradicting conditions of $Q$, even from different assignments. 
The conditions included in $\cinstance_1$ and in $\cinstance_2$ are subsets of the conditions satisfied by $\ains$ and their conjunction is also satisfied by $\ains$ and thus they do not contradict each other. 

For coverage, observe that $\cov_\ains = \cov^1_\ains \cup \cov^2_\ains$. This is exactly the coverage of $\cinstance^\star$, obtained from merging $\cinstance_1$ and $\cinstance_2$.

% To compute the c-instances for $Q$, Algorithm 
% \ref{alg:rd-tree-chase-main} calls Algorithm 
% \ref{alg:rd-conj-tree-chase} that calls Algorithm 
% \ref{alg:and-op} to handle the conjunction. 


% From lemma \ref{lemma:ground_to_c}, we know that there exists a c-instance $\cinstance^\star$ that has coverage $\cov_\ains$. 
% Thus, there are two c-instances $\cinstance_1$ and $\cinstance_2$ that are part of the lists generated in lines 1 and 5 of the algorithm, respectively, such that $\cinstance_1 \cup \cinstance_2$ does not have a contradiction and has coverage $\cov_\ains$. 

Suppose the root of $Q$ is a disjunction node, i.e., $Q = Q_1 \lor Q_2$ where $|Q_1| < n$ and $|Q_2| < n$. 
% and then the coverage $\cov = \cov_1 \cup \cov_2$ where $\cov_1$ is a subset of leaf atoms of $Q_1$ and $\cov_2$ is a subset of leaf atoms of $Q_2$. 
The disjunction algorithm (Algorithm \ref{alg:or-op}) splits $Q$ into three cases (line 1), where each is rooted by a $\land$ node: (1) $Q_1 \land Q_2$, (2) $\neg Q_1 \land Q_2$, and (3) $Q_1 \land \neg Q_2$. $\ains$ can only satisfy one of these cases since they are disjoint. W.l.o.g., suppose $\ains$ satisfies (1) with coverage $\cov_1$. 
Form the previous conjunction case, we know that, for each of the conjunctive cases, there is an instance $\cinstance_1$, $\cinstance_2$, $\cinstance_3$ with coverage $\cov_1$, $\cov_2$, $\cov_3$, respectively.
In particular, $\cinstance_1$ has the same coverage as $\ains$.

Suppose the root of $Q$ is an existential node: $Q = \exists x.~ Q'(x)$ where $|Q'| < n$.
Then, $\ains$ has coverage $\cov$ of $Q'[x \gets c]$, where $Q'[x \gets c]$ is $Q'$ with $x$ assigned to the constant $c$. 
By the induction hypothesis, there is a c-instance $\cinstance'$ outputted by Algorithm~\ref{alg:rd-tree-chase-main} for $Q'[x \gets c]$ with coverage $\cov'$. 
Algorithm \ref{alg:exists-op} tries all possible domain assignments to $x$, and in particular, it tries to assign the labeled null/constant appearing in domain of the current c-instance (lines 1--3) and a fresh labeled null in addition (lines 4--7). Therefore, the algorithm inevitably attempts to assign $x$ with the labeled null/constant appearing in the cell of $c$, creating $\cinstance'$ with coverage $\cov$. 
% $\cov' = \cov$ since the only difference between the queries is the assignment of a specific constant to $x$ which does not give more coverage. 
 

Suppose the root of $Q$ is a universal quantifier: $Q = \forall x.~ Q'(x)$ where $|Q'| < n$ and $\ains$ covers $Q$ with coverage $\cov$. Unlike the above $\exists$ case, for $Q'$, different subsets of $\cov$ (denoted as $\cov_1, ..., \cov_l$, where \cov = $\bigcup_{i=1}^{l}\cov_i$) are all covered under different mappings of the free variable $x$ to different constants $c_i$ in the domain of $x$ in $\ains$. 
Algorithm \ref{alg:forall-op} iterates over all of these mappings and joins all of them to see if the obtained instance with the many-to-many relation mapping $x$ to $c_1, \ldots, c_l$ is consistent (lines 5--15) and further tries to add a fresh labeled null as an assignment to $x$ (lines 16--24). 
From the induction hypothesis, we know that there are c-instances $\cinstance_1, \ldots, \cinstance_l$ with coverages $\cov_1, \ldots, \cov_l$ for each constant $c_i$. 
Since $\ains$ satisfies $Q$, there is no contradiction between $Q'[x \gets c_1], \ldots, Q'[x \gets c_l]$, where $Q'[x \gets c_i]$ is $Q'$ with $x$ assigned to $c_i$, i.e., $x$ can be assigned any constant from $\{c_1, \ldots, c_l\}$ and $\ains \models Q$. 
Therefore, Algorithm \ref{alg:forall-op} generates a consistent c-instance $\cinstance^\star$ that satisfies $Q'[x \gets c_1]\land \ldots \land Q'[x \gets c_l]$ and thus has coverage $\cup_{i=1}^l \cov_i$.
\end{proof}


\subsection{From Section 3}


\subsection{Analysis of Algorithm \ref{alg:rd-tree-chase-main}}\label{sec:analysis}


\mypar{Soundness and completeness}
% \begin{proposition}[Soundness]
% Given a right deep syntax query tree $Q$, the c-instances outputted by Algorithm \ref{alg:conj-tree-cons} all satisfy $Q$.
% \end{proposition}
Given a syntax tree $Q$ of a DRC query, Algorithm~\ref{alg:rd-tree-chase-main} when given $(\schemaOf{R}, Q, \emptyset, \emptyset)$ will output a list of c-instances that are consistent and satisfy the query denoted by $Q$ (validated in Line 13), i.e., our procedure is sound. 
%The full proofs can be found in the full version \cite{?} \amir{cite}.

% \begin{Theorem}[Soundness]
% Given a syntax tree $Q$ of a boolean DRC query and a c-instance $\cinstance$, $\cinstance$ satisfies $Q$ iff Algorithm
% ~\ref{alg:tree-sat} returns True on $\proc{Tree-SAT}(Q, \emptyset, \emptyset)$.
% \end{Theorem}

\cut{
\begin{Theorem}[Soundness]\label{thm:soundness}
Let $Q$ be a syntax tree of a DRC query over a schema $\schemaOf{R}$, and let $\cinstance$ be a c-instance in the set outputted by Algorithm \ref{alg:rd-tree-chase-main} when given $(\schemaOf{R}, Q, \emptyset, \emptyset)$, then $\cinstance$ satisfies $Q$.
\end{Theorem}



\begin{proof}[proof sketch]
To prove the proposition, it is enough to show that in Line 14 of Algorithm \ref{alg:rd-tree-chase-main} the procedure for checking that the c-instance $I$ satisfies the query $Q$\footnote{The pseudo code of the procedure, along with a proof of correctness are included in the full version \cite{?} \amir{cite}}. 
% This is shown in Proposition \ref{prop:soundness-conj-sat} in the Section \ref{sec:tree-sat}, proving that Algorithm \ref{alg:tree-sat} returns true iff the given c-instance $\cinstance$ satisfies the given syntax tree $Q$. \amir{The proof we rely on is in the appendix}
\end{proof}
}

% \begin{Lemma}
% Given a syntax tree $Q$ and the set of c-instances $\mathcal{S}_{\cinstance} = \{\cinstance_1, \ldots, \cinstance_k\}$ outputted by Algorithm \ref{alg:rd-tree-chase-main}, if $\cov$ is the coverage of some ground instance $K$ satisfying $Q$, then there is $\cinstance_i \in \mathcal{S}_{\cinstance}$ with coverage $\cov$.
% \end{Lemma}

%\begin{Theorem}[Completeness]\label{theorem:completeness}
\begin{Proposition}
[Completeness]\label{theorem:completeness}
Given a syntax query tree $Q$ and a ground instance $\ains$ such that $\ains \models Q$ and 
its coverage $\coverage(Q, k) = \cov$, and there exists a c-instance $\cinstance^\star$ of size $\leq limit$ with coverage $\cov$, 
then the set of c-instances $\mathcal{S}_{\cinstance} = \{\cinstance_1, \ldots, \cinstance_k\}$ returned by Algorithm \ref{alg:rd-tree-chase-main} with the parameter $limit$ contains a c-instance $\cinstance_i \in \mathcal{S}_{\cinstance}$ with coverage $\cov$.



\cut{
\red{Given a syntax query tree $Q$ and the set of c-instances $\mathcal{S}_{\cinstance} = \{\cinstance_1, \ldots, \cinstance_k\}$ returned by Algorithm \ref{alg:rd-tree-chase-main} with  parameter $limit$, if there is a ground instance $K$ such that $K \models Q$ and % that satisfies $Q$ with coverage 
its coverage $\coverage(Q, k) = \cov$, if there exists a c-instance of size $\leq limit$ with coverage $\cov$
then there exists a c-instance $\cinstance_i \in \mathcal{S}_{\cinstance}$ with coverage $\cov' = \cov$.} \sr{please check -- how does limit affect K?}

Given a syntax query tree $Q$ and the set of c-instances $\mathcal{S}_{\cinstance} = \{\cinstance_1, \ldots, \cinstance_k\}$ outputted by Algorithm \ref{alg:rd-tree-chase-main} with the parameter $limit$, if a ground instance $\ains$ that satisfies $Q$ with coverage $\cov$,
then there exists $\cinstance_i \in \mathcal{S}_{\cinstance}$ with coverage $\cov' = \cov$. \amir{Rephrased. Verify}
}
\end{Proposition}
%\end{Theorem}


\sr{do not follow the proof yet -- stopping here}
\begin{proof}[proof sketch]
The proof is by induction over the size of the syntax tree, where the base case is proven by considering a c-instance of size $1$ generated in lines 2--7 in Algorithm \ref{alg:rd-tree-chase}. 
The induction then proceeds to consider the cases where $Q = Q_1\land Q_2$, $Q = Q_1\lor Q_2$, $Q = \exists x.~Q'$, and $Q = \forall x.~Q'$. 

\amir{This can be removed if we need space:}
As an example, we give the proof for the conjunctive case: Assume $Q = Q_1 \land Q_2$ is of size $n$ and there is a ground instance $\ains$ covering $Q$ with coverage $\cov_\ains$. 
Thus, $\ains$ covers $Q_1$ with coverage $\cov^1_\ains$ and covers $Q_2$ with coverage $\cov^2_\ains$. 
Based on the induction hypothesis, there exist $\cinstance_1, \cinstance_2$ found by Algorithm 
\ref{alg:rd-tree-chase-main} with coverages $\cov^1_\ains$ and $\cov^2_\ains$ respectively (as $Q_1$ and $Q_2$ both have size smaller than $n$). 
To compute the c-instances for $Q$, Algorithm 
\ref{alg:rd-tree-chase-main} calls Algorithm 
\ref{alg:rd-tree-chase} that calls Algorithm 
\ref{alg:and-op} to handle the conjunction. 
So, the c-instance $\cinstance_1$ is part of the list generated in line 1 of the algorithm, and  $\cinstance_2$ is merged into it in line 5. 
Our goal is then to show that the algorithm generates a new c-instance $\cinstance^\star$ that is  of $\cinstance_1$ and $\cinstance_2$ is satisfiable and has coverage $\cov_\ains$. 
The merge is defined as adding the tuples in $\cinstance_1$ to $\cinstance_2$ along with its mappings, and joining their global conditions using a conjunction \amir{check with Zhengjie}. 

Since $\ains$ is a ground instance, it cannot contain a contradiction and cannot satisfy contradicting conditions of $Q$, even from different assignments. 
The conditions included in $\cinstance_1$ and in $\cinstance_2$ are subsets of the conditions satisfied by $\ains$ and their conjunction is also satisfied by $\ains$ and thus they do not contradict each other. 

For coverage, observe that $\cov_\ains = \cov^1_\ains \cup \cov^2_\ains$. This is exactly the coverage of $\cinstance^\star$, obtained from merging $\cinstance_1$ and $\cinstance_2$.
\end{proof}

\mypar{Termination}
Recall that in Section \ref{sec:model} we have determined that that the problem of finding a universal solution (Definition \ref{def:universal}) is undecidable. 
Despite this, Algorithm \ref{alg:rd-tree-chase-main} is guaranteed to terminate due to the $limit$ parameter (Line 11) and the $visited$ set.

\begin{proposition}
Given a query syntax tree $Q$, Algorithm \ref{alg:rd-tree-chase-main} is guaranteed to terminate.
\end{proposition}

\begin{proof}
Since the $limit$ parameter is finite, there are finitely many options for c-instances that it can generate. If the size of the c-instance increases over $limit$, the algorithm will ignore this c-instance and not push it into $queue$ (Lines 11--12). 
The algorithm will also not get into an infinite loop as well because of the $visited$ set. Every generated c-instance is placed into this set and c-instance already found is the set are ignored and are not pushed into $queue$ (Lines 11--12). 
% There may still be an infinite loop in Line 9 is a domain of a variable is infinite. However, since all the procedures used by Algorithm \ref{alg:rd-tree-chase-main}
Finally, note that the domain of all labeled nulls in the c-instance is derived from existing labeled nulls representing the same attribute in the c-instance, and thus cannot be infinite.
\end{proof}

% However, even without it, if the domain of all variables is finite, Algorithm \ref{alg:rd-tree-chase-main} is guaranteed to terminate since the number of combinations of domain values is finite. 
% Note that the algorithm may expand the initial domain of the variables (e.g., Lines 16--17 in Algorithm \ref{alg:forall-op}) but this would occur a finite number of times during the process.

% \amir{Add that if all domains a finite, then termination is guaranteed.}
% The proof of Theorem~\ref{theorem:completeness} needs Lemma~\ref{lemma:union-c-homo}, Lemma~\ref{lemma:and-sat}, and Lemma~\ref{lemma:forall-sat}.

% \begin{Lemma}\label{lemma:union-c-homo}
% Given two c-instances $J_1$ and $J_2$ that c-homomorphically map to a ground instance $K$ under $\assignment_1$ and $\assignment_2$ respectively, if for every $x \in vars(J_1) \cap vars(J_2)$, $\assignment_1(x) = \assignment_2(x)$, $J_1 \cup J_2$ c-homomorphically maps to $K$ under $\assignment_1 \cup \assignment_2$.
% \end{Lemma}

% \begin{proof}
% We show that $\assignment = \assignment_1 \cup \assignment_2$ is a c-homomorphism from $J_1 \cup J_2$ to $K$. Let $\phi \in J_1 \cup J_2$ be an arbitrary relational atom $\rel(x_1, ..., x_{\relarity})$, by the definition of c-homomorphism, $K$ contains $\rel(\assignment(x_1), ..., \assignment(x_{\relarity}))$; let $\phi$ be the negation of an arbitrary relational atom $\neg \rel(x_1, ..., x_{\relarity})$, $K$ does not contain the relational fact  $\rel(\assignment(x_1), ..., \assignment(x_{\relarity}))$, and thus $\assignment(J_1 \cup J_2)$ does not contain $\rel(\assignment(x_1), ..., \assignment(x_{\relarity}))$; let $\phi \in J_1 \cup J_2$ be an arbitrary binary expression $x~op~y$, we also have the image under $\assignment$ of this expression $\assignment(x)~op~\assignment(y)$ to be True in $K$. Hence $J_1 \cup J_2$ c-homomorphically maps to $K$ under $\assignment_1 \cup \assignment_2$. \SR{polish}
% \end{proof}

% \begin{Lemma}\label{lemma:and-sat}
% Given a DRC query $Q=Q_1 \land Q_2$, a ground instance $K$ that satisfies $Q$, and two c-instances $J_1$ and $J_2$ that c-homomorphically map to $K$ and satisfy $Q_1$ and $Q_2$ respectively, if either $Q_1$ or $Q_2$ has no quantifiers, then $J_1 \cup J_2$ c-homomorphically map to $K$ and satisfies $Q$.
% \end{Lemma}

% % \begin{Lemma}\label{lemma:union-coverage}
% % Given two c-instances $J_1$ and $J_2$ that c-homomorphically map to a ground instance $K$ under $h_1$ and $h_2$ respectively and a syntax query tree $Q$ where $J_1$ and $J_2$ satisfy $Q$ with coverage $\cov_1$ and $\cov_2$ respectively, $J_1 \cup J_2$ satisfies $Q$ 
% % \end{Lemma}

% \begin{Lemma}\label{lemma:forall-sat}
% Given a DRC query $Q=\forall x Q'(x)$, a ground instance $K$ that satisfies $Q$, and $l$ c-instances $J_1, J_2, ..., J_l$ that c-homomorphically map to $K$ and satisfy $h_i(Q')$ respectively, where $l = |K.dom(x)|$ and each $h_i$ maps the free variable $x$ in $Q'$ to a different value in $K.dom(x)$, if either $Q_1$ or $Q_2$ has no quantifiers, then there exist c-instances $J'_1, J'_2, ..., J'_l$ such that each $J_i$ homomorphically maps to $J'_i$ and $\bigcup_{i=1}^{l} J'_i$) c-homomorphically maps to $K$ and it satisfies $Q$.
% \end{Lemma}

% \begin{proof}[Proof for Theorem~\ref{theorem:completeness}]
% We prove the theorem by induction of the number of nodes in the syntax tree $Q$. 

% %\zhengjie{safety issue here}
% If $|V(Q)| = 1$, there is only one leaf node $u$ --- it can only be an atom or the negation of an atom \SR{do you keep the $\neg$? see defn 11}, and the coverage can only be $\{u.atom\}$ (otherwise $Q$ evaluates to an empty result), and the homomorphism $\mrel$ maps the free variables in $u.atom$ to vales in $K$, i.e., $h(u.atom)$ exists in $J$ if it is a relational atom, or it evaluates to True otherwise.
% In this case, the algorithm simply calls $\proc{RD-Tree-Chase}$ one time to add this atom to the empty c-instance and returns a list with only this instance, which covers $u.atom$. $\mrel$ is the c-homomorphism from the variables in $u.atom$ to values in $K$.

% Assume that for every $Q$ such that $|V(Q)| < n$, for a ground instance $K$ satisfying $Q$ with coverage $\cov$ under a homomorphism $\mrel$, there is a c-instance in the result of Algorithm~\ref{alg:rd-tree-chase-main} has coverage $\cov' \supseteq \cov$ for $Q$ that c-homomorphically maps to $K$.  We show that the claim is true for $Q$ with $|V(Q)| = n$.

% If the root of $Q$ is an $\land$ node, i.e., $Q = Q_1 \land Q_2$ where $V|Q_1| < n$ and $V|Q_2| < n$, and then the coverage of $K$ for $Q$ is $\cov = \cov_1 \cup \cov_2$ where $\cov_1$ is a subset of leaf atoms of $Q_1$ and $\cov_2$ is a subset of leaf atoms of $Q_2$.  Since the tree $Q$ is a right deep syntax tree, its left child $Q_1$ has no quantifiers (has only connecitves and leaf atoms), in lines 14 it directly generates a list of conjunction of atoms from $Q_1$ by expanding disjunctions into three conjuncive cases ($A \lor B \to \{A \land B, A \land \neg B, \neg A \land B$\}), then any $\cov_1$ \amir{any $\cov_1$?} of $Q_1$ must be covered in one of the expanded conjunctions. Furthermore, note that keep running the procedure $\proc{RD-Tree-Chase}$ in Algorithm~\ref{alg:rd-tree-chase-main} does not change the results on $Q_1$ --- the free variables are all assigned fresh variables at the beginning of Algorithm~\ref{alg:rd-tree-chase-main}, and thus it does not add new variables to the domain of the c-instances. 
% Therefore, we run Algorithm~\ref{alg:rd-tree-chase-main} on $Q$ as running Algorithm~\ref{alg:rd-tree-chase-main} on $Q_1$ and $Q_2$ separately, and then merging the result instances from $Q_1$ to the result instances from $Q_2$. %In line 15-16, we write it as a recursive call to $\proc{RD-Tree-Chase}$ on the right child $Q_2$ of $Q$ for each of the expanded conjunction from $Q_1$. 
% % \amir{I wasn't able to follow this argument. Can't there be an intersection between the domains considered in $Q_1$ and those considered in $Q_2$? e.g., if the root of $Q_2$ is a universal quantifier that applies to the vars in $Q_1$}. 
% %Since there must be a expanded conjunction from $Q_1$ with coverage $\cov_1$, and by

% \begin{figure}[h]
% \centering
%  \includegraphics[width=.8\linewidth]{figures/proof-theorem1-and.pdf}
%   \caption{Illustration of the $\land$ case in Proof of Theorem~\ref{theorem:completeness}}
%   \label{fig:proof-completeness-and}
% \end{figure}
% By the induction hypothesis, since $K$ satisfies $Q_1$ and $Q_2$ with coverage $\cov_1$ and $\cov_2$ respectively, there are a c-instance $J_1$ for $Q_1$ with coverage $\cov_1' \supseteq \cov_1$ and a c-instance $J_2$ for $Q_2$ with coverage $\cov_2' \supseteq \cov_2$ in the results of Algorithm~\ref{alg:rd-tree-chase-main}, and both $J_1$ and $J_2$ c-homomorphically map to $K$ under $\assignment_1$ and $\assignment_2$ respectively.
% % \amir{But $K$ can be satisfiable without $J_1$/$J_2$ being satisfiable, right? ($K$ is always satisfied because its grounded)}. 
% We next show that there is are two mappings between $J_1$ and $J_2$ to $K$ respectively, such that their union maps $J_1 \cup J_2$ to $K$. 

% Because $K$ satisfies $Q=Q_1 \land Q_2$, there exists a homomorphism $h_0$ that maps free variables in $Q_1 \land Q_2$ to values in $K$, such that $K$ satisifies $Q_1 \land Q_2$ under $h_0$. In particular, $K$ satisfies $Q_1$ and $Q_2$ so the induction hypothesis can be used. 
% Hence, we have $h_1 = h_0|_{vars(Q_1)}$ that maps the free variables in $Q_1$ to values in $K$, and $h_2 = h_0|_{vars(Q_2)}$ maps the free variables in $Q_2$ to values in $K$.
% We show that we can construct c-homomorphsims $\assignment_1$ and $\assignment_2$ that have no conflicts. Suppose $f_1$ and $f_2$ are the mappings from free variables in $Q_1$ and $Q_2$ to variables in $J_1$ and $J_2$ respectively, as initialized in Algorithm~\ref{alg:rd-tree-chase-main} to be identity functions. Hence for $Q_1$ we have $\assignment_1 = h_1 \circ f_1^{-1}$ to be a c-homomorphism from $J_1$ to $K$ (since the algorithm assigns fresh variables to all free variables in $J_1$ in lines \ref{l:iter-free}--\ref{l:add-fresh}, $f_1$ is bijective and therefore $f_1^{-1}$ is a mapping from $J_1$ to free variables in $Q_1$). For $Q_2$, we build two mappings 
% %$h_2^{**}: x \to h_2^*(x)$ 
% %$h_2^{**-1}: h_2^*(x) \to x$
% $(f_2^{*})^{-1}: Im(f_2) \to FreeVars(Q_2)$
% by restricting the co-domain of $f_2$ to its image and an identity function $g_2: vars(J_2)\setminus image(f_2) \to vars(J_2)\setminus image(f_2)$, then we construct $f'_2 = (h_2 \circ f_2^{*-1}) \cup g_2$ maps variables in the image of $f_2$ to values in $K$ and keeps other variables in $J_2$ unchanged. Then the c-instance $J_2' = f'_2(J_2)$ satisfies $f_2(Q_2)$ with coverage contains $f_2(C_2)$ (we abuse $f_2$ here, i.e., only free variables in $Q_2$ are mapped to values in $K$ while other variables and constants are not changed) \amir{Did not follow this. $h_2^*(Q_2)$ is a c-instance, not a query, right?}. Again by the induction hypothesis, $J_2'$ c-homomorphically maps to $K$ under some $\assignment_2'$, then we have $\assignment_2 =  (h_2 \circ f_2^{*-1}) \cup \assignment_2'$ is a c-homomorphsim from $J_2$ to $K$. 

% Now we show that $J_1 \cup J_2$ c-homomorphically maps to $K$ and covers $Q_1 \land Q_2$ with coverage $\cov' \supseteq \cov_1 \cup \cov_2$. 
% The former is directly by Lemma~\ref{lemma:union-c-homo}: since $h_1'$ and $h_2'$ \amir{$h_1$ and $h_2$?} agree on all variables in the intersection of their domains (variables that can be mapped from the free variables), implying that $h_1$ and $h_2$ have no conflicts, therefore $J_1 \cup J_2$ c-homomorphically maps to $K$. 
% % The former is directly by the fact that $h_0$ is a c-homomorphism from $J_1$ to $K$ and $h_2 \circ h_0$ is a c-homomorphism from $J_2$ to $K$.
% % Let $\phi \in J_1 \cup J_2$ be an arbitrary relational atom, by the definition of c-homomorphism, $K$ contains $(h_2 \circ h_0)(\phi)$; let $\phi$ be the negation of an arbitrary relational atom, $K$ does not contain the relational fact of $(h_2 \circ h_0)(\phi)$; let $\phi \in J_1 \cup J_2$ be an arbitrary binary expression $x op y$, we also have the image under $h_2 \circ h_0$ of this expression $(h_2 \circ h_0)(x) op (h_2 \circ h_0)(y)$ to be True in $K$. Hence $J_1 \cup J_2$ c-homomorphically maps to $K$ under $h_2 \circ h_0$. 

% For the claim on coverage, assume $J_1 \cup J_2$ does not satisfy $Q$ with coverage $\cov' \supseteq \cov$. Since $Q_1$ has no quantifiers, $J_1 \cup J_2$ must satisfy $Q_1$ with coverage $\cov'_1 \supseteq \cov_1$ (the c-homomorphism $\assignment_1 \cup \assignment_2$ also gives an assignment for $J_1 \cup J_2$ that satisfies $Q_1$); and since $J_1 \cup J_2$ c-homomorphically maps to $K$, $J_1 \cup J_2$ is consistent, then the only case is that there is an atom $\beta \in \cov_2$ is covered by $J_2$ but not by $J_1 \cup J_2$. That is, the insertion of some atoms in $J_1$ into $J_2$ makes $\beta$ not homomorphically map to some atom in $J_2$, which is impossible \amir{Couldn't $\beta$ be a condition that has a conflict with $J_2$?}. Hence, the assumption is wrong, $J_1 \cup J_2$ satisfies $Q$ with coverage $\cov' \supseteq \cov$.
 
% If the root of $Q$ is an $\lor$ node, i.e., $Q = Q_1 \lor Q_2$ where $V|Q_1| < n$ and $V|Q_2| < n$, and then the coverage $\cov = \cov_1 \cup \cov_2$ where $\cov_1$ is a subset of leaf atoms of $Q_1$ and $\cov_2$ is a subset of leaf atoms of $Q_2$. The algorithm splits the tree into three cases, where each is rooted by a $\land$ node: (1) where no child of the root is negated, (2) where the left child is negated and (3) where the right child is negated. Then it is reduced to the above $\land$ case.

% If the root of $Q$ is an $\exists$ node: $Q = \exists x Q'(x)$ where $V|Q'| < n$, 
% it is clear that if $\cov$ is covered by some instance $K$ for $Q$, then it is also covered by $K$ for $Q'$. By the induction hypothesis, there is a c-instance $J$ outputted by Algorithm~\ref{alg:rd-tree-chase-main} for $Q'$ with coverage containing $\cov$ that c-homomorphically maps to $K$, and $J$ is also a satisfying c-instance for $Q$ with coverage containing $\cov$.

% If the root of $Q$ is an $\forall$ node: $Q = \forall x Q'(x)$ where $V|Q'| < n$, $\cov$ is covered by $K$ for $Q$ under homomorphism $\mrel$. Unlike the above $\exists$ case, for $Q'$, different subsets of $\cov$ (denoted as $\cov_1, ..., \cov_l$, where \cov = $\bigcup_{i=1}^{l}\cov_i$) are covered under different homomorphisms that map the free variable $x$ to different values $v_i$ in the domain of $x$ in $K$. 

% We show by construction that a c-instance that c-homomorphically maps to $K$ and satisfies $Q$ with coverage $\cov' \supseteq \cov$ will be outputted by Algorithm~\ref{alg:rd-tree-chase-main}.
% For each value in $K$ we create a corresponding variable to obtain a c-instance $J_0$ with an empty global condition \amir{lines?}, and denote the bijection from the variables in $J_0$ to the values in $K$ as $\assignment$ (we also abuse $\assignment$ as a homomorphism from $J_0$ to $K$, $\assignment(J_0) = K$, $\assignment^{-1}(K) = J_0$).
% Then, we initialize the c-instance $\cinstance_0$ in Algorithm~\ref{alg:rd-tree-chase-main} by setting its domains to be the same as $J_0$ \amir{lines?}. That is, when running the algorithm, instead of allowing the algorithm to create fresh variables, we skip lines \ref{alg:rd-tree-chase:line:exists-add-fresh-start}-\ref{alg:rd-tree-chase:line:exists-add-fresh-end}, \ref{alg:rd-tree-chase:line:forall-add-fresh-start}-\ref{alg:rd-tree-chase:line:forall-add-fresh-end} in Algorithm~\ref{alg:rd-tree-chase} and thus only allow it to map the quantified variables to one of the variables added in advance in $J_0$.

% For each coverage subset $\cov_i$, we define a mapping $h_i = h \cup \{x \to v_i\}$ where $x$ is the quantified variable at the root of $Q$ and value $v_i \in K.\dom(x)$, then $h_i$ maps the free variables in $Q'$ to values in $K$, i.e., $K$ satisfies $Q'$ with coverage $\cov_i$ under $h_i$.

% \begin{figure}[h]
% \centering
%  \includegraphics[width=.6\linewidth]{figures/proof-theorem1-forall.pdf}
%   \caption{Illustration of the $\forall$ case in Proof of Theorem~\ref{theorem:completeness}}
%   \label{fig:proof-completeness-forall}
% \end{figure}

% By the induction hypothesis, for each $v_i$, since the ground instance $K$ covers $Q'$ with coverage $\cov_i$ under $h_i$, there is a c-instance $J_i$ outputted by Algorithm~\ref{alg:rd-tree-chase-main} that satisfies both $Q'$ with coverage $\cov'_i \supseteq \cov_i$ and c-homomorphically maps to $K$ under some $\assignment_i$. Since $\assignment$ is a bijection, let $J'_i = \assignment^{-1}(\assignment_i(J_i))$, then $J'_i$ also covers $Q'$ with coverage $\cov'_i$ \amir{explain why $J'_i$ is different from $J_0$}. Because each $J'_i$ is mapped to a sub-instance of $K$ under $\assignment$, the union of all $J'_i$-s ($J = \bigcup_{i=1}^{l} J'_i$) c-homomorphically maps to $K$ under $\assignment$ and thus it satisfies $Q$ with coverage $\cov' \supseteq \cov$. 

% The original algorithm can find such $J = \bigcup_{i=1}^{l} J'_i$, because (1) the algorithm dynamically increases the size of each domain and will reach the same cardinality in all domains as $J_0$, and (2) each ideal $J'_i$ will be returned the algorithm (line 51-53 in Algorithm~\ref{alg:rd-tree-chase}) --- from the construction procedure above we know that the difference between each $J_i$ and $J'_i$ is that they may contain a different subset of variables in $J_0$, however, since the Algorithm~\ref{alg:rd-tree-chase} will enumerate every variable in the domain when dealing with quantified variables, every possible subset of variables in $J_0$ will be considered. Therefore, whenever there is a valid $J = \bigcup_{i=1}^{l} J'_i$, the algorithm will find it.

% % Now we show the union of all $J'_i$-s ($J = \bigcup_{i=1}^{l} J_i$) c-homomorphically maps to $K$ and satisfies $Q$ with coverage $\cov' \supseteq \cov$. First, for each $J_i$ and $h_i$, we create a new variable $x_i$ to replace the universally quantified $x$ in $Q$ (remember that free variables are directly added to the domain of the c-instances). 
% % Then, in each $J_i$, we rename all variables such that there are no shared variables in all $J_i$-s except the free variables in $Q$.
% % To do this, in $\proc{RD-Tree-Chase}$, we set the domain of $x$ to be $\{x_1, ..., x_l\}$ (changee line 44) and do not create fresh variables for $x$ (line 34-37 and line 54-60 are skipped for the domain of $x$), and rename the variables in the resulting c-instances of the recursive call of $\proc{RD-Tree-Chase}$ for each variable in the domain (line 48-53), such that there are no shared variables except the free variables in $Q$. Because all $h_i$-s are extensions of $\mrel$, by Lemma~\ref{lemma:union-c-homo}, $J$ c-homomorphically maps to $K$ under $h' = \bigcup_{i=1}^{l} h_i$.

% % For the claim on coverage, assume that for some $Q'_i$, there is an atom $\beta \in \cov_i$ not covered by $J$ but covered by $J_i$. By definition, there exists some homomorphism that maps $\beta$ to an atom in $J_i$, and such an atom still appear in $J$. 

% For cases where the syntax tree is negated, the algorithm will change the root operator accordingly ($\land$ to $\lor$, $\land$ to $\lor$, $\exists$ to $\forall$, and $\forall$ to $exists$) and change the negated flags of the root and the children. 
% \end{proof}


\mypar{Complexity}
\amir{Verify:} 
The complexity of Algorithm \ref{alg:rd-tree-chase-main} is $\Theta(3^{d \cdot |Dom|^{u + e}} \cdot |Dom|^2)$, where $d$ is the number of disjunctions, $|Dom|$ is the number of cells in the c-instance (the maximum number is $limit \cdot k \cdot \schemaOf{\rel}$ where $k$ is the number of tables in the c-instance), and $u$ ($e$) is the number of universal (existential) quantifiers. This bound is also tight. 
To explain why it is a lower bound, consider the query $\forall x_1 \ldots \forall x_m R(x_1) \lor R(x_2) \lor \ldots \lor R(x_m)$. Given this query, denoted by $Q$, Algorithm \ref{alg:rd-tree-chase-main} first generates a c-instance, where the free variables in $Q$ are mapped to fresh variables in the domain (there are no free variables in $Q$). Then, it performs a BFS using Algorithm \ref{alg:rd-tree-chase}. 
Algorithm \ref{alg:rd-tree-chase} recurses over the tree, and for each $\forall$ quantifier, it calls Algorithm \ref{alg:forall-op} that performs $|Dom|$ iterations and for each iteration, generates a tree (due to the loop in Line 5 and the recursive call in Line 7). For each tree, the algorithm iterates over the c-instances generated in Lines 9--10, resulting in the need for $|Dom|^2$ iterations. 
Then, for each $\lor$ operator, it calls Algorithm \ref{alg:or-op} that expands the subtree into $3$ trees resulting in $3^d$ trees. For each one of these trees, Algorithm \ref{alg:and-op} that performs a recursive call on the left child resulting in $|Dom|$ instances and for each of these instances, recurses on the right child (Line 5). Thus, we have $(3^{|Dom|^u})^{d} \cdot |Dom|^2$ operations. 
Since $\land$ does not expand the current number of trees and $\exists$ expands the number by $|Dom|$, the above expression is an upper bound on the number of trees as well. 


\mypar{Complexity of optimized algorithm}
The complexity of Algorithm \ref{alg:conj-tree-cons} is 
% $\mathcal{O}(3^{d} \cdot |Dom|^{u \cdot 2^limit + e})$, 
$\mathcal{O}(3^{d}\cdot |Dom|^{u + e + 2})$
where $d$ is the number of disjunctions in $Q$, $|Dom|$ is the maximum domain size, and $u$ ($e$) is the number of universal (existential) quantifiers. 
Since we only consider conjunctive trees, Algorithm \ref{alg:rd-tree-chase} always skips Line 13 and never calls Algorithm \ref{alg:or-op}. Thus, there is no extension of the original tree beyond the one done by Algorithm \ref{alg:conj-tree-cons}. 
The first factor is due to Algorithm \ref{alg:conj-tree-cons} generating $3$ trees for each $\lor$ operator. The second factor stems from the iterations over the entire domain size for each of the universal quantifiers in each conjunctive tree when Algorithm \ref{alg:or-op} is called.

==> sections/difficult_examples.tex <==
\section{Difficult Examples}
\subsection{Oct. 14}
\noindent\textbf{1. An example indicating the need of safety restriction, instantiating the free variables, and rethinking the elimination of universal quantifiers.}
\begin{Example}
Consider the beers database and the query $Q_1 = \{d_1 \ \mid \ \forall b_1 \ Likes(d_1,b_1) \implies \exists d_2 \ Likes(d_2, b_1) \land d_1 \neq d_2 \}$ that finds drinkers such that for every beer liked by the drinker, there exists another drinker who also likes the same beer. By converting the query into PDNF, we have $\{d_1 \ \mid \ \forall b_1 \exists d_2\ \big (\neg Likes(d_1,b_1) \lor (Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \}$. 

This example reveals two issues: (1) consider the first conjunction in PDNF, we have $\{d_1 \ \mid \ \forall b_1  (\neg Likes(d_1,b_1))\}$, which finds the drinkers who do not like any beer; however, this query is not safe and thus we do not know how to instantiate the database unless we know the domain of the drinker attribute is associated with the Drinker table. (2) consider the second conjunction in PDNF, we have $\{d_1 \ \mid \ \forall b_1 \exists d_2\ \big (Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \}$. By mapping the universally quantified $b_1$ to free variables or constants will not give us a valid counterexample.

Although one can argue that the query for the second conjunction above omits the fact that the predicate in the first conjunction $\neg Likes(d_1,b_1)$ is False, and thus the correct DRC should be $\{d_1 \ \mid \ \forall b_1 \exists d_2\ \big (Likes(d_1, b_1) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \}$, which addresses the issue. 
However, consider a similar query \\
$Q_2 = \{d_1 \ \mid \ \exists b Likes(d_1, b) \land \big (\forall b_1 \ Likes(d_1,b_1) \implies \exists b_2 \ Likes(d_1, b_2) \land b_1 \neq b_2 \big)\}$, we will have have the PDNF 

% \{d_1 \ \mid \ \exists b Likes(d_1, b) \land \big (\forall b_1 \ Likes(d_1,b_1) \implies \exists b_2 \ Likes(d_1, b_2) \land b_1 \neq b_2 \big)\}$

\exists _{\{b\}}\forall _{\{b1\}}\exists _{\{b2\}}(\text{Likes}(\text{d1},b)\land ((\text{Likes}(\text{d1},b2)\land b1\neq b2)\lor \neg \text{Likes}(\text{d1},b1)))

$\{d_1 \ \mid \ \exists b \forall b_1 \exists b_2\ \big (( Likes(d_1, b) \land \neg Likes(d_1,b_1)) \lor (Likes(d_1, b)\land Likes(d_1, b_2) \land b_1 \neq b_2) \big ) \}$

% $\{d_1 \ \mid \ \forall b_1 \exists b_2\ \big (\neg Likes(d_1,b_1) \lor (Likes(d_1, b_2) \land b_1 \neq b_2) \big ) \}$,
where the query built upon the first conjunction still finds the drinkers who do not like any beer and the query for the second conjunction requires the drinker likes two different beers.
If we try to map $b_1$ to $b_2$ in this case, the resulting c-instance will always be unsatisfiable, as it has only one tuple $(b_2, *)$ in Likes with the condition $b_2 \neq b_2$.
\end{Example}

Solution to the first issue: (1) as discussed earlier, we can have dummy relations for each attribute, and set up rules constructing c-tables given these dummy relations. (2) use tuple relational calculus.

Solution to the second issue: do not map universally quantified variables to existentially quantified variables, but map them to constants/free variables (not sure).

\subsection{Oct. 28}
\begin{figure*}[!h]
\raggedright
A safe query for the $Q_1 = \{d_1 \ \mid \ \forall b_1 \ \Big( Likes(d_1,b_1) \implies \exists d_2 \ Likes(d_2, b_1) \land d_1 \neq d_2 \Big)\}$above (find drinkers such that for every beer liked by the drinker, there exists another drinker who also likes the same beer:

$\{(d_1) \ \mid  \exists a_0 Drinker(d_1, a_0) \land \neg\exists b_1 \Big(Likes(d_1, b_1) \land \neg \exists d_2 \big(Likes(d_2, b_1) \land d_1 \neq d_2\big)\Big)\}$

Compare with the PNF from Mathematica:
$\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2\ \Big (Likes(d_1, b_0) \land \big(\neg Likes(d_1,b_1) \lor (Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \Big)\}$

PDNF:
$\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2\ \Big (\big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \big) \lor \big( Likes(d_1,b_0) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \Big)\}$

Convert to disjunction:
$\{d_1 \ \mid \ \exists b_0 \forall b_1 \big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \big) \lor \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \}$

The first part is equivalent to a safe formula $\exists b_0 Likes(d_1, b_0)  \land \neg\exists b_1Likes(d_1,b_1) $ .

While the second part is not safe as neither of $b_1$ and $d_1$ is limited: $\exists b_0 Likes(d_1,b_0) \land\neg\exists b_1 \neg\exists d_2 \big(  Likes(d_2, b_1) \land d_1 \neq d_2 \big )$

Option1: record the positive formula for $b_1$ and $d_1$, which is $Likes(d_1, b_1)$; add it to the conjunction: $\exists b_0 Likes(d_1,b_0) \land\neg\exists b_1 \bigg(Likes(d_1, b_1) \land \neg\exists d_2 \big(  Likes(d_2, b_1) \land d_1 \neq d_2 \big )\bigg)$, which goes back to the original formula :(

%Option2: Relax the safety constraint. Observe that in the second part, $\forall b_1$ is not followed by a predicate of $b_1$ ($Likes(d_2, b_1)$ is in the formula of $\exists  d_2$), so we have to add a predicate of $b_1$ without $d_2$:
%$\exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_1, b_1) \land  Likes(d_2, b_1) \land d_1 \neq d_2 \big ) $
Option2: more careful conversion to PDNF: For a disjunctive sub-formula $P_1 \lor P_2 \lor ... \lor P_m$, convert it into $(P_1 \land \neg P_2 \land ... \neg P_m) \lor (P_2 \land \neg P_1 ... \land \neg P_m) \lor ... \lor (P_m \land \neg P_1 ... \land \neg  P_{m-1})$

$\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2\ \Big (Likes(d_1, b_0) \land \big(\neg Likes(d_1,b_1) \land \neg(Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \\ \lor (Likes(d_2, b_1) \land d_1 \neq d_2 \land Likes(d_1,b_1)) \big ) \Big)\}$

$\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2 \big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \land d_1 = d_2\big) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_1, b_1) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land \neg Likes(d_1, b_1) \land \neg Likes(d_2, b_1)\big ) \}$ 

The first and the third cases will lead to UNSAT results.

\\

For the query $Q_2$ above, which finds drinkers who likes two different beers (in a overcomplex way), we can do the same trick: 

$Q_2 = \{d_1 \ \mid \ \exists b Likes(d_1, b) \land \big (\forall b_1 \ Likes(d_1,b_1) \implies \exists b_2 \ Likes(d_1, b_2) \land b_1 \neq b_2 \big)\}$, we will have have the PDNF 

$\{ d_1 \mid \exists _{\{b_0\}}\forall _{\{b_1\}}\exists _{\{b_2\}}(\text{Likes}(d_1,b_0)\land ((\text{Likes}(d_1,b_2)\land b_1\neq b_2)\lor \neg \text{Likes}(d_1,b_1))) \}$

$\{ d_1 \mid \exists _{\{b_0\}}\forall _{\{b_1\}}\exists _{\{b_2\}}(\text{Likes}(d_1,b_0)\land ((\text{Likes}(d_1,b_2)\land b_1\neq b_2 \land Likes(d_1, b_1))\lor (\neg \text{Likes}(d_1,b_1) \land \neq(\text{Likes}(d_1,b_2)\land b_1\neq b_2)))) \}$

$\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2 \big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \land d_1 = d_2\big) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_1, b_1) \land Likes(d_1, b_2) \land b_1 \neq b_2 \big ) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land \neg Likes(d_1, b_1) \land \neg Likes(d_1, b_2)\big ) \}$ 
Again the first and the third cases will lead to UNSAT results.

\end{figure*}

\begin{figure*}[!h]
\raggedright
Consider again the question: For each beer liked by any drinker with the first name Eve, find the bars that serve this beer at the non-lowest price.

Standard query $Q_1$: 
\begin{align*}
\projection_{beer1, bar1} &((\selection_{drinker LIKE  'Eve\ \%'} likes) \join_{beer = beer1} ( \\
    &\rename_{bar1, beer1, price1} Serves \join_{beer1 = beer2 \land  price1>price2} \\
    &\rename_{bar2, beer2, price2} Serves));
\end{align*}

Wrong query $Q_2$: 
\begin{align*}
\projection_{beer1, bar1} &((\selection_{drinker LIKE  'Eve\%'} likes) \join_{beer = beer1} ( \\
    &\rename_{bar1, beer1, price1} Serves \join_{beer1 = beer2 \land  price1 \geq price2  \land bar1 \neq bar2} \\
    &\rename_{bar2, beer2, price2} Serves));
\end{align*}

Similarly, the DRC of $Q_1$:
\begin{align*}
Q_1=\{(x_1, b_1) & \ \mid \ \\
\exists d_1, p_1 &( \\
\exists &x_2, p_2 ( Serves(x_1, b_1, p_1) \land Likes(d_1, b_1) \land d_1 \ LIKE \ 'Eve \ \%' \land Serves(x_2, b_1, p_2) \land p_1 > p_2) \}
\end{align*}

DRC of $Q_2$:
\begin{align*}
Q_2=\{(x_1, b_1) & \ \mid \ \\
\exists d_1, p_1 &( \\
\exists &x_2, p_2 ( Serves(x_1, b_1, p_1) \land Likes(d_1, b_1) \land d_1 \ LIKE \ 'Eve\%' \land Serves(x_2, b_1, p_2) \land p_1 \geq p_2 \land x_1 \neq x_2) \}
\end{align*}


DRC of $Q_2-Q_1$ ($x_1$ and $b_1$ are quantifier-free variables):
\begin{align*}
Q_2-Q_1=\{(x_1, B_1) & \ \mid \ \\
\exists d_1, p_1, x_2, p_2 &\Big(\forall x_3, p_3, d_2, p_4 \big(\\
Serves&(x_1, b_1, p_1) \land Likes(d_1, b_1) \land d_1 \ LIKE \ 'Eve\%' \land Serves(x_2, b_1, p_2) \land p_1 \geq p_2 \land x_1 \neq x_2\\
\land(p_3 \leq p_4 &\lor !Serves(x_3, b_1, p_4) \lor  !Likes(d_2,b_1) \lor !(d_2\ LIKE \ 'Eve\ \%') \lor !Serves(x_1, b_1, p_3))\big)\Big)\} \\
=\{(x_1, B_1) & \ \mid \ \\
\exists d_1, p_1, x_2, p_2 &\Big(\forall x_3, p_3, d_2, p_4 \big(\\
Serves&(x_1, b_1, p_1) \land Likes(d_1, b_1) \land d_1 \ LIKE \ 'Eve\%' \land Serves(x_2, b_1, p_2) \land p_1 \geq p_2 \land x_1 \neq x_2\land\\
&\big(
(\text{FNEve}(\text{d2})\land \text{p3}\leq \text{p4}\land \text{Likes}(\text{d2},\text{b1})\land \text{Serves}(\text{x1},\text{b1},\text{p3})\land \text{Serves}(\text{x3},\text{b1},\text{p4})) \\
&\lor (\text{FNEve}(\text{d2})\land \text{p3}>\text{p4}\land \text{Likes}(\text{d2},\text{b1})\land \text{Serves}(\text{x1},\text{b1},\text{p3})\land \neg \text{Serves}(\text{x3},\text{b1},\text{p4}))  -- UNSAT\\
& \lor (\text{FNEve}(\text{d2})\land \text{p3}>\text{p4}\land \text{Likes}(\text{d2},\text{b1})\land \neg \text{Serves}(\text{x1},\text{b1},\text{p3})\land \text{Serves}(\text{x3},\text{b1},\text{p4}))  -- UNSAT\\
& \lor (\text{FNEve}(\text{d2})\land \text{p3}>\text{p4}\land \neg \text{Likes}(\text{d2},\text{b1})\land \text{Serves}(\text{x1},\text{b1},\text{p3})\land \text{Serves}(\text{x3},\text{b1},\text{p4}))  -- UNSAT\\
&\lor (\neg \text{FNEve}(\text{d2})\land \text{p3}>\text{p4}\land \text{Likes}(\text{d2},\text{b1})\land \text{Serves}(\text{x1},\text{b1},\text{p3})\land \text{Serves}(\text{x3},\text{b1},\text{p4}))
\big)
\end{align*}


\end{figure*}


==> sections/disjunctive_tree.tex <==
\section{A Sound and Complete Solution}\label{sec:disjunct}
\amir{This section is very technical. Maybe we can build it differently: give the high-level intuition for the algorithm and the handling of each connective/quantifier and then just give the details of algorithms 1,2 and the characterization?}
% {\bf Outline of this section:}
% \begin{enumerate}
%     \item Detail the chase procedure for handling disjunction
%     \item Proofs for soundness and completeness $+$ complexity
%     \item Detail the post-processing step for obtaining minimal c-instances
%     \item Discussion on for which class of queries the algorithm is guaranteed to terminate
% \end{enumerate}



In this section we show how to compute satisfying c-instances for a DRC query $Q$. We first transform the syntax tree of the query $Q$ into a right-deep tree (a DRC syntax tree in which quantifier nodes can only appear at the root or be the right child of a node \sr{how can a quantifier be a right child? is not it a unique child?}), define a chase-like procedure called RD-chase, and then show that the procedure is sound and complete, i.e., the result of a finite RD-chase is a set of satisfying c-instances and is a universal solution. 

% \subsection{Query Syntax Tree}

% \begin{Definition}[Syntax Tree of Query]
% \amir{Not sure this is needed for the model part. Maybe just for the algo.}
% A syntax tree of a query $Q$ is \sout{a binary} tree \red{for the FOL formula $P_Q$} satisfying the following rules:
% \begin{enumerate}
%     \item \red{Each leaf node is a DRC atom;} \sout{either a DRC atom or its negation;} DRC atoms only appear in leaf nodes.
%     \item Each internal node is either a quantifier with a single variable (e.g., $\forall x$ and $\exists x$) with a single child, or a connective ($\land$ and $\lor$) with two children
%     \item \sout{Each quantifier node has only one child; each connective node has two children.} %\SR{negation has one}
%     % \item For each node with two children, if the sub-tree rooted at its left child contains universal quantifiers, then the sub-tree rooted at its right child must also contain universal quantifiers.
%     \item \red{The negation operator ($\neg$), rather than being a node in the tree, is assumed to be a {\bf flag} on a subtree, which can also be the entire tree or the leaves Other than the leaves.}
% \end{enumerate}
% % Only the entire tree can be negated. In this case, the negation operator ($\neg$) is applied over the entire tree, rather than being a node in the tree. 
% \end{Definition}

% \red{Given a DRC query $Q$, we can have a unique syntax tree following the order of quantifiers in $Q$ (e.g., for $\exists x \exists y$, $\exists y$ appears as the child of $\exists x$, and a fixed order of commutative connectives or with appropriate parentheses, e.g., $(p_1 \vee p_2 \vee p_3)$ is always assumed to be $((p_1 \vee p_2) \vee p_3)$. However, two equivalent DRC queries may have different syntax trees.}\sr{check}
% \red{The syntax tree for the query $\qcorrect - \qincorrect$ from Figure~\ref{fig:diff-query} is shown in Figure \ref{fig:syntax-tree} (to save space, we put multiple quantifiers with variables in the same node). \sr{TODO}. The special treatment of the negation operator $\neg$ is for the sake of convenience in our algorithms. }

% \sout{In the definition above, we do not have explicit negation in the tree, but rather a flag representing a negated tree/atom. 
% Note that a given DRC query maps to a unique syntax tree. 
% Note that the tree ignores output variables and considers only the FOL formula $\aFOL_Q$. % $\aFOL(x_1, ... x_{\folarity})$ part of the query. 

% However, converting the query formula to an equivalent logical formula may result in a different syntax tree, e.g., converting an arbitrary formula to Prenex Normal Form, (i.e., all quantifiers are at the beginning of the formula) changes the structure of the formula and thus the structure of the tree, despite being logically equivalent. }


% \begin{figure}[htb]
% \begin{minipage}{1.0\linewidth}
%     \centering
%     % \begin{tikzpicture}[scale=.8,
%     % level 1/.style={level distance=0.5cm, sibling distance=-10mm},
%     % level 2/.style={sibling distance=3mm}, level distance=0.6cm, 
%     % level 3/.style={level distance=0.5cm},
%     % level 4/.style={level distance=0.2cm, sibling distance=-10mm},
%     % snode/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=blue!20},
%     % logic/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=red!70}]
%     % \Tree
%     % [.\node[logic] {$\boldsymbol{\cdot}$}; \node[snode] {TAU};
%     % [.\node[logic] {$\boldsymbol{+}$};
%     % [.\node[logic] {$\boldsymbol{\cdot}$}; \node[snode] {Slava N.}; \node[snode] {OASSIS}; \node[snode] {2014}; \node[snode] {SIGMOD};]
%     % [.\node[logic] {$\boldsymbol{\cdot}$}; \node[snode] {Tova M.}; [\qroof{sub-circuit}. ] ]
%     % ]
%     % ]
%     % \end{tikzpicture}
%     % \caption{\amir{Update to the syntax tree in Example 1}} \label{fig:syntax-tree}
%         \begin{tikzpicture}[%grow=right,
%         scale=.8,
%     level 1/.style={level distance=0.6cm, sibling distance=-10mm},
%     level 2/.style={sibling distance=-10mm, level distance=0.6cm}, 
%     level 3/.style={level distance=0.6cm, sibling distance=-10mm},
%     level 4/.style={level distance=0.6cm, sibling distance=3mm},
%     level 5/.style={level distance=0.6cm, sibling distance=3mm},
%     snode/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=blue!20},
%     logic/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=red!70}]
%     \Tree
%     [.\node[logic] {$\boldsymbol{\exists {d_1, p_1}}$}; 
%         [.\node[logic] {$\boldsymbol{\land}$}; 
%             [.\node[logic] {$\boldsymbol{\land}$}; 
%                 [.\node[logic] {$\boldsymbol{\land}$}; \node[snode]{$Likes(d_1, b_1)$}; \node[snode]{$d_1$ LIKE 'Eve\%'};]
%                 \node[snode] {$Serves(x_1, b_1, p_1)$};]
%             [.\node[logic] {$\boldsymbol{\exists {x_2, p_2}}$};
%                 [.\node[logic] {$\boldsymbol{\land}$}; \node[snode] {$Serves(x_2, b_1, p_2)$}; \node[snode] {$p_1 > p_2$};
%                 ]
%             ]
%         ]
%     ]
%     \end{tikzpicture}
    
    
%     \begin{tikzpicture}[%grow=right,
%         scale=.8,
%     level 1/.style={level distance=0.6cm, sibling distance=-10mm},
%     level 2/.style={sibling distance=-10mm, level distance=0.6cm}, 
%     level 3/.style={level distance=0.6cm, sibling distance=-10mm},
%     level 4/.style={level distance=0.6cm, sibling distance=3mm},
%     level 5/.style={level distance=0.6cm, sibling distance=3mm},
%     level 6/.style={level distance=0.6cm, sibling distance=3mm},
%     snode/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=blue!20},
%     logic/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=red!70}]
%     \Tree
%     [.\node[logic] {$\boldsymbol{\exists {d_1, p_1}}$}; 
%         [.\node[logic] {$\boldsymbol{\land}$}; 
%             [.\node[logic] {$\boldsymbol{\land}$}; 
%                 [.\node[logic] {$\boldsymbol{\land}$}; \node[snode]{$Likes(d_1, b_1)$}; \node[snode]{$d_1$ LIKE 'Eve \%'};]
%                 \node[snode] {$Serves(x_1, b_1, p_1)$};]
%             [.\node[logic] {$\boldsymbol{\forall {x_2, p_2}}$};
%                 [.\node[logic] {$\boldsymbol{\lor}$};
%                     \node[snode] {$\neg Serves(x_2, b_1, p_2)$}; \node[snode] {$p_1 \geq p_2$};
%                 ]
%             ]
%         ]
%     ]
%     \end{tikzpicture}
%     \end{minipage}
%     \caption{Syntax trees of \qincorrect\ and \qcorrect\ in Example~\ref{ex:query}\sr{plz change this to $QA-QB$ with negation flags as figure*}} \label{fig:syntax-tree}
    
    
% \end{figure}
% \begin{figure*}[htb]
%     \begin{minipage}{1.0\linewidth}
%      \centering
%     \begin{tikzpicture}[%grow=right,
%         scale=.8,
%     level 1/.style={level distance=0.6cm, sibling distance=3mm},
%     level 2/.style={sibling distance=-10mm, level distance=0.6cm}, 
%     level 3/.style={level distance=0.8cm,sibling distance=-15mm},
%     level 4/.style={level distance=1.0cm,sibling distance=-3mm},
%     level 5/.style={level distance=1.0cm, sibling distance=0mm},
%     % level 6/.style={level distance=1.0cm, sibling distance=0mm},
%     snode/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=blue!20},
%     coverednode/.style = {shape=rectangle, rounded corners, draw, align=center, top color=applegreen, bottom color=applegreen!20},
%     logic/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=red!70}]
%     \Tree
%     [.\node[logic] {$\boldsymbol{\land}$}; 
%         [.\node[logic] {$\boldsymbol{\exists {d_1, p_1}}$}; 
%             [.\node[logic] {$\boldsymbol{\land}$}; 
%                 [.\node[logic] {$\boldsymbol{\land}$}; 
%                     [.\node[logic] {$\boldsymbol{\land}$}; \node[coverednode]{$Likes(d_1, b_1)$}; \node[coverednode]{$d_1$ LIKE 'Eve\%'};]
%                     \node[coverednode,xshift=0mm] {$Serves(x_1, b_1, p_1)$};]
%                 [.\node[logic] {$\boldsymbol{\exists {x_2, p_2}}$};
%                     [.\node[logic] {$\boldsymbol{\land}$}; \node[coverednode] {$Serves(x_2, b_1, p_2)$}; \node[coverednode] {$p_1 > p_2$};
%                     ]
%                 ]
%             ]
%         ]
%         [.\node[logic,xshift=0mm] {$\boldsymbol{\forall {d_2, p_3}}$}; 
%             [.\node[logic,xshift=0mm] {$\boldsymbol{\lor}$}; 
%                 [.\node[logic, xshift=0mm] {$\boldsymbol{\lor}$}; 
%                     [.\node[logic] {$\boldsymbol{\lor}$}; \node[snode]{$\neg Likes(d_2, b_1)$}; \node[snode]{$\neg$($d_2$ LIKE 'Eve \%')};]
%                     \node[coverednode,xshift=0mm] {$\neg Serves(x_1, b_1, p_3)$};]
%                 [.\node[logic,xshift=0mm] {$\boldsymbol{\exists {x_3, p_4}}$};
%                     [.\node[logic, xshift=0mm] {$\boldsymbol{\land}$};
%                         \node[coverednode,xshift=0mm] {$Serves(x_3, b_1, p_4)$}; \node[coverednode,xshift=0mm] {$p_3 < p_4$};
%                     ]
%                 ]
%             ]
%         ]
%     ]
%     \end{tikzpicture}
%     \caption{Syntax tree of $\qincorrect-\qcorrect$ in Example~\ref{ex:query}. Atoms covered by the c-instance in Figure~\ref{fig:c-instance} are colored in green} \label{fig:syntax-tree-minus}
% \end{minipage}
% \end{figure*}


% \begin{Example}
% % \amir{add running example of the syntax tree of the query in the previous example}
% \sout{Figure \ref{fig:syntax-tree} depicts the syntax trees of the two queries in Example \ref{ex:query} where red nodes are logical quantifiers and connectors and blue nodes are atoms. The top tree is for $\qincorrect$ while the bottom tree is for \qcorrect, where some of the differences are in the $Serves(x_2, b_1, p_2)$ atom which is negated in the bottom tree, and the $p_1 > p_2$ which is changed to $p_1 \geq p_2$ in the bottom tree. The root of the top tree contains two variables for brevity. 
% The formal representation is $\exists d_1$ and $\exists p_1$ as its child. 
% \resolved{\sr{does it affect the algo execution? otherwise better to draw the tree precisely.} \amir{This is just to save space}}}
% \end{Example}


\subsection{Right Deep Tree Chase}


\amir{Check if removing the Right Deep requirement is possible and if the completeness proof still works}
We can convert any syntax tree of a DRC query to a right deep tree (RD-tree) when 
no variables are reused in the query formula, which can be guaranteed through renaming.  \sr{need an example} To deal with arbitrary FOL formulae with negations, we define a chase procedure, call $RD-Chase$.
Unlike the classic chase algorithm that directly adds or modifies tuples, our procedure converts the query into conjunction of atoms and then adds relational atoms and conditions from the conjunction. Since there can be multiple quantifiers in the syntax tree, our procedure recursively calls itself on the subtrees.
Our algorithm is inspired by the chase procedure which was originally proposed in the context Data Exchange problem \cite{FaginKMP03,FaginKP03}. 

% \begin{Definition}[RD-Chase Step]
% \amir{Why do we need this def if have the algorithms?}
% Let $J$ be a c-instance, we construct a c-instance $J'$ by adding relational atoms and conditions to $J$. This is done by traversing the right deep tree $Q$ and build the conjunction of atoms and atomic conditions $\phi$. Since the tree is right deep, we traverse the tree through right edges and stop when reaching a node where there is no quantifiers in its children.

% Let %$Q: \forall x (A(x) \land \exists y (B(x, y) \lor \forall z (C(z) \land D(x, z))))$
% $Q$ be the current tree,
% $\phi$ be the conjunction of relational atoms or atomic conditions from $Q$. Let $h$ be a c-homomorphism from $\phi$ to $J$. $\phi$ can be added to $J$ with c-homomorphism $h$ if there is an atom or atomic condition $\beta$ in $\phi$ such that $h(\beta) \notin J$. If $\beta$ is a relational atom $\rel(                          x_1, ... , x_\relarity)$, we add $\rel(h(x_1), ... , h(x_\relarity))$  to $\rel$ in $J$; if $\beta$ is an atomic condition $\neg\rel(x_1, ... , x_\relarity)$ or $x~op~y$, we add $\neg \rel(h(x_1), ... , h(x_\relarity))$ or $h(x)~op~h(y)$ to the condition in $J$. Hence we obtain $J'$ from $J$.

% Then we check the consistency of $J'$: (1) If $J'$ is not consistent, we say the result of adding $\phi$ under $h$ on $J$ is failure and denote $J \xrightarrow[]{\phi, h} \bot$, and (2) otherwise we say the result of adding $\phi$ under $h$ on $J$ is $J'$, and denote $J \xrightarrow[]{\phi, h} J'$.
% \end{Definition}

%Since the disjunction in the query tree leads to multiple ways to convert the tree into conjunction, a

Algorithm~\ref{alg:rd-tree-chase-main} and Algorithm~\ref{alg:rd-tree-chase} are the main body of our procedure. The procedure starts by calling $\proc{RD-Tree-Chase-Naive}$ on the schema $\schemaOf{\rel}$, the entire query $Q$, an empty instance $I_0$, and an empty mapping $h_0$. The size limit sets the maximum number of tuples allowed in the c-instance and is meant to avoid infinite running time of the algorithm. In practice, it is only set when we want to limit the runtime.



\begin{algorithm}[h]\caption{RD-Tree-Chase-Naive}\label{alg:rd-tree-chase-main}
{\small
\begin{codebox}
\algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
$Q$: a DRC query; $I_0$: a c-instance of schema of $\schemaOf{\rel}$;\\
$h_0$: a mapping from free variables in $Q$ to variables/constants in the c-instance;\\
$limit$: the maximum number of tuples and conditions in the c-instance;\\
\algorithmicensure A list of satisfying c-instances for $Q$. \\
\Procname{$\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q, h_0, I_0, limit)$}
\li res $\gets []$, queue $\gets $ an empty queue
% \li $I_0 \gets$ an empty c-instance of schema of  $\schemaOf{\rel}$
\li \For $x \in FreeVar(Q)$\label{l:iter-free}
    \Do
        \li \If $x \notin h_0.domain$
        \Then
          \li Create a fresh variable $x'$ in the domain of $x$
          \li $I_0.domain(x) \gets I_0.domain(x) \cup \{x'\}$
          \li $h_0 \gets h_0 \cup \{x \to  x'\}$\label{l:add-fresh}
        \End
    \End
\li queue.push($I_0$)
\li visited $\gets \emptyset$
\li \While $\neg$ queue.isEmpty()
    \Do
        \li $I \gets $ queue.pop()
        \li \If I $\in$ visited or $|I| > limit$
        \li \Then continue
        \End
        \li visited $\gets $ visited $\cup \{I\}$
        \li \If $\proc{Tree-SAT}(Q, I, \emptyset)$ and $Rep(I) \neq \emptyset$
            \Then  
                \li $res.append(I)$
                \li continue
            \End
        \li $Ilist \gets \proc{RD-Tree-Chase}(\schemaOf{\rel}, Q, I, h_0)$
        \li \For $J \in Ilist$
        \Do
           \li \If $J \neq \bot$ and $|J| \leq limit$ and $J \notin visited$
            \Then
                \li queue.push($J$)
            \End
        \End
    \End
\li \Return $res$
\end{codebox}
}
\end{algorithm}

\mypar{Breadth-first search}
\amir{maybe first give intuition for why does it makes sense to perform BFS? What is different between ``layers'' of instances in the queue?}
First, to initialize the instance $I_0$ and the mapping $h_0$ from free variables in the query to labeled nulls and constants in $I_0$, for each free variable $x$ in $Q$, Algorithm~\ref{alg:rd-tree-chase-main} will create a new labeled null and add it to the domain of $x$ in $I_0$ and update $h_0$ (Line 2-6). Then, the algorithm runs in a Breadth-first search manner: $I_0$ is initially added to the empty queue; every time the algorithm takes the head of the queue, checks whether the instance has already been generated and its size does not exceeds $limit$ (Line 11). 
The purpose of the $limit$ parameter is to ensure the halting of the algorithm, since, as we have showed in Section \ref{sec:model}, finding a universal solution is undecidable. 
% \sr{limit should be explained} 
This procedure for checking $I \in visited$ is done by first comparing the properties of the c-instance and filtering out candidates (number of tuples, size of conditions etc.), and then checking all mappings to previously generated c-instances. Due to the filtering step, this process is fast in practice \amir{do we have an experiment here?}. 
It also checks whether it is a valid solution (Line 14) or we still needs to run the recursive procedure on it (Line 17); and then the resulting instances are added to the queue (Line 18-20).

\newcounter{lastcodelinenumber}

\newif\ifcodeboxcontinued


\xapptocmd{\endcodebox}{%
  \setcounter{lastcodelinenumber}{\value{codelinenumber}}%
  \global\codeboxcontinuedfalse
}{}{}
\xapptocmd{\codebox}{%
  \ifcodeboxcontinued
  \setcounter{codelinenumber}{\value{lastcodelinenumber}}%
  \fi
}{}{}
\newcommand\continuecodebox{\global\codeboxcontinuedtrue}
%\SetKwProg{MyStruct}{Struct}{ contains}{end}


\begin{algorithm}[h]\caption{RD-Tree-Chase}\label{alg:rd-tree-chase}
  \centering
{\small
\begin{codebox}
\algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
$Q$: a right deep syntax tree of a DRC query; \\
$I$: current c-instance; \\
$f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
%$\phi$: current conjunction of literals.\\
\algorithmicensure a list of c-instances\\
  \Procname{$\proc{RD-Tree-Chase}(\schemaOf{\rel}, Q, I, f)$}
  \li res $\gets []$
  \li \If there is no quantifier in $Q$
  \Then
    \li $L \gets \proc{tree-to-conj}(Q)$
    \li \For $\psi \in L$
    \Do
        \li $J \gets \proc{Add-to-Ins}(\schemaOf{\rel}, I, f(\psi))$
        \li \If $J$ is consistent
            \Then \li res.append($J$)
        \End
    \End
%   \li \ElseIf Q.negated
%   \Then
%         \li res $\gets \proc{Handle-Negation}(Q, \proc{RD-Tree-Chase})$
  \li \ElseIf Q.root.operator $\in \{\land\}$
  \Then
        \li res $\gets \proc{Handle-And-Operator}(\schemaOf{\rel}, Q, I, f)$
    % \End
\li \ElseIf Q.root.operator $\in \{\lor\}$
  \Then
        \li res $\gets \proc{Handle-Or-Operator}(\schemaOf{\rel}, Q, I, f)$
    % \End
  \li \ElseIf Q.root.operator $\in \{\exists\}$
  \Then
        \li res $\gets \proc{Handle-Existential-Operator}(\schemaOf{\rel}, Q, I, f)$
  \li \ElseIf Q.root.operator $\in \{\forall\}$
  \Then 
        \li res $\gets \proc{Handle-Universal-Operator}(\schemaOf{\rel}, Q, I, f)$
    \End\label{alg:rd-tree-chase:line:forall-add-fresh-end}
\End
\li \Return res

\end{codebox}
}
\end{algorithm}

\sr{change vars in cinstances to labeled nulls and fix symbols}
\mypar{Recursive generation of c-instances}
The recursive procedure Algorithm~\ref{alg:rd-tree-chase} handles the query according to its root operators. 
It gets as input the schema of the relational database $\schemaOf{\rel}$, a right deep syntax tree of a DRC query $Q$, the current c-instance $I$,
the current mapping from $h: \varset_Q \cup \constset_Q \to \lnset_I \cup \constset_I$. 
For the case where the query has no quantifiers (Line 2-7), the algorithm converts the syntax tree into a list of conjunction of atoms/atomic conditions, and then an instance is created for each conjunction under the mapping $h$. 
If $Q$ is negated, the algorithm calls Algorithm \ref{alg:negation} that percolates the negation to the leaves (Lines \amir{?}). 
After that, that algorithm proceeds according to the four logical symbols that can appear in the root of $Q$ where each one is handled by a dedicated sub-method (Lines \amir{?}).
We next describe each of the sub-methods that are used the recursive procedure described by Algorithm~\ref{alg:rd-tree-chase}. Each sub-method gets as input the same input as Algorithm \ref{alg:rd-tree-chase} and outputs a list of c-instances. Note that there are mutual calls from Algorithm~\ref{alg:rd-tree-chase} to the sub-methods and vice-versa.
% the schema of the relational database $\schemaOf{\rel}$, a right deep syntax tree of a DRC query $Q$, the current c-instance $I$,
% the current homomorphism from $f: var(Q) \cup cons(Q) \to var(I) \cup cons(I)$, and the current conjunction of literals $\phi$. 
% Its output is a list of c-instances. Note that there are mutual calls from Algorithm~\ref{alg:rd-tree-chase} to the sub-methods and vice-versa.


% \begin{algorithm}[h]\caption{Handle-Negation}\label{alg:negation}
%   \centering
% {\small
% \begin{codebox}
%   \Procname{$\proc{Handle-Neg}(Q, Alg)$}
    
%     \li neg-counterpart $\gets$ Neg-Op-Counterpart(Q.root.operator)
%     \li Q.root.operator $\gets $ neg-counterpart, Q.negated $\gets$ false
%     \li \If Q.root.operator $\in \{\lor, \land\}$
%     \Then
        
%         \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated
%         \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
%     \End
    
%     \li \If Q.root.operator $\in \{\exists, \forall\}$
%     \Then
%         % \li Q.root.operator $\gets$ neg-counterpart, Q.negated $\gets$ false
%         \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
%     \End
%     % \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%     \li \Return $\proc{Alg}($\schemaOf{\rel}$, Q, I, f)$
% \end{codebox}
% }
% \end{algorithm}

% \mypar{Handling negation}
% We first consider the case where the syntax tree is negated. The procedure in this case is described in Algorithm \ref{alg:negation}. Given $Q$ that is negated, the algorithm first computes the negated counterpart of the rood operator (e.g., for $\land$ it is $\lor$ and for $\exists$ it is $\forall$). Then, the root operator is updated and the negation flag is removed from the root. The algorithm continues by examining two cases; if the root operator is $\land$ or $\lor$, it will negate its two subtrees and otherwise, there is only one subtree to negate. Finally, there is a call to Algorithm \ref{alg:rd-tree-chase} with the updated, non-negated root.


\begin{algorithm}[h]\caption{Handle-And-Operator}\label{alg:and-op}
  \centering
{\small
% \begin{codebox}
% % \algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
% % $Q$: a right deep syntax tree of a DRC query; \\
% % $I$: current c-instance; \\
% % $f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
% % $\phi$: current conjunction of literals.\\
% % \algorithmicensure a list of c-instances\\
%   \Procname{$\proc{Handle-And}(\schemaOf{\rel}, Q, I, f)$}
  
%     % \li \If Q.negated
%     % \Then
%     %     % \li Q.root.operator $\gets \lor$, Q.negated $\gets$ false
%     %     % \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated 
%     %     % \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
%     %     % \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%     %     \li \Return $\proc{Handle-Negation}(\schemaOf{\rel}, Q, I, f,\proc{RD-Tree-Chase})$
%     % \End
%     \li lres $\gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.lchild, I, f, limit)$
%     \li rres $\gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.rchild, I, f, limit)$
%     \li \For $J_1 \in lres$
%     \Do
%         \li \For $J_2 \in rres$
%         \Do
%           \li $K \gets \proc{MergeIns}(J_1, J_2)$
%           \li \If $K$ is consistent
%             \Then
%               \li res.append($K$)
%             \End
%         \End
%     \End
% \li \Return $res$
% \end{codebox}

\begin{codebox}
  \Procname{$\proc{Handle-And}(\schemaOf{\rel}, Q, I, f)$}
  
    \li lres $\gets \proc{RD-Tree-Chase}(\schemaOf{\rel}, Q.root.lchild, I, f, limit)$
    \li \For $J_1 \in lres$
    \Do
        \li \If $J_1$ is not consistent
        \Then
            \li Continue
        \End
        \li rres $\gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.rchild, J_1, f, limit)$
        \li \For $K \in rres$ 
        \Do
            \li \If $K$ is consistent
            \Then
              \li res.append($K$)
            \End
        \End
    \End
\li \Return $res$
\end{codebox}
}
\end{algorithm}

\mypar{Handling conjunction}
If the root node is $\land$, Algorithm~\ref{alg:rd-tree-chase-main} is calls Algorithm \ref{alg:and-op} which recursively calls Algorithm \ref{alg:rd-tree-chase} on both children of the root (Lines \amir{?}), and then every pair of solutions to each child is merged into one instance by unioning every solution to the left subtree with every solution to the right subtree (Lines \amir{?}), and adding the consistent instances to the list of c-instances (Lines \amir{?}). \amir{explain how consistency is checked}
Note that although the homomorphism $f$ guarantees that solutions to each child map the free variables in $Q$ to the same labeled nulls in the instance, there can be newly created labeled nulls in the recursive calls and hence we have to validate the consistency of the resulting instance. 


\begin{algorithm}[h]\caption{Handle-Or-Operator}\label{alg:or-op}
  \centering
{\small
\begin{codebox}
% \algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
% $Q$: a right deep syntax tree of a DRC query; \\
% $I$: current c-instance; \\
% $f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
% $\phi$: current conjunction of literals.\\
% \algorithmicensure a list of c-instances\\
  \Procname{$\proc{Handle-Or}(\schemaOf{\rel}, Q, I, f)$}
  
%   \li \If Q.negated
%     \Then
%         % \li Q.root.operator $\gets \land$, Q.negated $\gets$ false
%         % \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated
%         % \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
%         % \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%         \li \Return $\proc{Handle-Negation}(\schemaOf{\rel}, Q, I, f,\proc{RD-Tree-Chase})$
%     \End
    % \li ConjTrees $\gets \proc{DisjTree-to-ConjTrees}(Q.root)$
    \li ConjTrees $\gets \proc{Expand-DisjTree}(Q.root)$
    \li \For $T \in ConjTrees$
    \Do
        \li res.extend($\proc{RD-Tree-Chase-Naive}($\schemaOf{\rel}$, T, I, f)$)
    \End
\li \Return $res$
\end{codebox}
}
\end{algorithm}

\mypar{Handling disjunction}
For the case where the root node is $\lor$ (Line \amir{?}), Algorithm \ref{alg:rd-tree-chase} calls Algorithm \ref{alg:or-op} which uses the procedure Expand-DisjTree to reduce the disjunctive case into three structures by replacing $Q = A \lor B$ with one of $A \land B$, $A \land \neg B$, and $\neg A \land B$ ($A$ and $B$ represent two children of the root node), since one of the three formulae must be True iff $A \lor B$ is True. Then, Algorithm \ref{alg:rd-tree-chase} is called with each of the modified trees and each set of c-instances obtained from each of the three cases is added to the result set (Lines \amir{?}). 


\begin{algorithm}[h]\caption{Handle-Existential-Operator}\label{alg:exists-op}
  \centering
{\small
\begin{codebox}
% \algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
% $Q$: a right deep syntax tree of a DRC query; \\
% $I$: current c-instance; \\
% $f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
% $\phi$: current conjunction of literals.\\
% \algorithmicensure a list of c-instances\\
  \Procname{$\proc{Handle-Existential}(\schemaOf{\rel}, Q, I, f)$}
  
    % \li \If Q.negated
    % \Then
    %     % \li Q.root.operator $\gets \forall$, Q.negated $\gets$ false
    %     % \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
    %     % \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
    %     \li \Return $\proc{Handle-Negation}(\schemaOf{\rel}, Q, I, f,\proc{RD-Tree-Chase})$
    % \End
    \li \For $x \in I.domain(Q.root.variable)$
    \Do
        \li $g \gets f \cup \{Q.root.variable \to x\}$
        % \li res.extend($\proc{RD-Tree-Chase}(Q.root.child, I, g)$)
        \li res.extend($\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$)
    \End
    \li Create a fresh labeled null $y$ in the domain of $Q.root.variable$\label{alg:rd-tree-chase:line:exists-add-fresh-start}
    \li $g \gets f \cup \{Q.root.variable \to y\}$
    \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
    % \li res.extend($\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, f, limit)$)
    \li res.extend($\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$)\label{alg:rd-tree-chase:line:exists-add-fresh-end}
\li \Return $res$
\end{codebox}
}
\end{algorithm}


\mypar{Handling existential and universal quantifiers}
% If the root node is the quantifier $\exists$ or $\forall$, the algorithm will iterate over all labeled nulls or constants in the domain of the quantified variable (Line 35-37, 51-60) and also try to add a fresh labeled null (Line 38-41, 62-70), update the homomorphism (as the quantified variable becomes free in the subtree), and recursively call Algorithm~\ref{alg:rd-tree-chase-main}. The difference is that for the $\forall$ case, like the $\land$ case, the solutions to each different labeled null that the quantified variable maps to are merged into one instance (Line 55-60, 66-70).
If the root node is the quantifier $\exists$, Algorithm~\ref{alg:rd-tree-chase} calls Algorithm~\ref{alg:exists-op} will iterate over all labeled nulls or constants in the domain of the quantified variable (Lines \amir{?}) and also add a fresh labeled null (Line \amir{?}), update the homomorphism (as the quantified variable becomes free in the subtree), and recursively call Algorithm~\ref{alg:rd-tree-chase-main}. 
The difference in handling the universal quantifier in Algorithm \ref{alg:forall-op} (which is again called from Algorithm~\ref{alg:rd-tree-chase} when the root is a $\forall$ quantifier) is that for this case, like the $\land$ case, the solutions to each different labeled null and constant that the quantified variable is mapped to are merged into one instance (Line \amir{?}).


\begin{figure}[htb]
\begin{minipage}{1.0\linewidth}
    \centering
        \begin{tikzpicture}[%grow=right,
        scale=.8,
    level 1/.style={level distance=0.6cm, sibling distance=-10mm},
    level 2/.style={sibling distance=-10mm, level distance=0.6cm}, 
    level 3/.style={level distance=0.6cm, sibling distance=-10mm},
    level 4/.style={level distance=0.6cm, sibling distance=3mm},
    level 5/.style={level distance=0.6cm, sibling distance=3mm},
    snode/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=blue!20},
    logic/.style = {shape=rectangle, rounded corners, draw, align=center, top color=white, bottom color=red!70}]
    \Tree
    [.\node[logic] {$\boldsymbol{\exists {d_1, p_1}}$}; 
        [.\node[logic] {$\boldsymbol{\land}$}; 
            [.\node[logic] {$\boldsymbol{\land}$}; 
                [.\node[logic] {$\boldsymbol{\land}$}; \node[snode]{$Likes(d_1, b_1)$}; \node[snode]{$d_1$ LIKE 'Eve\%'};]
                \node[snode] {$Serves(x_1, b_1, p_1)$};]
            [.\node[logic] {$\boldsymbol{\exists {x_2, p_2}}$};
                [.\node[logic] {$\boldsymbol{\land}$};
                    [.\node[logic] {$\boldsymbol{\land}$}; \node[snode] {$Serves(x_2, b_1, p_2)$}; \node[snode] {$p_1 > p_2$};
                    ]
                    [.\node[logic] {$\boldsymbol{\forall {d_2, p_3}}$};
                        [.\node[snode] {...};]
                    ]
                ]
            ]
        ]
    ]
    \end{tikzpicture}
    \caption{Right deep tree of $\qincorrect-\qcorrect$ in Example~\ref{ex:query}. The rightmost sub-tree rooted at $\forall d_2, p_3$ is the same as the right branch of the tree in Figure~\ref{fig:syntax-tree-minus}}
     \label{fig:rd-tree}
\end{minipage}
\end{figure}


\mypar{Ensuring Minimality}
\amir{add procedure that compares c-instances and makes sure that each one is minimal and the final set is minimal}

\begin{Example}
We next demonstrate the operation of Algorithm \ref{alg:rd-tree-chase-main} using the query $Q-Q_0$, where $Q$ and $Q_0$ are shown in Figure~\ref{fig:queries}. The tree of $Q-Q_0$ is shown in Figure~\ref{fig:rd-tree}. Here we consider limit to be infinite, and the algorithm begins with empty $h_0$ and $I_0$.

At the beginning (line 2-6 in Algorithm~\ref{alg:rd-tree-chase-main}), for each free variable in $Q-Q_0$ ($x_1$ and $b_1$), a labeled null is created and are added to the domain of $I_0$ and then to $h_0$. Now we have $I_0.\dom(Bar.name)$ $= \{x_1\}$, $I_0.\dom(Beer.name)$ $= \{b_1\}$, $h = \{x_1 \to x_1, b_1 \to b_1\}$.

Then we add $I_0$ to the queue and start the BFS procedure. The current $I_0$ with no tuples has not been visited (line 11-13), and it does not satisfy the tree and is consistent (line 14-16), so we call procedure $\proc{RD-Tree-Chase}$.

In Algorithm~\ref{alg:rd-tree-chase}, it first goes into the $\exists$ case, i.e. Algorithm~\ref{alg:exists-op}, and since the domain of drinker names is empty, we can only create new labeled null $d_1$ and add $d_1 \to d_1$ to g (line 4-6 in Algorithm~\ref{alg:exists-op}), and do the same thing for $p_1$ when we run algorithm~\ref{alg:rd-tree-chase-main} for the next level (line 7). Then, for the conjunction node, we directly obtain c-instance from its left branch (Line 2-7 Algorithm~\ref{alg:rd-tree-chase}), which gives us a c-instance with tuples  $Likes(d_1, b_1)$ and $Serves(x_1, b_1, p_1)$ and condition $d_1 \ LIKE \ 'Eve\%'$.

For the next existential quantifier node, however, there are two options: we can either map $x_2$ to the existing labeled null $x_1$ created earlier, or we can create a new $x_2$ and add it to the domain of bar names in the instance. It is the same for $\exists p_2$. Hence, we can reach the node of $\land$ below $\exists p_2$ with four different mappings for $x_2$ and $p_2$: $\{x_2 \to x_1, p_2 \to p_1\}$, $\{x_2 \to x_1, p_2 \to p_2\}$, $\{x_2 \to x_2, p_2 \to p_1\}$, $\{x_2 \to x_2, p_2 \to p_2\}$. Again, we obtain c-instances by adding the atoms on the left branch of the $\land$ node. The resulting instances will be inconsistent if we choose mapping $p_2$ to $p_1$, because there is an atomic condition $p_1 > p_2$, which will be false if we map $p_1$ and $p_2$ to the same labeled null. 

To continue, we use the case $\{x_2 \to x_2, p_2 \to p_2\}$ to illustrate. Then we come to the $\forall d_2$ node. Note that currently we have one labeled null $d_1$ in the domain of drinker names, thus Algorithm~\ref{alg:forall-op} will try first mapping $d_2$ to $d_1$ and traverse to the next node (Line 5-7), where $\forall p_3$ would first map $p_3$ to $p_1, p_2$ one by one and goes to the $\lor$ node, where Algorithm~\ref{alg:or-op} will enumerate all three cases that convert disjunction to conjunction --- assume for $\{p_3 \to p_1\}$ we negate the right branch of $\lor$ and keep the left branch the same, then one possible conjunction under the mapping from the left branch can be $Likes(d_1, b_1)$ $\land d_2\ LIKE \ 'Eve\ \%'$ $\land Serves(x_1, b_1, p_1)$ (certainly we cannot have $\neg Likes(d_1, b_1)$ or $\neg Serves(x_1, b_1, p_1)$);
for the right branch, we transform it into $\forall x_3 \forall p_4 (\neg Serves(x_3, b_1, p_4) \lor p_3 \geq p_4)$ by calling Algorithm~\ref{alg:negation}, and we have
\begin{enumerate}
    \item $Serves(x_1, b_1, p_1) \land p_1 \geq p_1$ for $\{x_3 \to x_1, p_4 \to p_1\}$
    \item $\neg Serves(x_2, b_1, p_1) \land p_1 \geq p_1$ for $\{x_3 \to x_2, p_4 \to p_1\}$
    \item $\neg Serves(x_1, b_1, p_2) \land p_1 \geq p_2$ for $\{x_3 \to x_1, p_4 \to p_2\}$
    \item $Serves(x_2, b_1, p_2) \land p_1 \geq p_2$ for $\{x_3 \to x_2, p_4 \to p_2\}$
\end{enumerate}

For $\{p_3 \to p_2\}$  we keep both branches the same. One possible conjunction under the mapping from the left branch can be $Likes(d_1, b_1)$ $\land \neg(d_2\ LIKE \ 'Eve\ \%')$ $\land \neg Serves(x_1, b_1, p_2)$; 
for the right branch, we can map $x_3$ to $x_1$ and $p_4$ to $p_1$ and thus we get $Serves(x_1, b_1, p_1)$ $\land p_2 < p_1$. By merging the resulting instances in each $\land$ node, we can obtain the c-instance $\cinstance_1$ in Figure~\ref{fig:c-instance-2}.

\end{Example}




















\begin{algorithm}[h]\caption{Handle-Universal-Operator}\label{alg:forall-op}
  \centering
{\small
\begin{codebox}
% \algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
% $Q$: a right deep syntax tree of a DRC query; \\
% $I$: current c-instance; \\
% $f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
% $\phi$: current conjunction of literals.\\
% \algorithmicensure a list of c-instances\\
  \Procname{$\proc{Handle-Universal}(\schemaOf{\rel}, Q, I, f)$}
  
    %   \li \If Q.negated
    % \Then
    %     % \li Q.root.operator $\gets \exists$, Q.negated $\gets$ false
    %     % \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
    %     % \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
    %     \li \Return $\proc{Handle-Negation}(\schemaOf{\rel}, Q, I, f,\proc{RD-Tree-Chase})$
    % \End
    \li $Ilist \gets [I]$
    \li \If $I.domain(Q.root.variable) = \emptyset$
        \Then
            \li $res.append(I)$
            % \li $y \gets \proc{Add-Fresh-Var}(I, Q.root.variable)$
            % \li Create a fresh variable $y$ in the domain of $x$
            % \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
    \li \Else
        \li \For $x \in I.domain(Q.root.variable)$
        \Do
            \li $g \gets f \cup \{Q.root.variable \to x\}$
            \li $Ilist' \gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$
            \li $cur \gets []$
            \li \For $J_1 \in IList$
            \Do
                \li \For $J_2 \in Ilist'$
                \Do
                  \li $K \gets \proc{MergeIns}(J_1, J_2)$
                  \li \If $K$ is consistent
                    \Then
                      \li cur.append($K$)
                    \End
                \End
            \End
            \li $Ilist \gets cur$
        \End
        \li res.extend($Ilist$)
    \End
    \li Create a fresh variable $y$ in the domain of $Q.root.variable$\label{alg:rd-tree-chase:line:forall-add-fresh-start}
    \li $g \gets f \cup \{Q.root.variable \to y\}$
    \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
    % \li $Ilist' \gets []$
    % \li \For $J \in IList$
    % \Do
    %     \li $g \gets f \cup \{Q.root.variable \to x\}$
    %     \li $Ilist'.extend(\proc{RD-Tree-Chase}(Q.root.child, J, g))$ 
    % \End
    % \li res.extend($Ilist'$)
    % \li $Ilist' \gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, f, limit)$
    \li $Ilist' \gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$
    \li \For $J_1 \in IList$
    \Do
        \li \For $J_2 \in Ilist'$
        \Do
          \li $K \gets \proc{MergeIns}(J_1, J_2)$
          \li \If $K$ is consistent
            \Then
              \li res.append($K$)
            \End
        \End
    \End
\li \Return $res$
\end{codebox}
}
\end{algorithm}




\cut{
\begin{algorithm}[h]\caption{RD-Tree-Chase}\label{alg:rd-tree-chase}
  \centering
{\small
\begin{codebox}
\algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
$Q$: a right deep syntax tree of a DRC query; \\
$I$: current c-instance; \\
$f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
$\phi$: current conjunction of literals.\\
\algorithmicensure a list of c-instances\\
  \Procname{$\proc{RD-Tree-Chase}(Q, I, f, \phi)$}
  \li res $\gets []$
  \li \If there is no quantifier in $Q$
  \Then
    \li $L \gets \proc{tree-to-conj}(Q)$
    \li \For $\psi \in L$
    \Do
        \li $J \gets \proc{Add-to-Ins}(\schemaOf{\rel}, I, f(\phi \land \psi))$
        \li \If $J$ is consistent
            \Then \li res.append($J$)
        \End
    \End
  \li \ElseIf Q.root.operator $\in \{\land\}$
  \Then
    \li \If Q.negated
    \Then
        \li Q.root.operator $\gets \lor$, Q.negated $\gets$ false
        \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated 
        \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
        \li \Return $\proc{RD-Tree-Chase}(Q, I, f, \phi)$
    \End
    \li $L \gets \proc{tree-to-conj}(Q.root.lchild)$
    \li \For $\psi \in L$
    \Do
        \li res.extend($\proc{RD-Tree-Chase}(Q.root.rchild, I, f, \phi \land \psi)$)
    \End
\li \ElseIf Q.root.operator $\in \{\lor\}$
  \Then
    \li \If Q.negated
    \Then
        \li Q.root.operator $\gets \land$, Q.negated $\gets$ false
        \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated
        \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
        \li \Return $\proc{RD-Tree-Chase}(Q, I, f, \phi)$
    \End
    % \li ConjTrees $\gets \proc{DisjTree-to-ConjTrees}(Q.root)$
    \li ConjTrees $\gets \proc{Expand-DisjTree}(Q.root)$
    \li \For $T \in ConjTrees$
    \Do
        \li res.extend($\proc{RD-Tree-Chase}(T, I, f, \phi)$)
    \End
\end{codebox}
}
\end{algorithm}


\begin{algorithm}[ht]
\continuecodebox
{\small
\begin{codebox}
  \li \If Q.root.operator $\in \{\exists\}$
  \Then
    \li \If Q.negated
    \Then
        \li Q.root.operator $\gets \forall$, Q.negated $\gets$ false
        \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
        \li \Return $\proc{RD-Tree-Chase}(Q, I, f, \phi)$
    \End
    \li \For $x \in I.domain(Q.root.variable)$
    \Do
        \li $g \gets f \cup \{Q.root.variable \to x\}$
        \li res.extend($\proc{RD-Tree-Chase}(Q.root.child, I, g, \phi)$)
    \End
    % \li $y \gets \proc{Add-Fresh-Var}(I, Q.root.variable)$
    \li Create a fresh labeled null $y$ in the domain of $x$
    \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
    \li $g \gets f \cup \{Q.root.variable \to y\}$
    \li res.extend($\proc{RD-Tree-Chase}(Q.root.child, I, g, \phi)$)
  \li \ElseIf Q.root.operator $\in \{\forall\}$
  \Then 
    \li \If Q.negated
    \Then
        \li Q.root.operator $\gets \exists$, Q.negated $\gets$ false
        \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
        \li \Return $\proc{RD-Tree-Chase}(Q, I, f, \phi)$
    \End
    \li $Ilist \gets [I]$
    \li \If $I.domain(Q.root.variable) = \emptyset$
        \Then
            \li $res.append(I)$
            % \li $y \gets \proc{Add-Fresh-Var}(I, Q.root.variable)$
            % \li Create a fresh variable $y$ in the domain of $x$
            % \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
    \li \Else
        \li \For $x \in I.domain(Q.root.variable)$
        \Do
            \li $Ilist' \gets []$
            \li \For $J \in IList$
            \Do
                \li $g \gets f \cup \{Q.root.variable \to x\}$
                \li $Ilist'.extend(\proc{RD-Tree-Chase}(Q.root.child, J, g))$ 
            \End
            \li $Ilist \gets Ilist'$
        \End
        \li res.extend($Ilist$)
    \End
    \li Create a fresh labeled null $y$ in the domain of $x$
    \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
    \li $Ilist' \gets []$
    \li \For $J \in IList$
    \Do
        \li $g \gets f \cup \{Q.root.variable \to x\}$
        \li $Ilist'.extend(\proc{RD-Tree-Chase}(Q.root.child, J, g))$ 
    \End
    \li res.extend($Ilist'$)
  \End
\End
\li \Return res

\end{codebox}
}
\end{algorithm}
}





% \begin{algorithm}[h]\caption{RD-Tree-Chase}\label{alg:rd-tree-chase}
%   \centering
% {\small
% \begin{codebox}
% \algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
% $Q$: a right deep syntax tree of a DRC query; \\
% $I$: current c-instance; \\
% $f$: current homomorphism from $var(Q) \cup cons(Q)$ to $var(I) \cup cons(I)$.\\
% $\phi$: current conjunction of literals.\\
% \algorithmicensure a list of c-instances\\
%   \Procname{$\proc{RD-Tree-Chase}(\schemaOf{\rel}, Q, I, f)$}
%   \li res $\gets []$
%   \li \If there is no quantifier in $Q$
%   \Then
%     \li $L \gets \proc{tree-to-conj}(Q)$
%     \li \For $\psi \in L$
%     \Do
%         \li $J \gets \proc{Add-to-Ins}(\schemaOf{\rel}, I, f(\psi))$
%         \li \If $J$ is consistent
%             \Then \li res.append($J$)
%         \End
%     \End
%   \li \ElseIf Q.root.operator $\in \{\land\}$
%   \Then
%     \li \If Q.negated
%     \Then
%         \li Q.root.operator $\gets \lor$, Q.negated $\gets$ false
%         \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated 
%         \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
%         \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%     \End
%     % \li lres $\gets \proc{RD-Tree-Chase}(Q.root.lchild, I, f)$
%     % \li rres $\gets \proc{RD-Tree-Chase}(Q.root.rchild, I, f)$
%     \li lres $\gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.lchild, I, f, limit)$
%     \li rres $\gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.rchild, I, f, limit)$
%     \li \For $J_1 \in lres$
%     \Do
%         \li \For $J_2 \in rres$
%         \Do
%           \li $K \gets \proc{MergeIns}(J_1, J_2)$
%           \li \If $K$ is consistent
%             \Then
%               \li res.append($K$)
%             \End
%         \End
%     \End
% \li \ElseIf Q.root.operator $\in \{\lor\}$
%   \Then
%     \li \If Q.negated
%     \Then
%         \li Q.root.operator $\gets \land$, Q.negated $\gets$ false
%         \li Q.root.lchild.negated $\gets \neg$ Q.root.lchild.negated
%         \li Q.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
%         \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%     \End
%     % \li ConjTrees $\gets \proc{DisjTree-to-ConjTrees}(Q.root)$
%     \li ConjTrees $\gets \proc{Expand-DisjTree}(Q.root)$
%     \li \For $T \in ConjTrees$
%     \Do
%         \li res.extend($\proc{RD-Tree-Chase}($\schemaOf{\rel}$, T, I, f)$)
%     \End
% \end{codebox}
% }
% \end{algorithm}


% \begin{algorithm}[ht]
% \continuecodebox
% {\small
% \begin{codebox}
%   \li \If Q.root.operator $\in \{\exists\}$
%   \Then
%     \li \If Q.negated
%     \Then
%         \li Q.root.operator $\gets \forall$, Q.negated $\gets$ false
%         \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
%         \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%     \End
%     \li \For $x \in I.domain(Q.root.variable)$
%     \Do
%         \li $g \gets f \cup \{Q.root.variable \to x\}$
%         % \li res.extend($\proc{RD-Tree-Chase}(Q.root.child, I, g)$)
%         \li res.extend($\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$)
%     \End
%     \li Create a fresh variable $y$ in the domain of $Q.root.variable$\label{alg:rd-tree-chase:line:exists-add-fresh-start}
%     \li $g \gets f \cup \{Q.root.variable \to y\}$
%     \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
%     % \li res.extend($\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, f, limit)$)
%     \li res.extend($\proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$)\label{alg:rd-tree-chase:line:exists-add-fresh-end}
%   \li \ElseIf Q.root.operator $\in \{\forall\}$
%   \Then 
%     \li \If Q.negated
%     \Then
%         \li Q.root.operator $\gets \exists$, Q.negated $\gets$ false
%         \li Q.root.child.negated $\gets \neg$ Q.root.child.negated
%         \li \Return $\proc{RD-Tree-Chase}($\schemaOf{\rel}$, Q, I, f)$
%     \End
%     \li $Ilist \gets [I]$
%     \li \If $I.domain(Q.root.variable) = \emptyset$
%         \Then
%             \li $res.append(I)$
%             % \li $y \gets \proc{Add-Fresh-Var}(I, Q.root.variable)$
%             % \li Create a fresh variable $y$ in the domain of $x$
%             % \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
%     \li \Else
%         \li \For $x \in I.domain(Q.root.variable)$
%         \Do
%             \li $g \gets f \cup \{Q.root.variable \to x\}$
%             \li $Ilist' \gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$
%             \li $cur \gets []$
%             \li \For $J_1 \in IList$
%             \Do
%                 \li \For $J_2 \in Ilist'$
%                 \Do
%                   \li $K \gets \proc{MergeIns}(J_1, J_2)$
%                   \li \If $K$ is consistent
%                     \Then
%                       \li cur.append($K$)
%                     \End
%                 \End
%             \End
%             \li $Ilist \gets cur$
%         \End
%         \li res.extend($Ilist$)
%     \End
%     \li Create a fresh variable $y$ in the domain of $Q.root.variable$\label{alg:rd-tree-chase:line:forall-add-fresh-start}
%     \li $g \gets f \cup \{Q.root.variable \to y\}$
%     \li $I.domain(Q.root.variable) \gets I.domain(Q.root.variable) \cup \{y\}$
%     % \li $Ilist' \gets []$
%     % \li \For $J \in IList$
%     % \Do
%     %     \li $g \gets f \cup \{Q.root.variable \to x\}$
%     %     \li $Ilist'.extend(\proc{RD-Tree-Chase}(Q.root.child, J, g))$ 
%     % \End
%     % \li res.extend($Ilist'$)
%     % \li $Ilist' \gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, f, limit)$
%     \li $Ilist' \gets \proc{RD-Tree-Chase-Naive}(\schemaOf{\rel}, Q.root.child, I, g, limit)$
%     \li \For $J_1 \in IList$
%     \Do
%         \li \For $J_2 \in Ilist'$
%         \Do
%           \li $K \gets \proc{MergeIns}(J_1, J_2)$
%           \li \If $K$ is consistent
%             \Then
%               \li res.append($K$)
%             \End
%         \End
%     \End\label{alg:rd-tree-chase:line:forall-add-fresh-end}
% \End
% \li \Return res

% \end{codebox}
% }
% \end{algorithm}

% \clearpage
\begin{algorithm}[!htp]\caption{Conjunctive Tree Construction}\label{alg:conj-tree-cons}
{\small
\begin{codebox}
\algorithmicrequire $Q$ a syntax tree of a DRC query
\\
\algorithmicensure List of syntax trees with no disjunction \\(using the rule: $A \lor B \implies \{A \land B, A \land \neg B, \neg A \land B\}$)\\
  \Procname{$\proc{DisjTree-to-ConjTree}(Q)$}
  \li res $\gets $ an empty list.
  \li \If Q.root is a leaf node
  \Then 
    \li \If Q.negated
    \Then 
        \li Q.root.atom $\gets \neg$Q.root.atom
    \End
    \li res.append(Q)
  \li \ElseIf Q.negated 
  \Then
    \li $res \gets \proc{Handle-Negation}(Q, \proc{DisjTree-to-ConjTree})$
  \li \ElseIf Q.root.operator $\in \{\land\}$
  \Then
    \li T $\gets CopyOf(Q)$
    % \li \If T.negated
    % \Then 
    %     \li T.root.operator $\gets \lor$, T.negated $\gets$ False
    %     \li T.root.lchild.negated $\gets \neg $T.root.lchild.negated
    %     \li T.root.rchild.negated $\gets \neg $T.root.rchild.negated 
    %     % \amir{This line should just flip the negated state and not set it as negated=true, right?}\\
    %     % \zhengjie{since $\neg(A \land B) =  (\neg A) \lor (\neg B)$, this is pushing negation down to the leaves}
    %     \li res $\gets \proc{DisjTree-to-ConjTree}(T)$
    % \li \Else
        \li $LTList \gets \proc{DisjTree-to-ConjTree}(T.root.lchild)$
        \li $RTList \gets \proc{DisjTree-to-ConjTree}(T.root.rchild)$
        \li \For $l \in LTList$
        \Do
            \li \For $r \in RTList$
            \Do
                \li T $\gets CopyOf(Q)$, T.root.lchild $\gets l$, T.root.rchild $\gets r$
                \li $res.append(T)$
            \End
        \End
    % \End
  \li \ElseIf Q.root.operator  $\in \{\lor\}$
  \Then
    \li T $\gets CopyOf(Q)$, T.root.operator $\gets \land$
    % \li \If T.negated
    % \Then 
    %     \li T.negated $\gets$ False
    %     \li T.root.lchild.negated $\gets \neg $T.root.lchild.negated
    %     \li T.root.rchild.negated $\gets \neg $T.root.rchild.negated 
    %     \li res $\gets \proc{DisjTree-to-ConjTree}(T)$
    % \li \Else
        \li T.root.lchild.negated $\gets$ Q.root.lchild.negated
        \li T.root.rchild.negated $\gets$ Q.root.rchild.negated
        \li res $\gets \proc{DisjTree-to-ConjTree}(T)$
        \li T.root.lchild.negated $\gets$ Q.root.lchild.negated
        \li T.root.rchild.negated $\gets \neg$ Q.root.rchild.negated
        \li res.extend($\proc{DisjTree-to-ConjTree}(T)$
        \li T.root.lchild.negated $\gets \neg$ Q.root.lchild.negated
        \li T.root.rchild.negated $\gets$ Q.root.rchild.negated
        \li res.extend($\proc{DisjTree-to-ConjTree}(T)$
    % \End
  \li \ElseIf Q.root.operator $ \in \{\forall, \exists\}$
  \Then
    \li T $\gets CopyOf(Q)$
%   \li \If T.negated
%     \Then 
%         \li \If T.root.operator $ \in \{\forall\}$
%         \Then
%             \li T.root.operator $\gets \exists$
%         \li \Else
%             \li T.root.operator $\gets \forall$
%         \End
%         \li T.negated $\gets$ False, T.root.child.negated $\gets \neg$ T.root.child.negated 
%         \li res $\gets \proc{DisjTree-to-ConjTree}(T)$
%     \li \Else
        \li arr $\gets \proc{DisjTree-to-ConjTree}(T.root.child)$
        % \amir{Should this also account for negation?}\\
        % \zhengjie{Yes, fixed.}
        \li \For $t \in arr$
        \Do
            \li T.root.child $\gets CopyOf(t)$
            \li res.append(T)
        \End
    \End
%   \End
  \li \Return res
\end{codebox}
}
\end{algorithm}


\cut{
\begin{algorithm}[h]\caption{RD-Tree-Chase-main}\label{alg:rd-tree-chase-main}
{\small
\begin{codebox}
\algorithmicrequire $\schemaOf{\rel}$: the schema of the relational database; \\
$Q_1, Q_2$: two DRC queries; \\
$limit$: the maximum number of tuples and conditions in the c-instances\\
\algorithmicensure A list of counterexample c-instances for $Q_1$ and $Q_2$. \\
\Procname{$\proc{RD-Tree-Chase-main}(\schemaOf{\rel}, Q_1, Q_2, limit)$}
% \li $Q'_1 \gets \exists \bm{x} (Q_1)$ where $\bm{x}$ are the free variables in $Q_1$ (after renaming)
% \li $Q'_2 \gets \exists \bm{x} (Q_2)$ where $\bm{x}$ are the free variables in $Q_2$ (after renaming)
% \li $Q \gets$ a right deep syntax tree of $Q'_1 \land \neg Q'_2$
\li $Q \gets$ a right deep syntax tree of $Q_1 \land \neg Q_2$
\li res $\gets []$, queue $\gets $ an empty queue
\li $I_0 \gets$ an empty c-instance of schema of  $\schemaOf{\rel}$
\li $h_0 \gets \{\}$
% \li \For $x \in FreeVar(Q)$
%     \Do
%         %\li Create a fresh variable $x'$ in the domain of $x$
%         \li $I.domain(x) \gets I.domain(x) \cup \{x\}$
%         \li $h_0 \gets h_0 \cup \{x \to  x\}$
%     \End
\li \For $x \in FreeVar(Q)$
    \Do
        \li $Q \gets \exists x Q(x)$
    \End
\li queue.push($I_0$)
\li visited $\gets \emptyset$
\li \While $\neg$ queue.isEmpty()
    \Do
        \li $I \gets $ queue.pop()
        \li \If I $\in$ visited or $|I| > limit$
        \li \Then continue
        \End
        \li visited $\gets $ visited $\cup \{I\}$
        \li \If $\proc{Tree-SAT}(Q, I, \emptyset)$ and $I$ is consistent
            \Then  
                \li $res.append(I)$
                \li continue
            \End
        \li $Ilist \gets \proc{RD-Tree-Chase}(Q', I, h_0, True)$
        \li \For $J \in Ilist$
        \Do
           \li \If $J \neq \bot$ and $|J| \leq limit$ and $J \notin$ visited
            \Then
                \li queue.push(J)
            \End
        \End
    \End
\li \Return $res$
\end{codebox}
}
\end{algorithm}
}





\subsection{Analysis of Algorithm \ref{alg:rd-tree-chase-main}}\label{sec:analysis}


\mypar{Soundness and completeness}
% \begin{proposition}[Soundness]
% Given a right deep syntax query tree $Q$, the c-instances outputted by Algorithm \ref{alg:conj-tree-cons} all satisfy $Q$.
% \end{proposition}
Given a right deep syntax tree $Q$ of a DRC query, Algorithm~\ref{alg:rd-tree-chase-main} will output a list of c-instances that are consistent and satisfy the query denoted by $Q$ (validated in Line 14), i.e., our procedure is sound. 
The full proofs can be found in Section \ref{sec:appendix}.

% \begin{Theorem}[Soundness]
% Given a syntax tree $Q$ of a boolean DRC query and a c-instance $\cinstance$, $\cinstance$ satisfies $Q$ iff Algorithm
% ~\ref{alg:tree-sat} returns True on $\proc{Tree-SAT}(Q, \emptyset, \emptyset)$.
% \end{Theorem}

\begin{Theorem}[Soundness]\label{thm:soundness}
Let $Q$ be a syntax tree of a Boolean DRC query over a schema $\schemaOf{R}$, and let $\cinstance \in res$ be a c-instance, where $res$ is the list of c-instances outputted by Algorithm \ref{alg:rd-tree-chase-main} when given $(\schemaOf{R}, Q, \emptyset, \emptyset)$, then $\cinstance$ satisfies $Q$.
\end{Theorem}



\begin{proof}[proof sketch]
To prove the proposition, it is enough to show that in Line 14 of Algorithm \ref{alg:rd-tree-chase-main} the procedure for checking that the c-instance $I$ satisfies the query $Q$\footnote{The pseudo code of the procedure, along with a proof of correctness are included in the appendix to the full version \cite{?} \amir{cite}}. 
% This is shown in Proposition \ref{prop:soundness-conj-sat} in the Section \ref{sec:tree-sat}, proving that Algorithm \ref{alg:tree-sat} returns true iff the given c-instance $\cinstance$ satisfies the given syntax tree $Q$. \amir{The proof we rely on is in the appendix}
\end{proof}

% \begin{Lemma}
% Given a syntax tree $Q$ and the set of c-instances $\mathcal{S}_{\cinstance} = \{\cinstance_1, \ldots, \cinstance_k\}$ outputted by Algorithm \ref{alg:rd-tree-chase-main}, if $\cov$ is the coverage of some ground instance $K$ satisfying $Q$, then there is $\cinstance_i \in \mathcal{S}_{\cinstance}$ with coverage $\cov$.
% \end{Lemma}

\begin{Theorem}[Completeness]\label{theorem:completeness}
Given a right deep syntax query tree $Q$ and the set of c-instances $\mathcal{S}_{\cinstance} = \{\cinstance_1, \ldots, \cinstance_k\}$ outputted by Algorithm \ref{alg:rd-tree-chase-main} with the parameter $limit$, if a \amir{Minimal?} ground instance $\ains$ of size $\leq limit$ that satisfies $Q$ with coverage $\cov$,
% under a homomorphism $h$ from $FreeVar(Q)$ to values in $K$, 
then there exists $\cinstance_i \in \mathcal{S}_{\cinstance}$ with coverage $\cov' \supseteq \cov$ that c-homomorphically maps \amir{Just maps?} to $\ains$.
\end{Theorem}

\begin{proof}[proof sketch]
\amir{add. Check that without RD and with the latest changes in the algo. the proof still works}
\end{proof}

\mypar{Termination}
Recall that in Section \ref{sec:model} we have determined that that the problem of finding a universal solution (Definition \ref{def:universal}) is undecidable. 
Despite this, Algorithm \ref{alg:rd-tree-chase-main} is guaranteed to terminate due to the $limit$ parameter (Line 11) and the $visited$ set.

\begin{proposition}
Given a query $Q$, Algorithm \ref{alg:rd-tree-chase-main} is guaranteed to terminate.
\end{proposition}

\begin{proof}
Since the $limit$ parameter is finite, there are finitely many options for c-instances that it can generate. If the size of the c-instance increases over $limit$, the algorithm will ignore this c-instance and not push it into $queue$ (Lines 11--12). 
The algorithm will also not get into an infinite loop as well because of the $visited$ set. Every generated c-instance is placed into this set and c-instance already found is the set are ignored and are not pushed into $queue$ (Lines 11--12). 
% There may still be an infinite loop in Line 9 is a domain of a variable is infinite. However, since all the procedures used by Algorithm \ref{alg:rd-tree-chase-main}
Finally, note that the domain of all labeled nulls in the c-instance is derived from existing labeled nulls representing the same attribute in the c-instance, and thus cannot be infinite.
\end{proof}

% However, even without it, if the domain of all variables is finite, Algorithm \ref{alg:rd-tree-chase-main} is guaranteed to terminate since the number of combinations of domain values is finite. 
% Note that the algorithm may expand the initial domain of the variables (e.g., Lines 16--17 in Algorithm \ref{alg:forall-op}) but this would occur a finite number of times during the process.

% \amir{Add that if all domains a finite, then termination is guaranteed.}
% The proof of Theorem~\ref{theorem:completeness} needs Lemma~\ref{lemma:union-c-homo}, Lemma~\ref{lemma:and-sat}, and Lemma~\ref{lemma:forall-sat}.

% \begin{Lemma}\label{lemma:union-c-homo}
% Given two c-instances $J_1$ and $J_2$ that c-homomorphically map to a ground instance $K$ under $\assignment_1$ and $\assignment_2$ respectively, if for every $x \in vars(J_1) \cap vars(J_2)$, $\assignment_1(x) = \assignment_2(x)$, $J_1 \cup J_2$ c-homomorphically maps to $K$ under $\assignment_1 \cup \assignment_2$.
% \end{Lemma}

% \begin{proof}
% We show that $\assignment = \assignment_1 \cup \assignment_2$ is a c-homomorphism from $J_1 \cup J_2$ to $K$. Let $\phi \in J_1 \cup J_2$ be an arbitrary relational atom $\rel(x_1, ..., x_{\relarity})$, by the definition of c-homomorphism, $K$ contains $\rel(\assignment(x_1), ..., \assignment(x_{\relarity}))$; let $\phi$ be the negation of an arbitrary relational atom $\neg \rel(x_1, ..., x_{\relarity})$, $K$ does not contain the relational fact  $\rel(\assignment(x_1), ..., \assignment(x_{\relarity}))$, and thus $\assignment(J_1 \cup J_2)$ does not contain $\rel(\assignment(x_1), ..., \assignment(x_{\relarity}))$; let $\phi \in J_1 \cup J_2$ be an arbitrary binary expression $x~op~y$, we also have the image under $\assignment$ of this expression $\assignment(x)~op~\assignment(y)$ to be True in $K$. Hence $J_1 \cup J_2$ c-homomorphically maps to $K$ under $\assignment_1 \cup \assignment_2$. \SR{polish}
% \end{proof}

% \begin{Lemma}\label{lemma:and-sat}
% Given a DRC query $Q=Q_1 \land Q_2$, a ground instance $K$ that satisfies $Q$, and two c-instances $J_1$ and $J_2$ that c-homomorphically map to $K$ and satisfy $Q_1$ and $Q_2$ respectively, if either $Q_1$ or $Q_2$ has no quantifiers, then $J_1 \cup J_2$ c-homomorphically map to $K$ and satisfies $Q$.
% \end{Lemma}

% % \begin{Lemma}\label{lemma:union-coverage}
% % Given two c-instances $J_1$ and $J_2$ that c-homomorphically map to a ground instance $K$ under $h_1$ and $h_2$ respectively and a syntax query tree $Q$ where $J_1$ and $J_2$ satisfy $Q$ with coverage $\cov_1$ and $\cov_2$ respectively, $J_1 \cup J_2$ satisfies $Q$ 
% % \end{Lemma}

% \begin{Lemma}\label{lemma:forall-sat}
% Given a DRC query $Q=\forall x Q'(x)$, a ground instance $K$ that satisfies $Q$, and $l$ c-instances $J_1, J_2, ..., J_l$ that c-homomorphically map to $K$ and satisfy $h_i(Q')$ respectively, where $l = |K.dom(x)|$ and each $h_i$ maps the free variable $x$ in $Q'$ to a different value in $K.dom(x)$, if either $Q_1$ or $Q_2$ has no quantifiers, then there exist c-instances $J'_1, J'_2, ..., J'_l$ such that each $J_i$ homomorphically maps to $J'_i$ and $\bigcup_{i=1}^{l} J'_i$) c-homomorphically maps to $K$ and it satisfies $Q$.
% \end{Lemma}

% \begin{proof}[Proof for Theorem~\ref{theorem:completeness}]
% We prove the theorem by induction of the number of nodes in the syntax tree $Q$. 

% %\zhengjie{safety issue here}
% If $|V(Q)| = 1$, there is only one leaf node $u$ --- it can only be an atom or the negation of an atom \SR{do you keep the $\neg$? see defn 11}, and the coverage can only be $\{u.atom\}$ (otherwise $Q$ evaluates to an empty result), and the homomorphism $h$ maps the free variables in $u.atom$ to vales in $K$, i.e., $h(u.atom)$ exists in $J$ if it is a relational atom, or it evaluates to True otherwise.
% In this case, the algorithm simply calls $\proc{RD-Tree-Chase}$ one time to add this atom to the empty c-instance and returns a list with only this instance, which covers $u.atom$. $h$ is the c-homomorphism from the variables in $u.atom$ to values in $K$.

% Assume that for every $Q$ such that $|V(Q)| < n$, for a ground instance $K$ satisfying $Q$ with coverage $\cov$ under a homomorphism $h$, there is a c-instance in the result of Algorithm~\ref{alg:rd-tree-chase-main} has coverage $\cov' \supseteq \cov$ for $Q$ that c-homomorphically maps to $K$.  We show that the claim is true for $Q$ with $|V(Q)| = n$.

% If the root of $Q$ is an $\land$ node, i.e., $Q = Q_1 \land Q_2$ where $V|Q_1| < n$ and $V|Q_2| < n$, and then the coverage of $K$ for $Q$ is $\cov = \cov_1 \cup \cov_2$ where $\cov_1$ is a subset of leaf atoms of $Q_1$ and $\cov_2$ is a subset of leaf atoms of $Q_2$.  Since the tree $Q$ is a right deep syntax tree, its left child $Q_1$ has no quantifiers (has only connecitves and leaf atoms), in lines 14 it directly generates a list of conjunction of atoms from $Q_1$ by expanding disjunctions into three conjuncive cases ($A \lor B \to \{A \land B, A \land \neg B, \neg A \land B$\}), then any $\cov_1$ \amir{any $\cov_1$?} of $Q_1$ must be covered in one of the expanded conjunctions. Furthermore, note that keep running the procedure $\proc{RD-Tree-Chase}$ in Algorithm~\ref{alg:rd-tree-chase-main} does not change the results on $Q_1$ --- the free variables are all assigned fresh variables at the beginning of Algorithm~\ref{alg:rd-tree-chase-main}, and thus it does not add new variables to the domain of the c-instances. 
% Therefore, we run Algorithm~\ref{alg:rd-tree-chase-main} on $Q$ as running Algorithm~\ref{alg:rd-tree-chase-main} on $Q_1$ and $Q_2$ separately, and then merging the result instances from $Q_1$ to the result instances from $Q_2$. %In line 15-16, we write it as a recursive call to $\proc{RD-Tree-Chase}$ on the right child $Q_2$ of $Q$ for each of the expanded conjunction from $Q_1$. 
% % \amir{I wasn't able to follow this argument. Can't there be an intersection between the domains considered in $Q_1$ and those considered in $Q_2$? e.g., if the root of $Q_2$ is a universal quantifier that applies to the vars in $Q_1$}. 
% %Since there must be a expanded conjunction from $Q_1$ with coverage $\cov_1$, and by

% \begin{figure}[h]
% \centering
%  \includegraphics[width=.8\linewidth]{figures/proof-theorem1-and.pdf}
%   \caption{Illustration of the $\land$ case in Proof of Theorem~\ref{theorem:completeness}}
%   \label{fig:proof-completeness-and}
% \end{figure}
% By the induction hypothesis, since $K$ satisfies $Q_1$ and $Q_2$ with coverage $\cov_1$ and $\cov_2$ respectively, there are a c-instance $J_1$ for $Q_1$ with coverage $\cov_1' \supseteq \cov_1$ and a c-instance $J_2$ for $Q_2$ with coverage $\cov_2' \supseteq \cov_2$ in the results of Algorithm~\ref{alg:rd-tree-chase-main}, and both $J_1$ and $J_2$ c-homomorphically map to $K$ under $\assignment_1$ and $\assignment_2$ respectively.
% % \amir{But $K$ can be satisfiable without $J_1$/$J_2$ being satisfiable, right? ($K$ is always satisfied because its grounded)}. 
% We next show that there is are two mappings between $J_1$ and $J_2$ to $K$ respectively, such that their union maps $J_1 \cup J_2$ to $K$. 

% Because $K$ satisfies $Q=Q_1 \land Q_2$, there exists a homomorphism $h_0$ that maps free variables in $Q_1 \land Q_2$ to values in $K$, such that $K$ satisifies $Q_1 \land Q_2$ under $h_0$. In particular, $K$ satisfies $Q_1$ and $Q_2$ so the induction hypothesis can be used. 
% Hence, we have $h_1 = h_0|_{vars(Q_1)}$ that maps the free variables in $Q_1$ to values in $K$, and $h_2 = h_0|_{vars(Q_2)}$ maps the free variables in $Q_2$ to values in $K$.
% We show that we can construct c-homomorphsims $\assignment_1$ and $\assignment_2$ that have no conflicts. Suppose $f_1$ and $f_2$ are the mappings from free variables in $Q_1$ and $Q_2$ to variables in $J_1$ and $J_2$ respectively, as initialized in Algorithm~\ref{alg:rd-tree-chase-main} to be identity functions. Hence for $Q_1$ we have $\assignment_1 = h_1 \circ f_1^{-1}$ to be a c-homomorphism from $J_1$ to $K$ (since the algorithm assigns fresh variables to all free variables in $J_1$ in lines \ref{l:iter-free}--\ref{l:add-fresh}, $f_1$ is bijective and therefore $f_1^{-1}$ is a mapping from $J_1$ to free variables in $Q_1$). For $Q_2$, we build two mappings 
% %$h_2^{**}: x \to h_2^*(x)$ 
% %$h_2^{**-1}: h_2^*(x) \to x$
% $(f_2^{*})^{-1}: Im(f_2) \to FreeVars(Q_2)$
% by restricting the co-domain of $f_2$ to its image and an identity function $g_2: vars(J_2)\setminus image(f_2) \to vars(J_2)\setminus image(f_2)$, then we construct $f'_2 = (h_2 \circ f_2^{*-1}) \cup g_2$ maps variables in the image of $f_2$ to values in $K$ and keeps other variables in $J_2$ unchanged. Then the c-instance $J_2' = f'_2(J_2)$ satisfies $f_2(Q_2)$ with coverage contains $f_2(C_2)$ (we abuse $f_2$ here, i.e., only free variables in $Q_2$ are mapped to values in $K$ while other variables and constants are not changed) \amir{Did not follow this. $h_2^*(Q_2)$ is a c-instance, not a query, right?}. Again by the induction hypothesis, $J_2'$ c-homomorphically maps to $K$ under some $\assignment_2'$, then we have $\assignment_2 =  (h_2 \circ f_2^{*-1}) \cup \assignment_2'$ is a c-homomorphsim from $J_2$ to $K$. 

% Now we show that $J_1 \cup J_2$ c-homomorphically maps to $K$ and covers $Q_1 \land Q_2$ with coverage $\cov' \supseteq \cov_1 \cup \cov_2$. 
% The former is directly by Lemma~\ref{lemma:union-c-homo}: since $h_1'$ and $h_2'$ \amir{$h_1$ and $h_2$?} agree on all variables in the intersection of their domains (variables that can be mapped from the free variables), implying that $h_1$ and $h_2$ have no conflicts, therefore $J_1 \cup J_2$ c-homomorphically maps to $K$. 
% % The former is directly by the fact that $h_0$ is a c-homomorphism from $J_1$ to $K$ and $h_2 \circ h_0$ is a c-homomorphism from $J_2$ to $K$.
% % Let $\phi \in J_1 \cup J_2$ be an arbitrary relational atom, by the definition of c-homomorphism, $K$ contains $(h_2 \circ h_0)(\phi)$; let $\phi$ be the negation of an arbitrary relational atom, $K$ does not contain the relational fact of $(h_2 \circ h_0)(\phi)$; let $\phi \in J_1 \cup J_2$ be an arbitrary binary expression $x op y$, we also have the image under $h_2 \circ h_0$ of this expression $(h_2 \circ h_0)(x) op (h_2 \circ h_0)(y)$ to be True in $K$. Hence $J_1 \cup J_2$ c-homomorphically maps to $K$ under $h_2 \circ h_0$. 

% For the claim on coverage, assume $J_1 \cup J_2$ does not satisfy $Q$ with coverage $\cov' \supseteq \cov$. Since $Q_1$ has no quantifiers, $J_1 \cup J_2$ must satisfy $Q_1$ with coverage $\cov'_1 \supseteq \cov_1$ (the c-homomorphism $\assignment_1 \cup \assignment_2$ also gives an assignment for $J_1 \cup J_2$ that satisfies $Q_1$); and since $J_1 \cup J_2$ c-homomorphically maps to $K$, $J_1 \cup J_2$ is consistent, then the only case is that there is an atom $\beta \in \cov_2$ is covered by $J_2$ but not by $J_1 \cup J_2$. That is, the insertion of some atoms in $J_1$ into $J_2$ makes $\beta$ not homomorphically map to some atom in $J_2$, which is impossible \amir{Couldn't $\beta$ be a condition that has a conflict with $J_2$?}. Hence, the assumption is wrong, $J_1 \cup J_2$ satisfies $Q$ with coverage $\cov' \supseteq \cov$.
 
% If the root of $Q$ is an $\lor$ node, i.e., $Q = Q_1 \lor Q_2$ where $V|Q_1| < n$ and $V|Q_2| < n$, and then the coverage $\cov = \cov_1 \cup \cov_2$ where $\cov_1$ is a subset of leaf atoms of $Q_1$ and $\cov_2$ is a subset of leaf atoms of $Q_2$. The algorithm splits the tree into three cases, where each is rooted by a $\land$ node: (1) where no child of the root is negated, (2) where the left child is negated and (3) where the right child is negated. Then it is reduced to the above $\land$ case.

% If the root of $Q$ is an $\exists$ node: $Q = \exists x Q'(x)$ where $V|Q'| < n$, 
% it is clear that if $\cov$ is covered by some instance $K$ for $Q$, then it is also covered by $K$ for $Q'$. By the induction hypothesis, there is a c-instance $J$ outputted by Algorithm~\ref{alg:rd-tree-chase-main} for $Q'$ with coverage containing $\cov$ that c-homomorphically maps to $K$, and $J$ is also a satisfying c-instance for $Q$ with coverage containing $\cov$.

% If the root of $Q$ is an $\forall$ node: $Q = \forall x Q'(x)$ where $V|Q'| < n$, $\cov$ is covered by $K$ for $Q$ under homomorphism $h$. Unlike the above $\exists$ case, for $Q'$, different subsets of $\cov$ (denoted as $\cov_1, ..., \cov_l$, where \cov = $\bigcup_{i=1}^{l}\cov_i$) are covered under different homomorphisms that map the free variable $x$ to different values $v_i$ in the domain of $x$ in $K$. 

% We show by construction that a c-instance that c-homomorphically maps to $K$ and satisfies $Q$ with coverage $\cov' \supseteq \cov$ will be outputted by Algorithm~\ref{alg:rd-tree-chase-main}.
% For each value in $K$ we create a corresponding variable to obtain a c-instance $J_0$ with an empty global condition \amir{lines?}, and denote the bijection from the variables in $J_0$ to the values in $K$ as $\assignment$ (we also abuse $\assignment$ as a homomorphism from $J_0$ to $K$, $\assignment(J_0) = K$, $\assignment^{-1}(K) = J_0$).
% Then, we initialize the c-instance $I_0$ in Algorithm~\ref{alg:rd-tree-chase-main} by setting its domains to be the same as $J_0$ \amir{lines?}. That is, when running the algorithm, instead of allowing the algorithm to create fresh variables, we skip lines \ref{alg:rd-tree-chase:line:exists-add-fresh-start}-\ref{alg:rd-tree-chase:line:exists-add-fresh-end}, \ref{alg:rd-tree-chase:line:forall-add-fresh-start}-\ref{alg:rd-tree-chase:line:forall-add-fresh-end} in Algorithm~\ref{alg:rd-tree-chase} and thus only allow it to map the quantified variables to one of the variables added in advance in $J_0$.

% For each coverage subset $\cov_i$, we define a mapping $h_i = h \cup \{x \to v_i\}$ where $x$ is the quantified variable at the root of $Q$ and value $v_i \in K.\dom(x)$, then $h_i$ maps the free variables in $Q'$ to values in $K$, i.e., $K$ satisfies $Q'$ with coverage $\cov_i$ under $h_i$.

% \begin{figure}[h]
% \centering
%  \includegraphics[width=.6\linewidth]{figures/proof-theorem1-forall.pdf}
%   \caption{Illustration of the $\forall$ case in Proof of Theorem~\ref{theorem:completeness}}
%   \label{fig:proof-completeness-forall}
% \end{figure}

% By the induction hypothesis, for each $v_i$, since the ground instance $K$ covers $Q'$ with coverage $\cov_i$ under $h_i$, there is a c-instance $J_i$ outputted by Algorithm~\ref{alg:rd-tree-chase-main} that satisfies both $Q'$ with coverage $\cov'_i \supseteq \cov_i$ and c-homomorphically maps to $K$ under some $\assignment_i$. Since $\assignment$ is a bijection, let $J'_i = \assignment^{-1}(\assignment_i(J_i))$, then $J'_i$ also covers $Q'$ with coverage $\cov'_i$ \amir{explain why $J'_i$ is different from $J_0$}. Because each $J'_i$ is mapped to a sub-instance of $K$ under $\assignment$, the union of all $J'_i$-s ($J = \bigcup_{i=1}^{l} J'_i$) c-homomorphically maps to $K$ under $\assignment$ and thus it satisfies $Q$ with coverage $\cov' \supseteq \cov$. 

% The original algorithm can find such $J = \bigcup_{i=1}^{l} J'_i$, because (1) the algorithm dynamically increases the size of each domain and will reach the same cardinality in all domains as $J_0$, and (2) each ideal $J'_i$ will be returned the algorithm (line 51-53 in Algorithm~\ref{alg:rd-tree-chase}) --- from the construction procedure above we know that the difference between each $J_i$ and $J'_i$ is that they may contain a different subset of variables in $J_0$, however, since the Algorithm~\ref{alg:rd-tree-chase} will enumerate every variable in the domain when dealing with quantified variables, every possible subset of variables in $J_0$ will be considered. Therefore, whenever there is a valid $J = \bigcup_{i=1}^{l} J'_i$, the algorithm will find it.

% % Now we show the union of all $J'_i$-s ($J = \bigcup_{i=1}^{l} J_i$) c-homomorphically maps to $K$ and satisfies $Q$ with coverage $\cov' \supseteq \cov$. First, for each $J_i$ and $h_i$, we create a new variable $x_i$ to replace the universally quantified $x$ in $Q$ (remember that free variables are directly added to the domain of the c-instances). 
% % Then, in each $J_i$, we rename all variables such that there are no shared variables in all $J_i$-s except the free variables in $Q$.
% % To do this, in $\proc{RD-Tree-Chase}$, we set the domain of $x$ to be $\{x_1, ..., x_l\}$ (changee line 44) and do not create fresh variables for $x$ (line 34-37 and line 54-60 are skipped for the domain of $x$), and rename the variables in the resulting c-instances of the recursive call of $\proc{RD-Tree-Chase}$ for each variable in the domain (line 48-53), such that there are no shared variables except the free variables in $Q$. Because all $h_i$-s are extensions of $h$, by Lemma~\ref{lemma:union-c-homo}, $J$ c-homomorphically maps to $K$ under $h' = \bigcup_{i=1}^{l} h_i$.

% % For the claim on coverage, assume that for some $Q'_i$, there is an atom $\beta \in \cov_i$ not covered by $J$ but covered by $J_i$. By definition, there exists some homomorphism that maps $\beta$ to an atom in $J_i$, and such an atom still appear in $J$. 

% For cases where the syntax tree is negated, the algorithm will change the root operator accordingly ($\land$ to $\lor$, $\land$ to $\lor$, $\exists$ to $\forall$, and $\forall$ to $exists$) and change the negated flags of the root and the children. 
% \end{proof}


\mypar{Complexity}
\amir{Verify:} 
The complexity of Algorithm \ref{alg:rd-tree-chase-main} is $\Theta(3^{d \cdot |Dom|^{u + e}} \cdot |Dom|^2)$, where $d$ is the number of disjunctions, $|Dom|$ is the number of cells in the c-instance (the maximum number is $limit \cdot k \cdot \schemaOf{\rel}$ where $k$ is the number of tables in the c-instance), and $u$ ($e$) is the number of universal (existential) quantifiers. This bound is also tight. 
To explain why it is a lower bound, consider the query $\forall x_1 \ldots \forall x_m R(x_1) \lor R(x_2) \lor \ldots \lor R(x_m)$. Given this query, denoted by $Q$, Algorithm \ref{alg:rd-tree-chase-main} first generates a c-instance, where the free variables in $Q$ are mapped to fresh variables in the domain (there are no free variables in $Q$). Then, it performs a BFS using Algorithm \ref{alg:rd-tree-chase}. 
Algorithm \ref{alg:rd-tree-chase} recurses over the tree, and for each $\forall$ quantifier, it calls Algorithm \ref{alg:forall-op} that performs $|Dom|$ iterations and for each iteration, generates a tree (due to the loop in Line 5 and the recursive call in Line 7). For each tree, the algorithm iterates over the c-instances generated in Lines 9--10, resulting in the need for $|Dom|^2$ iterations. 
Then, for each $\lor$ operator, it calls Algorithm \ref{alg:or-op} that expands the subtree into $3$ trees resulting in $3^d$ trees. For each one of these trees, Algorithm \ref{alg:and-op} that performs a recursive call on the left child resulting in $|Dom|$ instances and for each of these instances, recurses on the right child (Line 5). Thus, we have $(3^{|Dom|^u})^{d} \cdot |Dom|^2$ operations. 
Since $\land$ does not expand the current number of trees and $\exists$ expands the number by $|Dom|$, the above expression is an upper bound on the number of trees as well. 
% Algorithm will enumerate $O(3^{|Disj| \cdot |Dom|^U}))$ tree structures, where $D$ is the size of the domain in the resulting instance (number of labeled nulls and constants), $M$ is the number of disjunctions, and $U$ is the number of universal quantifiers. \zhengjie{Not a tight bound, also ignore the model checking part}
% \amir{Why is $|Dom|$ in the exponent?}

% The complexity comes from two parts: (1) the elimination of one disjunction node in the syntax tree introduces three different conjunctive trees, and (2) the universal quantifier allows the subtree to have different conjunctive tree structures for different values or labelled nulls taken by the quantified variable. Consider the example $\forall x (A(x) \land (\forall y (B(y) \lor C(x,y))))$ where $x$ and $y$ are in the same domain. The innermost disjunction $B(y) \lor C(x,y)$ will be introduce three conjunctive cases; and then when iterating $\forall y$, the subtree structures for different labeeled null are independent. That is, assume there two labeled nulls $a$ and $b$ in the domain, we have two consider all possible combinations of $B(y) \land C(x,y)$, $B(y) \land \neg C(x,y)$, $\neg B(y) \land C(x,y)$ for each labeled null, e.g., $B(a) \land C(x,a)$ and $B(b) \land \neg C(x,b)$, $\neg B(a) \land C(x,a)$ and $B(b) \land C(x,b)$, etc., resulting in $O(3^2)$ tree structures. Then the outer $\forall x$ leads to another round of iteration, then we will encounter formulas such as $B(a) \land C(a,a)$ $\land B(b) \land \neg C(a,b)$, $\neg B(a) \land C(a,a)$ $\land B(b) \land C(a,b)$,...,  $B(a) \land C(b,a)$ and $B(b) \land \neg C(b,b)$, and so on, thus we have $O(3^4)$ different structures.

==> sections/implementation_discussion.tex <==
\section{Discussion of our approach}

{\bf Outline of this section:}
\begin{enumerate}
    \item DRC vs. TRC including examples of scenarios where we get different results in each
    \item Using solvers for checking satisfiability 
    \item Different notions of coverage and minimality
\end{enumerate}

\amir{Status: we don't have anything here yet}

==> sections/methods.tex <==
\section{Methods}

\subsection{The first step: Convert queries into DRC}

\subsection{Method 1: Brute-force algorithm}
\cut{\mypar{Method 1 (brute-force)}
\begin{enumerate}
    \item Convert $Q-Q_0$ (or $Q_0 - Q$) into a prenex normal form formula.
    \item Enumerate over all subsets of quantified varibles.
    \item For a subset of variables $S_v$, rebuild the DRC formula by removing all variables not in $S_v$ and predicates referring to varaibles not in $S_v$.
    \item For each rebuilt DRC, create a c-instance $I$ of $D$, where initial tuples are based on references in the DRC and conditions are from the atomic predicates in DRC.
    \item For every universal quantified variable, apply conditions on it to all tuples referring it.
    \item Add/delete tuples according to key constraints.
    \item Convert $Q-Q_0$ into SMT constraints; convert the c-instance $I$ into SMT constraints $\psi$ (note that translating universal quantifier into SMT constraints needs to enumerate over all values)
    \item Solve ($\psi \implies Q-Q_0$) or ($\psi \implies Q_0-Q$), record every $I$ with valid $\psi$
    \item Return all minimal $I$ (not a sub-instance of other valid c-instances)

\end{enumerate}

\begin{Example}
Consider again the beer database and queries $Q$ and $Q_0$. We have the DRC version of $Q-Q_0$ in PNF:
\begin{align*}
Q-Q_0=\{(X_1, B_1) & \ \mid \ \\
\exists C1, C2, C3, C4 &\Big( \\
\forall C5, C6 \Big(\exists &C7, C8, C9, C10, C11 \big(\\
Serves(X_1, B_1, C2) &\land Likes(C1, B_1) \land C1 \ LIKE \ 'Eve\%' \land Serves(C3, B_1, C4) \land C2>C4\\
\land(&(Serves(C7, C8, C9) \land  Serves(C10, C8, C11) \land C9<C11 \land X_1 == C7 \land B_1==C8) \\
&\lor  !Likes(C5,B_1) \lor !(C5 \ LIKE \ 'Eve\ \%') \lor !Serves(X_1, B_1, C6))\big)\Big)\Big)\}
\end{align*}

\begin{figure*}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\linewidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $C1$ & $daddr1$ & $PrefixEve(C1) \land \neg FNEve(C1)$ \\
        $C5$ & $daddr2$ & 
        $\neg FNEve(C5)$ \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.3\linewidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $X_1$ & $baddr1$ &$true$\\
        $C3$ & $baddr2$ &$true$\\
        \rowcolor{grey}$C7$ & $baddr3$ &$true$\\
        $C10$ & $baddr4$ &$true$\\\hline
        \multicolumn{3}{|c|}{$X_1 = C7$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.3\linewidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $B_1$ &  $brewer1$ &$true$\\
        \rowcolor{grey}$C8$ &  $brewer2$ &$true$\\\hline
    \multicolumn{3}{|c|}{$B_1 = C8$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\linewidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\linewidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $C1$ & $B_1$ & $true$ \\
       $C5$ & $B_1$ & $true$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\linewidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
        $X_1$ &$B_1$ &$C2$ &$true$\\
        $C3$ &$B_1$  &$C4$ & $true$ \\
        \rowcolor{grey}$C7$ & $C8$ & $C9$ &$true$\\
        $C10$ & $C8$ & $C11$ &$true$\\
        \rowcolor{grey}$X_1$ & $B_1$ & $C6$ &$true$\\
        \hline
        \multicolumn{4}{|c|}{$C4 < C2 \land C9 < C11$ $\land X_1 = V7$ $\land B_1 = C8$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:brute-force-c-ins}\small
  A c-instance built directly from $Q-Q_0$. Grey rows means the tuple can be removed by database constraints.}
\end{figure*}

Figure~\ref{fig:brute-force-c-ins} shows a c-instance built with the complete DRC of $Q-Q_0$.
\end{Example}
}
\mypar{Method 1 (brute-force)}
\begin{enumerate}
    \item Convert the formula in the DRC of $Q-Q_0$ (or $Q_0 - Q$) into prenex disjunctive normal form (PDNF): $$\exists x_1,x_2,...,x_n \forall y_1, ..., y_m C_1 \lor C_2 ... \lor C_k$$, where each $C_i$ is a clause in the form of a literal or the conjunction of literals; and a literal can a DRC atom or the negation of a DRC atom.   
    \item For each clause $C_i$ (it represents a class of counterexamples if it is satisfiable).
    \begin{enumerate}
    \item Let $C_i$ be in the form of $P_{i1} \land P_{i2} ... \land P_{ik_i} \land Q_{i1} \land Q_{i2} ... \land Q_{il_i}$, where each $P_{ij}$ is a literal involving only constants and existentially quantified variables $(x_1, ..., x_n)$ and each $Q_{ij}$ is a literal involving at least one universally quantified variables $(y_1, ..., y_n)$.
    \item Let $D_i$ be an c-instance with empty c-tables.
    \item For each $P_{ij}$ in the form of $r(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ where each $z^s_{ij}$ is either a constant or one of existential quantified $x_i$, add a tuple $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ to c-table $r$ in $D_i$.
    \item For each $P_{ij}$ in the form of $\neg r(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$, check if the tuple $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ exists in $r$. If it exists, the current $C_i$ cannot be satisfied. If it does not exist, add a table-wise condition that not all c-tuples in $r$ are equal to  $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$.
    \item For each $P_{ij}$ in the form of $z^1_{ij}~op~z^2_{ij}$, add it as a condition to the global condition of $D_i$ if $z^1_{ij}$ and $z^2_{ij}$ are variables that appear in multiple c-tables; add it as a table-wise condition  to $D_i$ if the variables appear in only one c-table; or, add it as a local condition to $D_i$ if the variables appear in only one c-tuple or $z^2_{ij}$ is a constant.
    \item Let $X$ the set of existentially quantified variables in $Ci$, and $Y$ be the set of universally quantified variables in $Ci$, let $F$ be the set of all possible mappings from $Y$ to $X$. 
    \item For each $f$ in F:
    \begin{enumerate}
    \item For each $Q_{ij}$ in the form of $r(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$, replace all variables in $Y$ with its mapped variable in $X$, then add the mapped c-tuple $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ to c-table $r$ in $D_i$ if it does not exist in $r$.
    \end{enumerate}
    \item For each $f$ in F:
    \begin{enumerate}
    \item In all $Q_{ij}$, replace all variables in $Y$ with its mapped variable in $X$.
    \item For each $Q_{ij}$ in the form of $z^1_{ij}~op~z^2_{ij}$, treat is the same as $P_{ij}$ but add conditions to $D_i$.
    \item For each $Q_{ij}$ in the form of $\neg r(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$, check if the tuple $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ exists in $r$. If it exists, the current $C_i$ cannot be satisfied.
    \end{enumerate}
    \item If $D_i$ is satisfiable, then $D_i$ is a valid c-instance. 
    \end{enumerate}
    %\item Return all minimal $I$ (not a sub-instance of other valid c-instances)
    \item Return all valid c-instances.

\end{enumerate}

\amir{1. translation of a formula to a c-table, 2. how many c-tables can a formula generate (upper bound)? 3. what is the max size of a generated c-table? 4. is this algorithm generating all possible counter example c-tables?}

\zhengjie{2. only one c-table is generated per clause in DNF. 3. the size should be bounded by the number of variables and constants, if there is no cyclic tuple generating dependencies. 4. No, as we are only looking into one clause in the DNF when building the c-table; but I conjecture it would be yes if we add some restrictions on valid counterexamples, more thoughts needed here}

\begin{algorithm}[t]\caption{InitDomain}\label{alg:init-domain}
{\small
\begin{codebox}
  \Procname{$\proc{InitDomain}(X, Y, R)$}
  \li $M \gets$ an empty map
  \li \For $R_i \in R$
  \Do
    \li \For $A \in attr(R_i)$
    \Do
        
        
        \li $M[A] \gets \emptyset$
    \End
  \End
  
  \li \For each $x \in X$
  \Do
    \li $A \gets attr(x)$ 
    \li $M[A] \gets M[A] \cup \{x\}$
  \End
  \li \For each $y \in Y$
  \Do
    \li $A \gets attr(y)$ 
    \li \If $M[A] = \emptyset$
    \Then 
    \li $x' \gets $ a fresh variable in $var(A)$
    \li $M[A] \gets M[A] \cup \{x'\}$
    \End
  \End
  \li \Return $M$
\end{codebox}
}
\end{algorithm}

\begin{algorithm}[t]\caption{Enumerate all possible mappings that eliminates universally quantified variables}\label{alg:build-map}
{\small
\begin{codebox}
  \Procname{$\proc{BuildMap}(Y, M, vis, F, f)$}
%   \li $S_1 \gets $ atoms in $C$ involving variables in $Y$
%   \li $S_2 \gets $ atoms in $C$ not involving variables in $Y$\
%   \li \If for some $y \in Y$, there does not exist a variable in $X$ or a constant in $C$ 
%   \\such that they are of the same attribute
%   \li \Then add a fresh variable of the same attribute as $y$ to $X$
%   \End
  \li \If $vis = Y$ 
  \Then \li $F \gets F \cup {f}$
  \li \Return $F$
  \End
  \li \For $y \in Y$
  \Do
    \li $A \gets attr(y)$
    \li \If $y \notin vis$ 
        \Then \li $vis \gets vis \cup \{y\}$
        \li \For $x \in M[A]$
        \Do
        \li $f \gets f \cup \{(y, x)\}$
        \li $\proc{BuildMap}(Y, M, vis, F, f)$
        \li $f \gets f \setminus \{(y, x)\}$
        \End
    \End
  \End
  \li \Return $F$
\end{codebox}
}
\end{algorithm}

\begin{algorithm}[t]\caption{Build Instance From a Conjunction}\label{alg:build-ins}
{\small
\begin{codebox}
\Procname{$\proc{BuildIns}(C, R, F)$}
\li $D \gets $ empty c-tables in schema $R$.
\li \For $f \in F$
      \Do
          \li $C' \gets P_{i1} \land P_{i2} \dots \land P_{ik_i}$
          \li \For $j \in \{1, \dots\, l_i\}$
          \Do
            % \li $Q'_{ij} \gets$ the result of mapping all variables in $Y$ in $Q_{ij}$ using $f$
            \li $Q'_{ij} \gets$ $f(Q_{ij})$
            \li $C' \gets C' \land Q'_{ij}$
          \End
          \li \For literal $e \in C'$
          \Do 
          \li \If  $e = r(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$
            \li \Then \If $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ $\notin D.r$
                \li \Then
                add $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$ to $D.r$
                \End
            \li \ElseIf $e = \neg r(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$\label{line:unsat-start}
            \li \Then  \If $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$  $\in D.r$
                \li \Then   current $C$ cannot be satisfied
                \li \Return UNSAT \label{line:unsat-end}
                \li \Else   \li add a table-wise condition that not all c-tuples \\ \quad\quad\quad\quad\quad \quad\quad\quad\quad\quad in $D.r$ are equal to  $(z^1_{ij}, z^2_{ij}, ..., z^{|attr(r)|}_{ij})$
                \End
            \li \Else   \li $e == z^1_{ij}~op~z^2_{ij}$, add it as a condition to $D$
            \End
          \End
      \End
\li \Return D
\end{codebox}
}
\end{algorithm}
      
      
\begin{algorithm}[t]\caption{\algobruteforce}\label{alg:brute-force}
{\small
\begin{codebox}
  \Procname{$\proc{\algobruteforce}(R, Q, Q_0)$}
  \li  $\phi \gets$ the FOL formula in the DRC of $Q-Q_0$ in prenex disjunctive \\normal form (PDNF), i.e., $\exists x_1,x_2,...,x_n \forall y_1, ..., y_m C_1 \lor C_2 ... \lor C_k$ \\
  where each $C_i$ is in the form of $P_{i1} \land P_{i2} ... \land P_{ik_i} \land Q_{i1} \land Q_{i2} ... \land Q_{il_i}$ \\
  (each $P_{ij}$ is a literal involving only constants and existentially quantified \\
  variables and each $Q_{ij}$ is a literal involving at least one universally\\
  quantified variables $(y_1, ..., y_n)$).
  \li $I \gets \emptyset$
  \li \For $i \in \{1, \ldots, k\}$
  \Do
      \li $X \gets$ the union of the set of existentially quantified variables, \\\quad\quad 
      the set of free variables, and the set of constants used n $C_i$
      \li $Y \gets$ the set of universally quantified variables used in $C_i$
    %   \li $F \gets$ the set of all possible mappings from $Y$ to $X$. 
      \li $M_i \gets \proc{InitDomain}(X, Y, R)$
      \li $F \gets \proc{BuildMap}(Y, M_i, \emptyset, \emptyset, \emptyset)$
      \li $D_i \gets \proc{BuildIns}(C_i, R, F)$
      \li \If generated $D_i$ is satisfiable
      \li \Then
        $I \gets I \cup \{D_i\}$
      \End
  \End
  \li \Return $I$
\end{codebox}
}
\end{algorithm}

\begin{Example}
Consider again the beer database, now the queries are $Q_1$: find drinkers who frequent some bar that does not serve all beers she likes, and a $Q_2$: find drinkers who frequent some bar that serves some beer she likes. We have the DRCs:
\begin{align*}
Q_1=\{(d_1) & \ \mid \ \exists b_1, x_1, t_1, p_1 \Big( \\
Likes(d_1, b_1) &\land Frequents(d_1, x_1, t_1) \land \neg Serves(x_1, b_1, p_1)\Big)\}\\
Q_2=\{(d_1) & \ \mid \ \exists b_1, x_1, t_1, p_1 \Big( \\
Likes(d_1, b_1) &\land Frequents(d_1, x_1, t_1) \land Serves(x_1, b_1, p_1)\Big)\}\\
\end{align*}
\begin{align*}
Q_2-Q_1=\{(d_1) & \ \mid \ \exists b_1, x_1, t_1, p_1 \Big( \\
Likes(d_1, b_1) &\land Frequents(d_1, x_1, t_1) \land Serves(x_1, b_1, p_1)\Big) \land\\
\neg \exists b_2, x_2, t_2, p_2 \Big( \\
Likes(d_1, b_2) &\land Frequents(d_1, x_2, t_2) \land \neg Serves(x_2, b_2, p_2)\Big) \}\\
= \{(d_1)  \ \mid \ &\exists b_1, x_1, t_1, p_1 \forall b_2, x_2, t_2, p_2\Big( \\
Likes(d_1, b_1) &\land Frequents(d_1, x_1, t_1) \land Serves(x_1, b_1, p_1)\Big) \land\\
 \Big( &!Likes(d_1, b_2) \lor !Frequents(d_1, x_2, t_2) \lor  Serves(x_2, b_2, p_2)\Big)
\}\\
= \{(d_1)  \ \mid \ &\exists b_1, x_1, t_1, p_1 \forall b_2, x_2, t_2, p_2\Big( \\
\big( Frequents&(d_1, x_1, t_1) \land Likes(d_1, b_1) \land\\
&Serves(x_1, b_1, p_1) \land !Frequents(d_1, x_2, t_2)  \big) \lor \\ 
\big( Frequents&(d_1, x_1, t_1) \land Likes(d_1, b_1) \land \\
&!Likes(d_1, b_2) \land 
   Serves(x_1, b_1, p_1) \big) \lor \\
   \big (Frequents&(d_1, x_1, t_1) \land 
   Likes(d_1, b_1) \land \\ &Serves(x_1, b_1, p_1) \land Serves(x_2, b_2, p_2) \big )
   \Big)
\}\\
\end{align*}
$\forall x (P(x) \lor Q(x)) \leftarrow \forall x P(x) \lor \forall x Q(x)$

$X = \{b_1, x_1, t_1, p_1\}$, $Y = \{b_2, x_2, t_2, p_2\}$, $b_2$ can only be mapped to $b_1$, $x_2$ can only be mapped to $x_1$, ..., etc. 
\par
$C_1 = Frequents(d_1, x_1, t_1) \land Likes(d_1, b_1) \land$
$Serves(x_1, b_1, p_1) \land$ $!Frequents(d_1, x_2, t_2) $, thus $C'_1 = Frequents(d_1, x_1, t_1) \land Likes(d_1, b_1) \land$
$Serves(x_1, b_1, p_1) \land$ $!Frequents(d_1, x_1, t_1) $, which is not satisfiable because of the frequent tuples.
\par $C_2 = Frequents(d_1, x_1, t_1) \land Likes(d_1, b_1) \land $ $!likes(d_1, b_2) \land$ \\$Serves(x_1, b_1, p_1)$, thus $C'_2 = Frequents(d_1, x_1, t_1) \land Likes(d_1, b_1) \land $ $!likes(d_1, b_1) \land$ $Serves(x_1, b_1, p_1)$, which is not satisfiable because of the likes tuples.
\par $C_3 = Frequents(d_1, x_1, t_1) \land Likes(d_1, b_1) \land $ $Serves(x_1, b_1, p_1) \land$ \\$Serves(x_2, b_2, p_2)$, thus $C'_3 = Frequents(d_1, x_1, t_1) \land Likes(d_1, b_1) \land $ $Serves(x_1, b_1, p_1) \land$ $Serves(x_1, b_1, p_1)$, which is satisfiable and will return the c-instance below:

\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & T \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $x_1$ & $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $b_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
        $d_1$& $x_1$ & $t_1$ & T \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $d_1$ & $b_1$ & $T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $b_1$ &$r_1$ &$p_1$ &$T$\\\hline
        % \multicolumn{4}{|c|}{$p_1 \leq p_2 \land p_2 \leq p_1$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\small
  The c-instance by $C_3$ for wrong $Q_2$ and correct $Q_1$.}
\end{figure}

\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{6em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & PrefixEve($d_1$) $\land$ FNEve($d_1$) \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $b_1$ & $*$ &$T$\\
        $b_2$ & $*$ &$T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $r_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $d_1$ & $r_1$ & $T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $b_1$ &$r_1$ &$p_1$ &$T$\\
        $b_2$ &$r_1$  &$p_2$ & $T$\\\hline
        \multicolumn{4}{|c|}{$p_1 \leq p_2 \land p_2 \leq p_1$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case2}\small
  The c-instance for wrong $Q_2$ and correct $Q_1$.}
\end{figure}
\end{Example}

\begin{Example}
Consider $Q_1$: find drinkers who frequent every bar that serves Corona, and a $Q_2$: find drinkers who frequent some bar that does not serve Corona. We have the DRCs:
\begin{align*}
Q_1=\{(d_1) & \ \mid \ \forall x_1  \Big( \big(\forall p_1 \neg Serves(x_1, \text{Corona}, p_1)\big) \lor\\
 \big(\exists t_1 &Frequents(d_1, x_1, t_1)\big) \Big)\}\\
Q_2=\{(d_1) & \ \mid \ \exists x_2, t_2  \forall p_2\Big( \neg Serves(x_2, \text{Corona}, p_2) \land\\
&Frequents(d_1, x_2, t_2) \Big)\}\\
\end{align*}
\begin{align*}
Q_1-Q_2=\{(d_1) & \ \mid \ \forall x_1, x_2, t_2, p_1 \exists t_1, p_2 \Big( \\
\big(\neg &Serves(x_1, \text{Corona}, p_1) \lor Frequents(d_1, x_1, t_1) \big)\land \\
\big(\neg &Frequents(d_1, x_2, t_2) \lor  Serves(x_2, \text{Corona}, p_2) \big)\Big) \\
= \{(d_1) & \ \mid \ \forall x_1, x_2, t_2, p_1 \exists t_1, p_2 \Big( \\
\big(&Frequents(d_1, x_1, t_1) \land \neg 
    Frequents(d_1, x_2, t_2)\big) \lor\\
\big(&Frequents(d, x_1, t_1)\land 
   Serves(x_2, \text{Corona}, p_2)\big) \lor\\
   \big(&\neg Frequents(d_1, x_2, t_2) \land  
    Serves(x_1, \text{Corona}, p_1)\big) \lor\\
\big(& Serves(x_1, \text{Corona}, p_1) \land
   Serves(x_2, \text{Corona}, p_2) \big)
\}\\
\end{align*}

$X = \{t_1, p_2, \text{Corona}, d_1\}$, $Y = \{x_1, x_2, t_2, p_1\}$, $t_2$ in $times\_a\_week$ column and $p_1$ in price column can be mapped, so we need to create fresh variables $x_3$ for bar. Now there is one possible mapping: both $x_1, x_2$ to $x_3$, $p_1$ to $p_3$, and $t_2$ to $t_1$.
\par
$C_1 = Frequents(d_1, x_1, t_1) \land \neg 
    Frequents(d_1, x_2, t_2)$, thus $C'_1 = Frequents(d_1, x_3, t_1) \land \neg Frequents(d_1, x_3, t_1)$, which is not satisfiable.
\par $C_2 = Frequents(d_1, x_1, t_1)\land 
   Serves(x_2, \text{Corona}, p_2)$, thus $C'_2 = Frequents(d_1, x_3, t_1)\land Serves(x_3, \text{Corona}, p_2)$, which is satisfiable and will return the c-instance below:
\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & T \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $x_3$ & $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $\text{Corona}$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
        $d_1$& $x_3$ & $t_1$ & T \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $x_3$ &$\text{Corona}$ &$p_3$ &$T$\\\hline
        % \multicolumn{4}{|c|}{$p_1 \leq p_2 \land p_2 \leq p_1$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\small
  The c-instance by $C_2$ for Example 4.}
\end{figure}
% \par $C_3 = \neg Frequents(d_1, x_2, t_2) \land  
%     \neg Serves(x_1, \text{Corona}, p_1)$, thus $C'_3 = \neg Frequents(d_1, x_3, t_1) \land  
%     \neg Serves(x_3, \text{Corona}, p_3)$, which is satisfiable and will return a c-instance with only one drinker tuple.

% \par $C_4 = \neg Serves(x_1, \text{Corona}, p_1) \land
%   Serves(x_2, \text{Corona}, p_2)$, thus $C'_4 = \neg Serves(x_3, \text{Corona}, p_3) \land
%   Serves(x_3, \text{Corona}, p_3)$, which is not satisfiable.

\par $C_3 = \neg Frequents(d_1, x_2, t_2) \land  
    Serves(x_1, \text{Corona}, p_1)$, thus $C'_3 = \neg Frequents(d_1, x_3, t_1) \land  
    Serves(x_3, \text{Corona}, p_1)$, which is satisfiable and will return the c-instance below:
\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & T \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $x_3$ & $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $\text{Corona}$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
        %$d_1$& $x_3$ & $t_1$ & T \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $x_3$ &$\text{Corona}$ &$p_2$ &$T$\\\hline
        % \multicolumn{4}{|c|}{$p_1 \leq p_2 \land p_2 \leq p_1$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\small
  The c-instance by $C_3$ for Example 4.}
\end{figure}
\par $C_4 = \neg Serves(x_1, \text{Corona}, p_1) \land
  Serves(x_2, \text{Corona}, p_2)$, thus $C'_4 = \neg Serves(x_3, \text{Corona}, p_2) \land
  Serves(x_3, \text{Corona}, p_2)$, which is not satisfiable.

% \zhengjie{1. There is some gap when constructing the tuples from free variables and fresh variables. 2. Case 3 gives an instance with only the drinker but no other tuples, which does not generalize the concrete counterexample, so I am afraid that we have to add the constraints to the c-table that ``the drinker does not frequent any bars and no bar serves Corona''. }
\end{Example}

% \begin{proposition}\label{prop:homomorphism_correctnesss}
% Let $C$ be a clause in $Q - Q_0$ and let $F$ be the output of Algorithm \ref{alg:build-map} on the input $C$. 
% An assignment $\alpha$ to $Q - Q_0$ satisfies $C$ iff there exists a homomorphism $h \in F$ such that $\alpha$ satisfies $h(C)$. \amir{is that correct?}
% \end{proposition}
% \zhengjie{No, $\alpha$ should be an assignment to one of the c-instances output by Algo 2, and it should satisfy $h(C)$ for all $h \in F$, or say, the result of evaluating the $C$ part of the query $Q-Q_0$ over the c-instance instantiated using $\alpha$ is not empty.}

\begin{proposition}\label{prop:sufficiency}
Given schema $R$, let $C$ be a clause in $Q - Q_0$, $M$ be the output of Algorithm~\ref{alg:init-domain}, $F$ be the output of Algorithm~\ref{alg:build-map} on $C, M$, let $D$ be the output of Algorithm~\ref{alg:build-ins} on the input $C, R, F$. 
If $D$ is UNSAT, for any $M'$ where $\forall A $ $M[A] \subseteq M'[A]$ and  $\exists A' $ $M[A'] \subsetneq M'[A']$, replacing $M$ with $M'$ in the input of Algorithm~\ref{alg:build-map} will not make $D$ SAT. \amir{has this been updated?}
\end{proposition}
\begin{proof}
Assume that on the input $C, R, F$, line~\ref{line:unsat-start} to line~\ref{line:unsat-end} in Algorithm~\ref{alg:build-ins} returns UNSAT, then there exists a mapping $h \in F$ such that there are two conflicting literals (tuple existence and non-existence) in $h(C)$. If more variables or constants are added to any of the domains in $M$, by re-running line 6 to line 8 in Algorithm~\ref{alg:brute-force}, we would obtain a new set of mappings $F'$ from Algorithm~\ref{alg:build-map} on $C, M$.
Note that the mapping $h$ that makes two literals conflict in $h(C)$ would still exist in new $F'$, since no variables or constants are removed from the domains. Therefore Algorithm~\ref{alg:build-ins} would still return UNSAT on the input $C, R, F'$.
\end{proof}

\amir{I think what you want for soundness is: `Every C-table outputted by Algorithm 4 is a minimal generalized counterexample' for this you will probably need lemmas about the output of the other algorithms}

\mypar{Method 2 (chase-based)}
Convert Q-Q0 or Q0-Q into Prenex Disjunctive Normal Form, e.g.., exists x1,x2 forall y1,y2 P1(x1, x2) || P2(x1, y1) || P3(x2, y2) ...
For each conjunction clause, use database constraints to eliminate variables
Group conjunction clauses by their use of universal-quantified variables
In each group enumerate the domain of universal-quantified variables
Issue: things get complicated when there are both universal quantifier and disjunction, in this case completeness may be hard to satisfy
Another thing is we may use the second method to initialize or guide the set of rules to be searched in method 1, when it is hard to derive rules directly.





==> sections/saved-prelim.tex <==

% \subsection{Complexity}
% The query complexity of finding a universal solution for different query classes in detailed in Table \ref{tab:complexity}.
% In general, finding a universal solution is an undecidable problem since the problem of checking DRC containment can be reduced to it (this is known to be in $co-\mathcal{RE} \setminus \mathcal{R}$ (see \cite{AHV}, Corollary 6.3.2) since if we take two queries, $Q_1$ and $Q_2$, the universal solution for $Q_1 - Q_2$ is empty iff $Q_1 \subsetneq Q_2$. 
% To show this, consider the case where the universal solution for $Q_1 - Q_2$ is empty. 
% Thus, there is no satisfying c-instance for this query, and in particular, there is no ground instance that satisfies it. 
% Suppose now that $Q_1 \subsetneq Q_2$, so we know that there is no ground instance satisfying $Q_1 - Q_2$, and therefore, there is no c-instance that satisfies $Q_1 - Q_2$.
% Hence, to ensure halting, in the following sections, we present solutions that restrict the size of the generated c-instances for the universal solution.

% For simple query classes like CQs with negations over individual atoms or conditions (denoted by $CQ_{\neg}$) and UCQs with the same type of negation (denoted by $UCQ_{\neg}$), the problem is PTime and $\#P$-complete, respectively.
% The universal solution of $q \in CQ_{\neg}$ is always a single c-instance composed of all atoms of the query and a global condition that is the conjunction of all conditions and negated atoms in the query. This implies a PTime complexity. 
% The universal solution of $Q = \{q_1, \ldots, q_u\} \in UCQ_{\neg}$ is composed of a set of c-instances where each of them is a conjunction of a subset of CQs from $\{q_1, \ldots, q_u\}$ that can be satisfied together. This is equivalent to enumerating all satisfying assignments to a DNF formula (every CQ is a conjunct in the formula) and is thus \#P-complete. 

% \begin{table}[t]
% \begin{small}
% \centering
% \caption{Complexity of finding a universal solution. The proofs can be found in the full version \cite{?} \amir{cite}}\label{tab:complexity}
% \begin{tabularx}{\linewidth}{| c | >{\centering\arraybackslash}X | c |}
% \hline Query Class & Operators & Complexity/Compatibility\\
% \hline $CQ_{\neg}$ & $\land$,$\exists$, $\neg$ for individual atoms and cond. & PTime\\
% \hline $UCQ_{\neg}$ & $\land$, $\exists$, $\lor$, $\neg$ for individual atoms and cond. & $\#P$-complete\\
% \hline $DRC$ & $\land$, $\exists$, $\neg$, $\lor$, $\forall$ & $\mathcal{RE} \setminus \mathcal{R}$ (undecidable)\\
% \hline
% \end{tabularx}
% \end{small}
% \end{table}


\cut{
Given two queries $Q_1, Q_2$ where $\exists D \in DB~ s.t. ~(Q_1 - Q_2)(D) \neq \emptyset$, then $Q_1 \neq Q_2$ can be presented as $Q_1 \land \neg Q_2$ in DRC. This will be the basis for our problem definition.
% and the c-tables are also DRC formulas such that for all $\localcond \in \localcond$,  $\localcond \implies Q_1 \land \neg Q_2$.

\begin{Definition}[Generalized counterexample using conditional tables]
Given two queries $Q_1$ and $Q_2$, and a database schema $R$, a generalized counterexample for $Q_1$ and $Q_2$ is
%a collection of c-tables $\mathcal{I}$ where for each relation $R_i \in D (1 \leq i \leq n)$ there exists a c-table $(T_i, \localcond_i) \in \mathcal{I}$, such that for all instances $D'$ of the same schema $D$, $D'=\{R'_1, R'_2, ..., R'_n\}$, $\forall i R'_i \in Rep(T_i, \localcond_i) \implies Q_1(D') \neq Q_2(D')$.
a c-instance $\mathcal{I}$ of $R$ such that for all instances $D' \in Rep(\mathcal{I}) \implies Q_1(D') \neq Q_2(D')$.
\end{Definition}

\begin{proposition}
There can be more than one generalized counterexample for two queries $Q_1, Q_2$.
\end{proposition}

\begin{proof}
Consider the simplest case where both $Q_1$ and $Q_2$ are conjunctive queries, let $Q_1 = \{(x_1) \ |\  \exists y_1 \ R(x_1, y_1)\}$ and  $Q_2 = \{(x_1) \ |\ \exists y_2, z_1 \ S(x_1, y_2) \land T(x_1, z_1)\}$. \\
$Q_1 \land \neg Q_2 = \{(x_1)\ |\  \exists y_1 \forall y_2, z_1 \ R(x_1, y_1)\land (\neg S(x_1, y_2) \lor \neg T(x_1, z_1))\}$. Since we do not allow disjunctions in the conditions of c-instances, the predicate $(\neg S(x_1, y_2) \lor \neg T(x_1, z_1))$ can only be expressed using two different c-instances, leading to two generalized counterexamples for $Q_1$ and $Q_2$.
\end{proof}

Therefore, we generate a generalized counterexamples. 

% Reformulation: what is the objective for finding such $\localcond$?
% \begin{itemize}
% \item Completeness
% \item Minimum description length --- Minimal learning effort: how complex is the generated natural language description?
% \item Diversity
% \end{itemize}

\begin{Example}

Question: For each beer liked by any drinker with the first name Eve, find the bars that serve this beer at the highest price.

Wrong query Q: 
\begin{align*}
\projection_{beer1, bar1} &((\selection_{drinker LIKE  'Eve\%'} likes) \join_{beer = beer1} ( \\
    &\rename_{bar1, beer1, price1} Serves \join_{beer1 = beer2 \land  price1>price2}\\ 
    &\rename_{bar2, beer2, price2} Serves));
\end{align*}

Standard query \qcorrect:
\begin{align*}
\projection_{beer, bar} &\Big(\big(\projection_{beer, bar} serves \difference \projection_{beer1, bar1}(\\
&\rename_{bar1, beer1, price1} serves \join_{beer1 = beer2\ \land\ price1 < price2} \\
&\rename_{bar2, beer2, price2} serves)\big) \\
\join &(\selection_{drinker \ LIKE \ 'Eve\ \%'} likes)\Big);
\end{align*}

DRC of $Q-Q_0$ ($X_1$ and $B_1$ are quantifier-free variables):
\begin{align*}
Q-Q_0=\{(X_1, B_1) & \ \mid \ \\
\exists C1, C2, C3, C4 &\Big( \\
\forall C5, C6 \Big(\exists &C7, C8, C9, C10, C11 \big(\\
Serves(X_1, B_1, C2) &\land Likes(C1, B_1) \land C1 \ LIKE \ 'Eve\%' \\
\land &Serves(C3, B_1, C4) \land C2>C4\\
\land((&Serves(C7, C8, C9) \land  Serves(C10, C8, C11) \\
\land &C9<C11 \land X_1 == C7 \land B_1==C8) \\
&\lor  !Likes(C5,B_1) \lor !(C5 \ LIKE \ 'Eve\ \%') \lor !Serves(X_1, B_1, C6))\big)\Big)\Big)\}
\end{align*}

\begin{figure*}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.3\linewidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        Eve Edwards & 32767 Magic Way& $d_1$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.38\linewidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        Restaurant Memory & 1276 Evans Estate &$b_1$\\
        Tadim & 082 Julia Underpass &$b_2$\\
        Restaurante Raffaele & 7357 Dalton Walks& $b_3$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\linewidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        American Pale Ale &  Sierra Nevada &$r_1$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.25\linewidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\linewidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       Eve Edwards & American Pale Ale & $l_1$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.4\linewidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         Restaurant Memory &American Pale Ale &2.25 &$s_1$\\
Restaurante Raffaele & American Pale Ale & 2.75 &$s_2$ \\
Tadim & American Pale Ale & 3.5 &$s_3$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:running}\small
  A counterexample instance with tuples identifiers.}
\end{figure*}

Two generalized rules:
\begin{itemize}
\item Case1: With bar $X_1, C3, C10$ serving beer $B_1$ at prices $C4 < C2 < C11$ (implied by the key constraint that $C2 = C9$), and one drinker $C1$ whose name has $PrefixEve$ and likes $B_1$.
\item Case2: With bar $X_1, C3$ serving beer $B_1$ at prices $C4 < C2 $, and one drinker $C1$ who likes $B_1$ with name has  $PrefixEve$ but not $FirstNameEve$.
\end{itemize}

\end{Example}
The tricky part: eliminating universal quantifiers, i.e. $C5$ and $C6$ in the above example. By minimizing the database we can let $C5=C1$ and $C6=C2$.

\begin{Definition}[Minimal counterexample]
\amir{verify:} A counterexample $D$ is minimal if for every set of variables $S$ in $D$ that are not referenced by any relational condition, removing all tuples and conditions containing any $x \in S$ will not convert $D$ into another counterexample. 
\end{Definition}

\begin{Definition}[Counterexample Generalization Problem]
Given two queries $Q_1$ and $Q_2$, and a database $D$ of schema $R$ where $Q_1(D) \neq Q_2(D)$, the counterexmaple generalization problem (CGP) is to find a set of generalized counterexamples $\mathcal{C}$ $=\{\mathcal{I}_1, \mathcal{I}_2 ... \}$ such that every  $\mathcal{I}_i \in \mathcal{C}$ is minimal.
% , i.e., there exists no other generalized counterexample $\mathcal{J}$ for $Q_1$ and $Q_2$ such that $Rep(\mathcal{I}_i) \subseteq Rep(\mathcal{J})$, and every for counterexample $D'$, there exists $\mathcal{I}_i \in \mathcal{C}$ such that $D' \in Rep(\mathcal{I}_i)$ \amir{Completeness}.
\end{Definition}

% \amir{Each element in the lattice is a c-table? If so, what do we have an example where one c-table implies another c-table?}



\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{7em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & $PrefixEve(d_1)$ $\land \neg$ $FNEve(d_1)$\\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $b_1$ & $*$ &$T$\\
        $b_2$ & $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $r_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $d_1$ & $r_1$ & $T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $b_1$ &$r_1$ &$p_1$ &$T$\\
        $b_2$ &$r_1$  &$p_2$ & $T$ \\\hline
        \multicolumn{3}{|c|}{$p_1 < p_2$} & \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:running}\small
  The c-instance of case 2 for wrong \qincorrect\ and correct \qcorrect.}
\end{figure}



\subsection{A simpler SPJ example}
\begin{Example}

Question: For each beer liked by any drinker with the first name Eve, find the bars that serve this beer at the non-lowest price.

Standard query $Q_1$: 
\begin{align*}
\projection_{beer1, bar1} &((\selection_{drinker LIKE  'Eve\ \%'} likes) \join_{beer = beer1} ( \\
    &\rename_{bar1, beer1, price1} Serves \join_{beer1 = beer2 \land  price1>price2} \\
    &\rename_{bar2, beer2, price2} Serves));
\end{align*}

Wrong query $Q_2$: 
\begin{align*}
\projection_{beer1, bar1} &((\selection_{drinker LIKE  'Eve\%'} likes) \join_{beer = beer1} ( \\
    &\rename_{bar1, beer1, price1} Serves \join_{beer1 = beer2 \land  price1 \geq price2  \land bar1 \neq bar2} \\
    &\rename_{bar2, beer2, price2} Serves));
\end{align*}

Similarly, the DRC of $Q_1$:
\begin{align*}
Q_1=\{(X_1, B_1) & \ \mid \ \\
\exists C1, C2 &( \\
\exists &C3, C4 ( Serves(X_1, B_1, C2) \land Likes(C1, B_1) \\
&\land C1 \ LIKE \ 'Eve \ \%' \land Serves(C3, B_1, C4) \land C2 > C4) \}
\end{align*}

DRC of $Q_2$:
\begin{align*}
Q_2=\{(X_1, B_1) & \ \mid \ \\
\exists C1, C2 &( \\
\exists &C3, C4 ( Serves(X_1, B_1, C2) \land Likes(C1, B_1) \\
&\land C1 \ LIKE \ 'Eve\%' \land Serves(C3, B_1, C4) \land C2 \geq C4 \land X_1 \neq C3) \}
\end{align*}


DRC of $Q_2-Q_1$ ($X_1$ and $B_1$ are quantifier-free variables):
\begin{align*}
Q_2-Q_1=\{(X_1, B_1) & \ \mid \ \\
\exists C1, C2, C3, C4 &\Big(\forall C5, C6, C7, C8 \big(\\
Serves&(X_1, B_1, C2) \land Likes(C1, B_1) \land C1 \ LIKE \ 'Eve\%' \land \\
Serves&(C3, B_1, C4) \land C2 \geq C4 \land X_1 \neq C3\\
\land(C6 \leq C8 &\lor !Serves(C7, B1, C8) \lor  !Likes(C5,B_1) \lor !(C5 \ LIKE \ 'Eve\ \%') \\
&\lor !Serves(X_1, B_1, C6))\big)\Big)\}
\end{align*}

Two generalized rules:
\begin{itemize}
\item Case1: With bar $X_1, C3$ serving beer $B_1$ at prices $C4 \leq C2$, and one drinker $C1$ whose name has $PrefixEve$ but not $FirstNameEve$, and likes $B_1$.
\item Case2: With bar $X_1, C3$ serving beer $B_1$ at prices $C4 = C2$, and one drinker $C1$ whose name has $PrefixEve$ and $FNEve$ and likes $B_1$.
\end{itemize}

{\color{red} 
Steps:
\begin{enumerate}
    \item DRC
    \item ``Disjunctive'' Normal form -- each disjunct forms a ``case''
    \item Form c-instance (relations are formed with $\exists$ variables, constraints with $\forall$ variables (?))
\end{enumerate}

}

\end{Example}

\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{7em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $C1$ & $*$ & PrefixEve($C1$) $\land \neg$ FNEve($C1$) \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $X_1$ & $*$ &$T$\\
        $C3$ & $*$ &$T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $B_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $C1$ & $B_1$ & $T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $X_1$ &$B_1$ &$C2$ &$T$\\
        $C3$ &$B_1$  &$C4$ & $T$\\ \hline
        \multicolumn{4}{|c|}{$C4 \leq C2$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case1}\small
  The c-instance of case 1 for wrong $Q_2$ and correct $Q_1$.}
\end{figure}

\begin{figure}[h]\scriptsize\setlength{\tabcolsep}{3pt}
 \vspace{-2mm}
  \subfloat[\small Drinker relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
  {\scriptsize
      \begin{tabular}[b]{|c|c||p{6em}|}\hline
        {\tt name} & {\tt addr} &  {\tt cond} \\ \hline
        $d_1$ & $*$ & PrefixEve($d_1$) $\land$ FNEve($d_1$) \\\hline
      \end{tabular}
      }
      \end{minipage}
      }
  \subfloat[\small Bar relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt addr} &  \\ \hline
        $b_1$ & $*$ &$T$\\
        $b_2$ & $*$ &$T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \subfloat[\small Beer relation]{
    \begin{minipage}[b]{0.27\columnwidth}\centering
    {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt name} & {\tt brewer} &  \\ \hline
        $r_1$ &  $*$ &$T$\\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-3mm}
  \\
  \hfill
    \subfloat[\small Frequents relation]{
    \begin{minipage}[b]{0.3\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
        {\tt drinker} & {\tt bar} & {\tt times} & \\ \hline
      \end{tabular}
      }
    \end{minipage}
   
  }
   \subfloat[\small Likes relation]{
    \begin{minipage}[b]{0.30\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c||c|}\hline
        {\tt drinker} & {\tt beer}  &  \\ \hline
       $d_1$ & $r_1$ & $T$ \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
   \hfill
   \subfloat[\small Serves relation]{
    \begin{minipage}[b]{0.35\columnwidth}\centering
     {\scriptsize
      \begin{tabular}[b]{|c|c|c||c|}\hline
         {\tt bar} & {\tt beer} & {\tt price} &  \\ \hline
         $b_1$ &$r_1$ &$p_1$ &$T$\\
        $b_2$ &$r_1$  &$p_2$ & $T$\\\hline
        \multicolumn{4}{|c|}{$p_1 \leq p_2 \land p_2 \leq p_1$} \\\hline
      \end{tabular}
      }
    \end{minipage}
  }
  \vspace{-2mm}
  \caption{\label{fig:spj-case2}\small
  The c-instance of case 2 for wrong $Q_2$ and correct $Q_1$.}
\end{figure}

}
% \section{Details of DRC Simplification}

% Translate $Q$ to DRC:\\
% $X_1$ and $B_1$ are quantifier-free variables

% \begin{lstlisting}[language=Mathematica]
% Reduce`ToPrenexForm[
%  Exists[{E1, P1}, 
%   Serves[X1, B1, P1] && Likes[E1, B1] && PrefixEve[E1] && 
%   Exists[{X2, P2}, (Serves[X2, B1, P2]) && (P1 > P2)]]]
% \end{lstlisting}
% Output:
% \begin{lstlisting}
% Exists[{C[1], C[2]}, 
%  Exists[{C[3], C[4]}, Serves[X1, B1, C[2]] && Likes[C[1], B1] && 
%       PrefixEve[C[1]] && Serves[C[3], B1, C[4]] && C[2] > C[4]]]
% \end{lstlisting}

% \begin{align*}
% Q=\{(X_1, B_1) & \ \mid \ \\
% \exists C1, C2 &( \\
% \exists &C3, C4 ( Serves(X_1, B_1, C2) \land Likes(C1, B_1) \\
% &\land C1 \ LIKE \ 'Eve\%' \land Serves(C3, B_1, C4) \land C2 > C4) \}
% \end{align*}

% \noindent
% Standard query \qcorrect\:
% \begin{align*}
% \projection_{beer, bar} &\Big(\big(\projection_{beer, bar} serves \difference \projection_{beer1, bar1}(\\
% &\rename_{bar1, beer1, price1} serves \join_{beer1 = beer2\ \land\ price1 < price2} \rename_{bar2, beer2, price2} serves)\big) \\
% &\join (\selection_{drinker \ LIKE \ 'Eve\ \%'} likes)\Big);
% \end{align*}

% Translate \qcorrect\ to DRC ($X_3$ and $B_4$ are quantifier-free):
% \begin{lstlisting}[language=Mathematica]
% Reduce`ToPrenexForm[
%  Exists[{E2, P3}, 
%   Serves[X3, B4, P3] && Likes[E2, B4] && 
%   FNEve[E2] && 
%     !Exists[{X4, B5}, 
%      Exists[{P4}, 
%       Serves[X4, B5, P4] && 
%         Exists[{X5, P5}, (Serves[X5, B5, P5]) && (P4 < P5)]] && 
%         (X3 == X4) && (B4 == B5)] ]]
% \end{lstlisting}
% Output:
% \begin{lstlisting}[language=Mathematica]
% Exists[{C[1], C[2]}, ForAll[{C[3], C[4], C[5], C[6], C[7]}, 
%      Serves[X3, B4, C[2]] && Likes[C[1], B4] && FNEve[C[1]] && 
%       (B4 != C[4] || X3 != C[3] || C[5] >= C[7] ||  ! Serves[C[6], C[4], C[7]] || 
%           ! Serves[C[3], C[4], C[5]])]]
% \end{lstlisting}
% \begin{align*}
% Q_0=\{(X_3, B_4) & \ \mid \ \\
% \exists C1, C2 &\Big( \\
% \forall C3, C4&, C5, C6, C7 \big( Serves(X_3, B_4, C2) \land Likes(C1, B_4) \\
% &\land C1 \ LIKE \ 'Eve \%' \land Serves(C3, B_1, C4) \land \\
% &(B_4 \neq C4 \lor X_3 \neq C3 \lor C5 \geq C7 \lor  !Serves(C6, C4, C7) \\
% &\lor !Serves(C3, C4, C5))\big)\Big)\}
% \end{align*}


% $Q - Q_0$:
% $X_1$ and $B_1$ are quantifier-free

% \begin{lstlisting}[language=Mathematica]
% Reduce`ToPrenexForm[
%  Exists[{E1, P1}, 
%   Serves[X1, B1, P1] && Likes[E1, B1] && PrefixEve[E1] && 
%     Exists[{X2, P2}, (Serves[X2, B1, P2]) && (P1 > P2)]]
%   && ! Exists[{E2, P3}, 
%     Serves[X1, B1, P3] && Likes[E2, B1] && FNEve[E2] &&  
%      !Exists[{X4, B5}, 
%       Exists[{P4}, 
%          Serves[X4, B5, P4] && 
%           Exists[{X5, P5}, 
%             (Serves[X5, B5, P5]) && (P4 < P5)]] && (X1 == X4) && (B1 == B5)]]]
% \end{lstlisting}

% Output:

% \begin{lstlisting}[language=Mathematica]
% Exists[{C[1], C[2], C[3], C[4]}, ForAll[{C[5], C[6]}, 
%      Exists[{C[7], C[8], C[9], C[10], C[11]}, 
%   Serves[X1, B1, C[2]] && Likes[C[1], B1] && 
%          PrefixEve[C[1]] && Serves[C[3], B1, C[4]] && C[2] > C[4] && 
%          ((Serves[C[7], C[8], C[9]] && Serves[C[10], C[8], C[11]] && 
%           C[9] < C[11] && X1 == C[7] && B1 == C[8]) 
%           ||  ! Likes[C[5], B1] ||  ! FNEve[C[5]] || ! Serves[X1, B1, C[6]])]]]
% \end{lstlisting}
% \begin{align*}
% Q-Q_0=\{(X_1, B_1) & \ \mid \ \\
% \exists C1, C2, C3, C4 &\Big( \\
% \forall C5, C6 \Big(\exists &C7, C8, C9, C10, C11 \big(\\
% Serves(X_1, B_1, C2) &\land Likes(C1, B_1) \land C1 \ LIKE \ 'Eve\%' \land Serves(C3, B_1, C4) \land C2>C4\\
% \land(&(Serves(C7, C8, C9) \land  Serves(C10, C8, C11) \land C9<C11 \land X_1 == C7 \land B_1==C8) \\
% &\lor  !Likes(C5,B_1) \lor !(C5 \ LIKE \ 'Eve\ \%') \lor !Serves(X_1, B_1, C6))\big)\Big)\Big)\}
% \end{align*}

% \begin{lstlisting}[language=Mathematica]
% (*By constraint: ForAll[{x1, b1, p1, p2},Implies[Serves[x1, b1, p1] &&
% Serves[x1, b1, p2], p1 == p2]],  c7 == X1 and c8 == B1 --> eliminate C6*)

% Exists[{C[1], C[2], C[3], C[4]}, ForAll[{C[5]}, 
%      Exists[{C[7], C[8], C[9], C[10], C[11]}, 
%   Serves[X1, B1, C[2]] && Likes[C[1], B1] && 
%          PrefixEve[C[1]] && Serves[C[3], B1, C[4]] && C[2] > C[4] && 
%          ((Serves[C[7], C[8], C[9]] && Serves[C[10], C[8], C[11]] && 
%           C[9] < C[11] &&  X1 == C[7] && B1 == C[8]) 
%           ||  ! Likes[C[5], B1] ||  ! FNEve[C[5]] || ! Serves[X1, B1, C[2]])]]]
% \end{lstlisting}


% \begin{lstlisting}[language=Mathematica]
% (* !Serves[X1, B1, C[2]] must be false, rerun reduce to PNF *)
% Exists[{C[1], C[2], C[3], C[4]}, 
%  ForAll[{C[5]}, Exists[{C[6], C[7], C[8], C[9], C[10]}, 
%       (B1 == C[7] && X1 == C[6] && PrefixEve[C[1]] && C[8] < C[10] && 
%       C[2] > C[4] && Likes[C[1], B1] && Serves[C[3], B1, C[4]] && 
%       Serves[C[6], C[7], C[8]] && Serves[C[9], C[7], C[10]] && Serves[X1, B1, C[2]]) || 
%       (PrefixEve[C[1]] && C[2] > C[4] && Likes[C[1], B1] &&  ! Likes[C[5], B1] && 
%             Serves[C[3], B1, C[4]] && Serves[X1, B1, C[2]]) 
%             || (PrefixEve[C[1]] && C[2] > C[4] && Likes[C[1], B1] &&  ! FNEve[C[5]] && 
%       Serves[C[3], B1, C[4]] && Serves[X1, B1, C[2]])]]]
% \end{lstlisting}

% \begin{lstlisting}[language=Mathematica]
% Clause1 : (B1 == C[7] && X1 == C[6] && PrefixEve[C[1]] && C[8] < C[10] && 
%       C[2] > C[4] && Likes[C[1], B1] && Serves[C[3], B1, C[4]] && 
%       Serves[C[6], C[7], C[8]] && Serves[C[9], C[7], C[10]] && Serves[X1, B1, C[2]])
% \end{lstlisting}

% \begin{lstlisting}[language=Mathematica]
% By the key constraint of serves table again, Implies[B1 == C[7] && X1 == C[6],  C[2]==C[8]]
% Reduce to:
%     (PrefixEve[C[1]] && C[2] < C[10] && C[2] > C[4] && Likes[C[1], B1] && Serves[C[3], B1, C[4]] && Serves[X1, B1, C[2]] && Serves[C[9], B1, C[10]] && Serves[X1, B1, C[2]])
% We have C[1] with Prefix Eve, B1 served at three bars of prices C[4] < C[2] < C[10], X1 serves B1 at C[2]
% \end{lstlisting}

% \begin{lstlisting}[language=Mathematica]
% Clause2 : (PrefixEve[C[1]] && C[2] > C[4] && Likes[C[1], B1] &&  ! Likes[C[5], B1] && 
%             Serves[C[3], B1, C[4]] && Serves[X1, B1, C[2]]) 
% It is impossible to have ! Likes[C[5], B1] for all C[5]; No further info for C[5] does not like B1. For C[5] likes B1, discuss the case that C[5] equals to C[1].
% \end{lstlisting}

% \begin{lstlisting}[language=Mathematica]
% Clause3 : (PrefixEve[C[1]] && C[2] > C[4] && Likes[C[1], B1] &&  ! FNEve[C[5]] && 
%       Serves[C[3], B1, C[4]] && Serves[X1, B1, C[2]])]]]
      
% (* So we have C[1] with Prefix Eve, B1 served at two bars of prices C[4] < C[2], X1 serves B1 at C[2].
% We have to discuss the domain of C[5]:
%     If there exists only one drinker name: C[5] == C[1], we have C[1]'s first name is not Eve; 
%     Otherwise, for all drinkers C[5], either ! Likes[C[5], B1] (Case 2) or ! FNEve[C[5]] (Case 3), which ensures that the correct query Q0 will not return (X1, B1)
%     *)
% \end{lstlisting}

% To sum up, we have three cases:
% Beer $B_1$ is served at 
% \begin{itemize}
% \item Case1: 3 bars of 3 different prices, and one drinker $C1$ has $PrefixEve$
% \item Case2: 2 bars of 2 different prices, there only exists one drinker $C1$ has $PrefixEve$ and not $FNEve$
% \item Case3: 2 bars of 2 different prices, there exists one drinker $C1$ has $PrefixEve$ (and not $FNEve$) , and other drinkers neither $FNEve$ nor $LikesB1$

% \end{itemize}

% \end{Example}

% A Subproblem: when do we use the concrete drinker name \textit{Eve} or \textit{Evelyn} instead of the rule: drinker with $PrefixEve$ not $FNEve$? 
% In our proposal, Case 3 is dropped, as it is an extension of case 2 (Case 2 implies Case 3). Case 2 and 3 come from analyzing Clause 2 and 3 and discussing the domain of the universal-quantified variable.




==> sections/working_example.tex <==
\section{Working Example}
Find drinkers such that for every beer liked by the drinker, there exists another drinker who also likes the same beer.
\begin{enumerate}
    \item $Q_1 = \{(d_1) \ \mid  \exists a_0 Drinker(d_1, a_0) \land \neg\exists b_1 \Big(Likes(d_1, b_1) \land \neg \exists d_2 \big(Likes(d_2, b_1) \land d_1 \neq d_2\big)\Big)\}$
    
    \item Convert $\neg \exists$ to $\forall$: $ \{(d_1) \ \mid  \exists a_0 Drinker(d_1, a_0) \land \forall b_1 \neg\Big(Likes(d_1, b_1) \land \neg \exists d_2 \big(Likes(d_2, b_1) \land d_1 \neq d_2\big)\Big)\}$
    
    \item Put negation inside second clause: $ \{(d_1) \ \mid  \exists a_0 Drinker(d_1, a_0) \land \forall b_1 \Big(\neg Likes(d_1, b_1) \lor \exists d_2 \big(Likes(d_2, b_1) \land d_1 \neq d_2\big)\Big)\}$
    
    % \item $\{d_1 \ \mid \ \exists a_0 \forall b_1 \exists d_2\ \Big (Drinker(d_1, a_0) \land \big(\neg Likes(d_1,b_1) \lor (Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \Big)\}$
    
    \item Convert to PNF: $\{d_1 \ \mid \ \exists a_0 \forall b_1 \exists d_2\ \Big (Drinker(d_1, a_0) \land \big(\neg Likes(d_1,b_1) \lor (Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \Big)\}$
    \item Convert to PDNF: $\{d_1 \ \mid \ \exists a_0 \forall b_1 \exists d_2\ \Big (\big(Drinker(d_1, a_0) \land \neg Likes(d_1,b_1) \big) \lor \big( Drinker(d_1,a_0) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \Big)\}$
    
    \item Wishful Thinking (the bold atom does not exist in step 5). Adding $Likes(d_1, b_1)$ ensures that the two conjuncts would give different counter-examples:
    $\{d_1 \ \mid \ \exists a_0 \forall b_1 \big(Drinker(d_1, a_0) \land \neg Likes(d_1,b_1) \big)$ \\
    $\lor \exists a_0 \forall b_1 \exists d_2 \big( Drinker(d_1,a_0) \land {\bf Likes(d_1, b_1)} \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \}$
    
\end{enumerate}

% \paragraph*{Suggestions}
% \begin{itemize}
%     \item When dividing the PDNF into multiple branches, we should guarantee that every quantified variable is followed with a relational atom without inner quantified variables.
% \end{itemize}

\paragraph*{Requirements}
\begin{itemize}
    \item Every clause can be satisfied
    \item When dividing the PDNF into multiple branches, we should guarantee that every quantified variable \amir{universally quantified?} is followed with a relational atom without inner quantified variables.
    \item Every clause defines a generalized counter example that is not subsumed in another generalized counter example defined by a different clause
    \item \amir{more?}
\end{itemize}

% \begin{figure*}[!h]
% \raggedright
% A safe query for the $Q_1 = \{d_1 \ \mid \ \forall b_1 \ \Big( Likes(d_1,b_1) \implies \exists d_2 \ Likes(d_2, b_1) \land d_1 \neq d_2 \Big)\}$above (find drinkers such that for every beer liked by the drinker, there exists another drinker who also likes the same beer:

% $\{(d_1) \ \mid  \exists a_0 Drinker(d_1, a_0) \land \neg\exists b_1 \Big(Likes(d_1, b_1) \land \neg \exists d_2 \big(Likes(d_2, b_1) \land d_1 \neq d_2\big)\Big)\}$

% Compare with the PNF from Mathematica:
% $\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2\ \Big (Likes(d_1, b_0) \land \big(\neg Likes(d_1,b_1) \lor (Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \Big)\}$

% PDNF:
% $\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2\ \Big (\big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \big) \lor \big( Likes(d_1,b_0) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \Big)\}$

% Convert to disjunction:
% $\{d_1 \ \mid \ \exists b_0 \forall b_1 \big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \big) \lor \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \}$

% The first part is equivalent to a safe formula $\exists b_0 Likes(d_1, b_0)  \land \neg\exists b_1Likes(d_1,b_1) $ .

% While the second part is not safe as neither of $b_1$ and $d_1$ is limited: $\exists b_0 Likes(d_1,b_0) \land\neg\exists b_1 \neg\exists d_2 \big(  Likes(d_2, b_1) \land d_1 \neq d_2 \big )$

% Option1: record the positive formula for $b_1$ and $d_1$, which is $Likes(d_1, b_1)$; add it to the conjunction: $\exists b_0 Likes(d_1,b_0) \land\neg\exists b_1 \bigg(Likes(d_1, b_1) \land \neg\exists d_2 \big(  Likes(d_2, b_1) \land d_1 \neq d_2 \big )\bigg)$, which goes back to the original formula :(

% %Option2: Relax the safety constraint. Observe that in the second part, $\forall b_1$ is not followed by a predicate of $b_1$ ($Likes(d_2, b_1)$ is in the formula of $\exists  d_2$), so we have to add a predicate of $b_1$ without $d_2$:
% %$\exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_1, b_1) \land  Likes(d_2, b_1) \land d_1 \neq d_2 \big ) $
% Option2: more careful conversion to PDNF: For a disjunctive sub-formula $P_1 \lor P_2 \lor ... \lor P_m$, convert it into $(P_1 \land \neg P_2 \land ... \neg P_m) \lor (P_2 \land \neg P_1 ... \land \neg P_m) \lor ... \lor (P_m \land \neg P_1 ... \land \neg  P_{m-1})$

% $\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2\ \Big (Likes(d_1, b_0) \land \big(\neg Likes(d_1,b_1) \land \neg(Likes(d_2, b_1) \land d_1 \neq d_2) \big ) \\ \lor (Likes(d_2, b_1) \land d_1 \neq d_2 \land Likes(d_1,b_1)) \big ) \Big)\}$

% $\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2 \big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \land d_1 = d_2\big) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_1, b_1) \land Likes(d_2, b_1) \land d_1 \neq d_2 \big ) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land \neg Likes(d_1, b_1) \land \neg Likes(d_2, b_1)\big ) \}$ 

% The first and the third cases will lead to UNSAT results.

% \\

% For the query $Q_2$ above, which finds drinkers who likes two different beers (in a overcomplex way), we can do the same trick: 

% $Q_2 = \{d_1 \ \mid \ \exists b Likes(d_1, b) \land \big (\forall b_1 \ Likes(d_1,b_1) \implies \exists b_2 \ Likes(d_1, b_2) \land b_1 \neq b_2 \big)\}$, we will have have the PDNF 

% $\{ d_1 \mid \exists _{\{b_0\}}\forall _{\{b_1\}}\exists _{\{b_2\}}(\text{Likes}(d_1,b_0)\land ((\text{Likes}(d_1,b_2)\land b_1\neq b_2)\lor \neg \text{Likes}(d_1,b_1))) \}$

% $\{ d_1 \mid \exists _{\{b_0\}}\forall _{\{b_1\}}\exists _{\{b_2\}}(\text{Likes}(d_1,b_0)\land ((\text{Likes}(d_1,b_2)\land b_1\neq b_2 \land Likes(d_1, b_1))\lor (\neg \text{Likes}(d_1,b_1) \land \neq(\text{Likes}(d_1,b_2)\land b_1\neq b_2)))) \}$

% $\{d_1 \ \mid \ \exists b_0 \forall b_1 \exists d_2 \big(Likes(d_1, b_0) \land \neg Likes(d_1,b_1) \land d_1 = d_2\big) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land Likes(d_1, b_1) \land Likes(d_1, b_2) \land b_1 \neq b_2 \big ) \\ \lor  \exists b_0 \forall b_1 \exists d_2 \big( Likes(d_1,b_0) \land \neg Likes(d_1, b_1) \land \neg Likes(d_1, b_2)\big ) \}$ 
% Again the first and the third cases will lead to UNSAT results.

% \end{figure*}

